Taming the Zoo of Tetraquarks and Pentaquarks using the HISH Model

In this paper we scan over all possible charmed tetraquarks and pentaquarks. Using the holography inspired stringy hadron (HISH) model we determine the trajectories associated with each of the exotic hadron candidates. The trajectories include further exotic states with higher angular momentum or higher stringy excited states. A trajectory is a property of a genuine exotic hadron and can be used to distinguish between the latter and a molecule. We examine 71 tetraquarks and 210 pentaquarks. Few of these states have already been found but most of the predicted zoo have yet not been discovered. We analyze the strong decay processes of these exotic hadrons and compute the corresponding decay widths of part of them.

==> pentaquarks/PN_plus_psi/baryon/fit-_PN__psi__baryon_fixed_slope_n.tex <==
\begin{longtable}[c]{|c|c|c|c|c|c|}
  \hline
  \thead{$State$} & \thead{$M$ \\ $[MeV]$} & \thead{Thry \\ $M$ \\ $[MeV]$} & \thead{$J$} & \thead{Thry \\ $n$} & \thead{Thry \\ $J + n$} \\
  \hline
  \hline
$P(4312)^{N^{+}}_{\psi 0}$ & $4312$ & $4312$ & $0$ & $0$ & $0$ \\
\hline
$P(4440)^{N^{+}}_{\psi 0}$ & $4440$ & $4449$ & $0$ & $1$ & $2$ \\
\hline
$P(4450)^{N^{+}}_{\psi 0}$ & $4450$ & $4449$ & $0$ & $1$ & $2$ \\
\hline
$P(4457)^{N^{+}}_{\psi 0}$ & $4457$ & $4449$ & $0$ & $1$ & $2$ \\
\hline
 &  & $4581$ &  &  & $2$ \\
\hline
 &  & $4708$ &  &  & $4$ \\
\hline
 &  & $4832$ &  &  & $4$ \\
\hline
 &  & $4952$ &  &  & $6$ \\
\hline
  \caption{$P_{\psi}^{N^{+}}$ $(J, M^{2})$ HMRT.}
 \end{longtable}

==> pentaquarks/PN_plus_psi/baryon/fit-_PN__psi__baryon_fixed_slope_n_fit_output_all.tex <==
\begin{longtable}[c]{|c|c|c|c|c|c|c|}
  \hline
  \thead{$\chi^{2}_{r}$} & \thead{$\chi^{2}_{hish}$} & \thead{$\alpha^{'}$} & \thead{$a$} & \thead{$m_{1}$} & \thead{$m_{2}$} & \thead{Fit Type} \\
  \hline
  \hline
0.04 & 0.00 & 1.19 & -7.11 & 2.31 & 0.04 & free fit \\
\hline
0.08 & 0.00 & 0.95 & -5.80 & 2.25 & 0.01 & fixed $m_{1}$, $m_{2}$ and $\alpha^{'}$ \\
\hline
0.04 & 0.00 & 0.95 & -10.94 & 1.37 & 0.02 & fixed $\alpha^{'}$ \\
\hline
0.02 & 0.00 & 1.17 & -7.41 & 2.25 & 0.01 & fixed $m_{1}$ and $m_{2}$ \\
\hline
  \caption{}
 \end{longtable}

==> pentaquarks/PN_plus_psi/baryon/fit-_PN__psi__baryon_new_n.tex <==
\begin{longtable}[c]{|c|c|c|c|c|c|}
  \hline
  \thead{$State$} & \thead{$M$ \\ $[MeV]$} & \thead{Thry \\ $M$ \\ $[MeV]$} & \thead{$J$} & \thead{Thry \\ $n$} & \thead{Thry \\ $J + n$} \\
  \hline
  \hline
$P(4312)^{N^{+}}_{\psi 0}$ & $4312$ & $4312$ & $0$ & $0$ & $0$ \\
\hline
$P(4440)^{N^{+}}_{\psi 0}$ & $4440$ & $4449$ & $0$ & $1$ & $2$ \\
\hline
$P(4450)^{N^{+}}_{\psi 0}$ & $4450$ & $4449$ & $0$ & $1$ & $2$ \\
\hline
$P(4457)^{N^{+}}_{\psi 0}$ & $4457$ & $4449$ & $0$ & $1$ & $2$ \\
\hline
 &  & $4579$ &  &  & $2$ \\
\hline
 &  & $4703$ &  &  & $4$ \\
\hline
 &  & $4822$ &  &  & $4$ \\
\hline
 &  & $4936$ &  &  & $6$ \\
\hline
  \caption{$P_{\psi}^{N^{+}}$ $(J, M^{2})$ HMRT.}
 \end{longtable}

==> pentaquarks/PN_plus_psi/baryon/fit-_PN__psi__baryon_prev_n.tex <==
\begin{longtable}[c]{|c|c|c|c|c|c|}
  \hline
  \thead{$State$} & \thead{$M$ \\ $[MeV]$} & \thead{Thry \\ $M$ \\ $[MeV]$} & \thead{$J$} & \thead{Thry \\ $n$} & \thead{Thry \\ $J + n$} \\
  \hline
  \hline
$P(4312)^{N^{+}}_{\psi 0}$ & $4312$ & $4288$ & $0$ & $0$ & $0$ \\
\hline
$P(4440)^{N^{+}}_{\psi 0}$ & $4440$ & $4457$ & $0$ & $1$ & $2$ \\
\hline
$P(4450)^{N^{+}}_{\psi 0}$ & $4450$ & $4457$ & $0$ & $1$ & $2$ \\
\hline
$P(4457)^{N^{+}}_{\psi 0}$ & $4457$ & $4457$ & $0$ & $1$ & $2$ \\
\hline
 &  & $4616$ &  &  & $2$ \\
\hline
 &  & $4766$ &  &  & $4$ \\
\hline
 &  & $4909$ &  &  & $4$ \\
\hline
 &  & $5046$ &  &  & $6$ \\
\hline
  \caption{$P_{\psi}^{N^{+}}$ $(J, M^{2})$ HMRT.}
 \end{longtable}

==> pentaquarks/PN_plus_psi/tetra/fit-_PN__psi__tetra_fixed_slope_n.tex <==
\begin{longtable}[c]{|c|c|c|c|c|c|}
  \hline
  \thead{$State$} & \thead{$M$ \\ $[MeV]$} & \thead{Thry \\ $M$ \\ $[MeV]$} & \thead{$J$} & \thead{Thry \\ $n$} & \thead{Thry \\ $J + n$} \\
  \hline
  \hline
$P(4312)^{N^{+}}_{\psi 0}$ & $4312$ & $4275$ & $0$ & $0$ & $0$ \\
\hline
$P(4440)^{N^{+}}_{\psi 0}$ & $4440$ & $4462$ & $0$ & $1$ & $2$ \\
\hline
$P(4450)^{N^{+}}_{\psi 0}$ & $4450$ & $4462$ & $0$ & $1$ & $2$ \\
\hline
$P(4457)^{N^{+}}_{\psi 0}$ & $4457$ & $4462$ & $0$ & $1$ & $2$ \\
\hline
 &  & $4640$ &  &  & $2$ \\
\hline
 &  & $4811$ &  &  & $4$ \\
\hline
 &  & $4976$ &  &  & $4$ \\
\hline
 &  & $5135$ &  &  & $6$ \\
\hline
  \caption{$P_{\psi}^{N^{+}}$ HMRT.}
 \end{longtable}

==> pentaquarks/PN_plus_psi/tetra/fit-_PN__psi__tetra_fixed_slope_n_fit_output_all.tex <==
\begin{longtable}[c]{|c|c|c|c|c|c|c|}
  \hline
  \thead{$\chi^{2}_{r}$} & \thead{$\chi^{2}_{hish}$} & \thead{$\alpha^{'}$} & \thead{$a$} & \thead{$m_{1}$} & \thead{$m_{2}$} & \thead{Fit Type} \\
  \hline
  \hline
0.04 & 0.00 & 0.98 & -10.23 & 1.51 & 0.14 & free fit \\
\hline
0.23 & 0.00 & 0.65 & -8.09 & 1.12 & 0.03 & fixed $m_{1}$, $m_{2}$ and $\alpha^{'}$ \\
\hline
0.55 & 0.00 & 0.65 & -9.19 & 0.83 & 0.05 & fixed $\alpha^{'}$ \\
\hline
0.02 & 0.00 & 0.91 & -11.88 & 1.12 & 0.03 & fixed $m_{1}$ and $m_{2}$ \\
\hline
  \caption{}
 \end{longtable}

==> pentaquarks/PN_plus_psi/tetra/fit-_PN__psi__tetra_new_n.tex <==
\begin{longtable}[c]{|c|c|c|c|c|c|}
  \hline
  \thead{$State$} & \thead{$M$ \\ $[MeV]$} & \thead{Thry \\ $M$ \\ $[MeV]$} & \thead{$J$} & \thead{Thry \\ $n$} & \thead{Thry \\ $J + n$} \\
  \hline
  \hline
$P(4312)^{N^{+}}_{\psi 0}$ & $4312$ & $4312$ & $0$ & $0$ & $0$ \\
\hline
$P(4440)^{N^{+}}_{\psi 0}$ & $4440$ & $4449$ & $0$ & $1$ & $2$ \\
\hline
$P(4450)^{N^{+}}_{\psi 0}$ & $4450$ & $4449$ & $0$ & $1$ & $2$ \\
\hline
$P(4457)^{N^{+}}_{\psi 0}$ & $4457$ & $4449$ & $0$ & $1$ & $2$ \\
\hline
 &  & $4581$ &  &  & $2$ \\
\hline
 &  & $4708$ &  &  & $4$ \\
\hline
 &  & $4831$ &  &  & $4$ \\
\hline
 &  & $4950$ &  &  & $6$ \\
\hline
  \caption{$P_{\psi}^{N^{+}}$ HMRT.}
 \end{longtable}

==> pentaquarks/PN_plus_psi/tetra/fit-_PN__psi__tetra_prev_n.tex <==
\begin{longtable}[c]{|c|c|c|c|c|c|}
  \hline
  \thead{$State$} & \thead{$M$ \\ $[MeV]$} & \thead{Thry \\ $M$ \\ $[MeV]$} & \thead{$J$} & \thead{Thry \\ $n$} & \thead{Thry \\ $J + n$} \\
  \hline
  \hline
$P(4312)^{N^{+}}_{\psi 0}$ & $4312$ & $4270$ & $0$ & $0$ & $0$ \\
\hline
$P(4440)^{N^{+}}_{\psi 0}$ & $4440$ & $4463$ & $0$ & $1$ & $2$ \\
\hline
$P(4450)^{N^{+}}_{\psi 0}$ & $4450$ & $4463$ & $0$ & $1$ & $2$ \\
\hline
$P(4457)^{N^{+}}_{\psi 0}$ & $4457$ & $4463$ & $0$ & $1$ & $2$ \\
\hline
 &  & $4647$ &  &  & $2$ \\
\hline
 &  & $4824$ &  &  & $4$ \\
\hline
 &  & $4993$ &  &  & $4$ \\
\hline
 &  & $5156$ &  &  & $6$ \\
\hline
  \caption{$P_{\psi}^{N^{+}}$ HMRT.}
 \end{longtable}

==> pentaquarks/Pccuds/by_J_one_point/fit-_P0_psi_s_baryon_one_by_j.tex <==
\begin{longtable}[c]{|c|c|c|c|c|c|}
  \hline
  \thead{$State$} & \thead{$M$ \\ $[MeV]$} & \thead{Thry \\ $M$ \\ $[MeV]$} & \thead{$J$} & \thead{Thry \\ $n$} & \thead{Thry \\ $J + n$} \\
  \hline
  \hline
$P_{\psi s0}(4338)^{0}$ & $4338$ & $4338$ &  &  & $0$ \\
\hline
 &  & $4506$ &  &  & $2$ \\
\hline
 &  & $4661$ &  &  & $2$ \\
\hline
 &  & $4806$ &  &  & $4$ \\
\hline
 &  & $4943$ &  &  & $4$ \\
\hline
  \caption{$\P^{\Lambda}_{\psi s} (J, M^{2})$ HMRT.} \label{table:Pccuds_J_HMRT}
 \end{longtable}

==> pentaquarks/Pccuds/by_J_one_point/fit-_P0_psi_s_tetra_one_by_j.tex <==
\begin{longtable}[c]{|c|c|c|c|c|c|}
  \hline
  \thead{$State$} & \thead{$M$ \\ $[MeV]$} & \thead{Thry \\ $M$ \\ $[MeV]$} & \thead{$J$} & \thead{Thry \\ $n$} & \thead{Thry \\ $J + n$} \\
  \hline
  \hline
$P_{\psi s0}(4338)^{0}$ & $3178$ & $3178$ &  &  & $0$ \\
\hline
 &  & $3442$ &  &  & $1$ \\
\hline
 &  & $3680$ &  &  & $2$ \\
\hline
 &  & $3898$ &  &  & $3$ \\
\hline
 &  & $4101$ &  &  & $4$ \\
\hline
  \caption{$\P^{\Lambda}_{\psi s} (J, M^{2})$ HMRT.} \label{table:Pccuds_J_HMRT}
 \end{longtable}

==> pentaquarks/Pccuds/by_n_one_point/fit-_P0_psi_s_baryon_one_by_n.tex <==
\begin{longtable}[c]{|c|c|c|c|c|c|}
  \hline
  \thead{$State$} & \thead{$M$ \\ $[MeV]$} & \thead{Thry \\ $M$ \\ $[MeV]$} & \thead{$J$} & \thead{Thry \\ $n$} & \thead{Thry \\ $J + n$} \\
  \hline
  \hline
$P_{\psi s0}(4338)^{0}$ & $4338$ & $4338$ &  &  & $0$ \\
\hline
 &  & $4522$ &  &  & $2$ \\
\hline
 &  & $4691$ &  &  & $2$ \\
\hline
 &  & $4848$ &  &  & $4$ \\
\hline
 &  & $4996$ &  &  & $4$ \\
\hline
  \caption{$\P^{\Lambda}_{\psi s} (n, M^{2})$ HMRT.} \label{table:Pccuds_n_HMRT}
 \end{longtable}

==> pentaquarks/Pccuds/by_n_one_point/fit-_P0_psi_s_tetra_one_by_n.tex <==
\begin{longtable}[c]{|c|c|c|c|c|c|}
  \hline
  \thead{$State$} & \thead{$M$ \\ $[MeV]$} & \thead{Thry \\ $M$ \\ $[MeV]$} & \thead{$J$} & \thead{Thry \\ $n$} & \thead{Thry \\ $J + n$} \\
  \hline
  \hline
$P_{\psi s0}(4338)^{0}$ & $3178$ & $3178$ &  &  & $0$ \\
\hline
 &  & $3562$ &  &  & $1$ \\
\hline
 &  & $3894$ &  &  & $2$ \\
\hline
 &  & $4192$ &  &  & $3$ \\
\hline
 &  & $4465$ &  &  & $4$ \\
\hline
  \caption{$\P^{\Lambda}_{\psi s} (n, M^{2})$ HMRT.} \label{table:Pccuds_n_HMRT}
 \end{longtable}

==> tetraquarks/T_cscs/by_n/Tcscs0/fit-_X_0j_Tccss_fixed_m_n.tex <==
\begin{longtable}[c]{|c|c|c|c|c|c|}
  \hline
  \thead{$State$} & \thead{$M$ \\ $[MeV]$} & \thead{Thry \\ $M$ \\ $[MeV]$} & \thead{$J$} & \thead{Thry \\ $n$} & \thead{Thry \\ $J + n$} \\
  \hline
  \hline
$X(3960)$ & $3955$ & $3994$ & $0$ & $0$ & $0$ \\
\hline
$X(4500)$ & $4506$ & $4407$ & $0$ & $1$ & $1$ \\
\hline
$X(4700)$ & $4704$ & $4758$ & $0$ & $2$ & $2$ \\
\hline
 &  & $5070$ &  &  & $3$ \\
\hline
 &  & $5354$ &  &  & $4$ \\
\hline
 &  & $5618$ &  &  & $5$ \\
\hline
 &  & $5864$ &  &  & $6$ \\
\hline
  \caption{$T_{\psi\phi}$ Regge trajectory.}
 \end{longtable}

==> tetraquarks/T_cscs/by_n/Tcscs0/fit-_X_0j_Tccss_fixed_slope_n.tex <==
\begin{longtable}[c]{|c|c|c|c|c|c|}
  \hline
  \thead{$State$} & \thead{$M$ \\ $[MeV]$} & \thead{Thry \\ $M$ \\ $[MeV]$} & \thead{$J$} & \thead{Thry \\ $n$} & \thead{Thry \\ $J + n$} \\
  \hline
  \hline
$X(3960)$ & $3955$ & $3985$ & $0$ & $0$ & $0$ \\
\hline
$X(4500)$ & $4506$ & $4411$ & $0$ & $1$ & $1$ \\
\hline
$X(4700)$ & $4704$ & $4765$ & $0$ & $2$ & $2$ \\
\hline
 &  & $5077$ &  &  & $3$ \\
\hline
 &  & $5360$ &  &  & $4$ \\
\hline
 &  & $5621$ &  &  & $5$ \\
\hline
 &  & $5865$ &  &  & $6$ \\
\hline
  \caption{$T_{\psi\phi}$ Regge trajectory.}
 \end{longtable}

==> tetraquarks/T_cscs/by_n/Tcscs0/fit-_X_0j_Tccss_fixed_slope_n_fit_output_all.tex.tex <==
\begin{table}[!ht]
 \centering
 {\small
 \begin{tabular}{ccccccc}
  \hline
  \hline
  \thead{$\chi^{2}_{r}$} & \thead{$\chi^{2}_{hish}$} & \thead{$\alpha^{'}$} & \thead{$a$} & \thead{$m_{1}$} & \thead{$m_{2}$} & \thead{Fit Type} \\
  \hline
  \hline
3.01 & 0.01 & 0.67 & -0.16 & 1.90 & 1.90 & free fit \\
\hline
6.52 & 0.04 & 0.59 & -2.10 & 1.50 & 1.50 & fixed $m_{1}$, $m_{2}$ and $\alpha^{'}$ \\
\hline
3.82 & 0.01 & 0.59 & -0.32 & 1.84 & 1.84 & fixed $\alpha^{'}$ \\
\hline
5.52 & 0.02 & 0.44 & -1.38 & 1.50 & 1.50 & fixed $m_{1}$ and $m_{2}$ \\
\hline
  \hline
 \end{tabular}}
 \caption{}
\end{table}

==> tetraquarks/T_cscs/by_n/Tcscs0/fit-_X_0j_Tccss_prev_n.tex <==
\begin{longtable}[c]{|c|c|c|c|c|c|}
  \hline
  \thead{$State$} & \thead{$M$ \\ $[MeV]$} & \thead{Thry \\ $M$ \\ $[MeV]$} & \thead{$J$} & \thead{Thry \\ $n$} & \thead{Thry \\ $J + n$} \\
  \hline
  \hline
$X(3960)$ & $3955$ & $4006$ & $0$ & $0$ & $0$ \\
\hline
$X(4500)$ & $4506$ & $4404$ & $0$ & $1$ & $1$ \\
\hline
$X(4700)$ & $4704$ & $4744$ & $0$ & $2$ & $2$ \\
\hline
 &  & $5046$ &  &  & $3$ \\
\hline
 &  & $5323$ &  &  & $4$ \\
\hline
 &  & $5579$ &  &  & $5$ \\
\hline
 &  & $5820$ &  &  & $6$ \\
\hline
  \caption{$T_{\psi\phi}$ Regge trajectory.}
 \end{longtable}

==> tetraquarks/T_cscs/by_n/Tcscs1/fit-_X_1j_Tccss_fixed_m_n.tex <==
\begin{longtable}[c]{|c|c|c|c|c|c|}
  \hline
  \thead{$State$} & \thead{$M$ \\ $[MeV]$} & \thead{Thry \\ $M$ \\ $[MeV]$} & \thead{$J$} & \thead{Thry \\ $n$} & \thead{Thry \\ $J + n$} \\
  \hline
  \hline
$X(4140)$ & $4148$ & $4100$ & $1$ & $0$ & $1$ \\
\hline
$X(4274)$ & $4273$ & $4377$ & $1$ & $1$ & $2$ \\
\hline
$X(4685)$ & $4684$ & $4624$ & $1$ & $2$ & $3$ \\
\hline
 &  & $4849$ &  &  & $4$ \\
\hline
 &  & $5059$ &  &  & $5$ \\
\hline
 &  & $5256$ &  &  & $6$ \\
\hline
 &  & $5442$ &  &  & $7$ \\
\hline
  \caption{$T_{\psi\phi}$ Regge trajectory.}
 \end{longtable}

==> tetraquarks/T_cscs/by_n/Tcscs1/fit-_X_1j_Tccss_fixed_slope_n.tex <==
\begin{longtable}[c]{|c|c|c|c|c|c|}
  \hline
  \thead{$State$} & \thead{$M$ \\ $[MeV]$} & \thead{Thry \\ $M$ \\ $[MeV]$} & \thead{$J$} & \thead{Thry \\ $n$} & \thead{Thry \\ $J + n$} \\
  \hline
  \hline
$X(4140)$ & $4148$ & $4102$ & $1$ & $0$ & $1$ \\
\hline
$X(4274)$ & $4273$ & $4372$ & $1$ & $1$ & $2$ \\
\hline
$X(4685)$ & $4684$ & $4626$ & $1$ & $2$ & $3$ \\
\hline
 &  & $4866$ &  &  & $4$ \\
\hline
 &  & $5094$ &  &  & $5$ \\
\hline
 &  & $5313$ &  &  & $6$ \\
\hline
 &  & $5522$ &  &  & $7$ \\
\hline
  \caption{$T_{\psi\phi}$ Regge trajectory.}
 \end{longtable}

==> tetraquarks/T_cscs/by_n/Tcscs1/fit-_X_1j_Tccss_fixed_slope_n_fit_output_all.tex.tex <==
\begin{table}[!ht]
 \centering
 {\small
 \begin{tabular}{ccccc}
  \hline
  \hline
  \thead{$\chi^{2}_{r}$} & \thead{$\chi^{2}_{hish}$} & \thead{$\alpha^{'}$} & \thead{$a$} & \thead{$m_{1}$} & \thead{$m_{2}$} & \thead{Fit Type} \\
  \hline
  \hline
6.16 & 0.02 & 0.43 & -6.20 & 0.08 & 0.08 & free fit \\
\hline
3.68 & 0.02 & 0.59 & -1.08 & 1.50 & 1.50 & fixed $m_{1}$, $m_{2}$ and $\alpha^{'}$ \\
\hline
6.58 & 0.02 & 0.59 & -2.30 & 1.30 & 1.30 & fixed $\alpha^{'}$ \\
\hline
6.80 & 0.02 & 0.65 & -1.37 & 1.50 & 1.50 & fixed $m_{1}$ and $m_{2}$ \\
\hline
  \hline
 \end{tabular}}
 \caption{}
\end{table}

==> tetraquarks/T_cscs/by_n/Tcscs1/fit-_X_1j_Tccss_new_n.tex <==
\begin{longtable}[c]{|c|c|c|c|c|c|}
  \hline
  \thead{$State$} & \thead{$M$ \\ $[MeV]$} & \thead{Thry \\ $M$ \\ $[MeV]$} & \thead{$J$} & \thead{Thry \\ $n$} & \thead{Thry \\ $J + n$} \\
  \hline
  \hline
$X(4140)$ & $4148$ & $4102$ & $1$ & $0$ & $1$ \\
\hline
$X(4274)$ & $4273$ & $4376$ & $1$ & $1$ & $2$ \\
\hline
$X(4685)$ & $4684$ & $4631$ & $1$ & $2$ & $3$ \\
\hline
 &  & $4870$ &  &  & $4$ \\
\hline
 &  & $5097$ &  &  & $5$ \\
\hline
 &  & $5312$ &  &  & $6$ \\
\hline
 &  & $5518$ &  &  & $7$ \\
\hline
  \caption{$T_{\psi\phi}$ Regge trajectory.}
 \end{longtable}

==> tetraquarks/X_3350_/by_J/fit-_X_X_3350__by_j_fixed_m_j.tex <==
\begin{longtable}[c]{|c|c|c|c|c|c|}
  \hline
  \thead{$State$} & \thead{$M$ \\ $[MeV]$} & \thead{Thry \\ $M$ \\ $[MeV]$} & \thead{$J$} & \thead{Thry \\ $n$} & \thead{Thry \\ $J + n$} \\
  \hline
  \hline
 &  & $1816$ &  &  & $1$ \\
\hline
 &  & $2745$ &  &  & $2$ \\
\hline
$X(3350)$ & $3350$ & $3350$ & $0$ & $3$ & $3$ \\
\hline
$X(3800)$ & $3840$ & $3840$ & $1$ & $3$ & $4$ \\
\hline
 &  & $4264$ &  &  & $5$ \\
\hline
 &  & $4644$ &  &  & $6$ \\
\hline
  \caption{$X(3350)$ HMRT.}
 \end{longtable}

==> tetraquarks/X_3350_/by_J/fit-_X_X_3350__by_j_new_j.tex <==
\begin{longtable}[c]{|c|c|c|c|c|c|}
  \hline
  \thead{$State$} & \thead{$M$ \\ $[MeV]$} & \thead{Thry \\ $M$ \\ $[MeV]$} & \thead{$J$} & \thead{Thry \\ $n$} & \thead{Thry \\ $J + n$} \\
  \hline
  \hline
 &  & $1529$ &  &  & $1$ \\
\hline
 &  & $2729$ &  &  & $2$ \\
\hline
$X(3350)$ & $3350$ & $3350$ & $0$ & $3$ & $3$ \\
\hline
$X(3800)$ & $3840$ & $3840$ & $1$ & $3$ & $4$ \\
\hline
 &  & $4260$ &  &  & $5$ \\
\hline
 &  & $4634$ &  &  & $6$ \\
\hline
  \caption{$X(3350)$ HMRT.}
 \end{longtable}

==> tetraquarks/X_3350_/by_J/fit-_X_X_3350__by_j_prev_j.tex <==
\begin{longtable}[c]{|c|c|c|c|c|c|}
  \hline
  \thead{$State$} & \thead{$M$ \\ $[MeV]$} & \thead{Thry \\ $M$ \\ $[MeV]$} & \thead{$J$} & \thead{Thry \\ $n$} & \thead{Thry \\ $J + n$} \\
  \hline
  \hline
 &  & $2891$ &  &  & $1$ \\
\hline
 &  & $3193$ &  &  & $2$ \\
\hline
$X(3350)$ & $3350$ & $3461$ & $0$ & $3$ & $3$ \\
\hline
$X(3800)$ & $3840$ & $3706$ & $1$ & $3$ & $4$ \\
\hline
 &  & $3932$ &  &  & $5$ \\
\hline
 &  & $4144$ &  &  & $6$ \\
\hline
  \caption{$X(3350)$ HMRT.}
 \end{longtable}

==> tetraquarks/X_3350_/by_n/fit-_X_X_3350__by_n_fixed_m_n.tex <==
\begin{longtable}[c]{|c|c|c|c|c|c|}
  \hline
  \thead{$State$} & \thead{$M$ \\ $[MeV]$} & \thead{Thry \\ $M$ \\ $[MeV]$} & \thead{$J$} & \thead{Thry \\ $n$} & \thead{Thry \\ $J + n$} \\
  \hline
  \hline
 &  & $1816$ &  &  & $0$ \\
\hline
 &  & $2745$ &  &  & $1$ \\
\hline
$X(3350)$ & $3350$ & $3350$ & $0$ & $2$ & $2$ \\
\hline
$X(3800)$ & $3840$ & $3840$ & $0$ & $3$ & $3$ \\
\hline
 &  & $4264$ &  &  & $4$ \\
\hline
 &  & $4644$ &  &  & $5$ \\
\hline
  \caption{$X(3350)$ HMRT.}
 \end{longtable}

==> tetraquarks/X_3350_/by_n/fit-_X_X_3350__by_n_new_n.tex <==
\begin{longtable}[c]{|c|c|c|c|c|c|}
  \hline
  \thead{$State$} & \thead{$M$ \\ $[MeV]$} & \thead{Thry \\ $M$ \\ $[MeV]$} & \thead{$J$} & \thead{Thry \\ $n$} & \thead{Thry \\ $J + n$} \\
  \hline
  \hline
 &  & $1791$ &  &  & $0$ \\
\hline
 &  & $2703$ &  &  & $1$ \\
\hline
$X(3350)$ & $3350$ & $3350$ & $0$ & $2$ & $2$ \\
\hline
$X(3800)$ & $3840$ & $3840$ & $0$ & $3$ & $3$ \\
\hline
 &  & $4254$ &  &  & $4$ \\
\hline
 &  & $4620$ &  &  & $5$ \\
\hline
  \caption{$X(3350)$ HMRT.}
 \end{longtable}

==> tetraquarks/X_3350_/by_n/fit-_X_X_3350__by_n_prev_n.tex <==
\begin{longtable}[c]{|c|c|c|c|c|c|}
  \hline
  \thead{$State$} & \thead{$M$ \\ $[MeV]$} & \thead{Thry \\ $M$ \\ $[MeV]$} & \thead{$J$} & \thead{Thry \\ $n$} & \thead{Thry \\ $J + n$} \\
  \hline
  \hline
 &  & $2507$ &  &  & $0$ \\
\hline
 &  & $3006$ &  &  & $1$ \\
\hline
$X(3350)$ & $3350$ & $3412$ & $0$ & $2$ & $2$ \\
\hline
$X(3800)$ & $3840$ & $3765$ & $0$ & $3$ & $3$ \\
\hline
 &  & $4082$ &  &  & $4$ \\
\hline
 &  & $4372$ &  &  & $5$ \\
\hline
  \caption{$X(3350)$ HMRT.}
 \end{longtable}

==> tetraquarks/X_3350_/by_n/fit-_X_X_3350__fixed_m_n.tex <==
\begin{table*}[t]
 \centering
  \caption{}
 {\small
 \begin{tabular}{cP{0.1\textwidth}cP{.06\textwidth}cP{.1\textwidth}cP{.05\textwidth}cP{.03\textwidth}cP{.03\textwidth}cP{.03\textwidth}cP{.03\textwidth}|}
  \hline
  \hline
  \thead{$State$} & \thead{$M [MeV]$} & \thead{Thry \\ $M [MeV]$} & \thead{$J$} & \thead{Thry \\ $n$} \\
  \hline
  \hline
 &  & $3644$ &  &  \\
\hline
 &  & $3799$ &  &  \\
\hline
$X(3960)$ & $3955$ & $3945$ & $0$ & $4$ \\
\hline
$X(4140)$ & $4148$ & $4218$ & $1$ & $5$ \\
\hline
$X(4274)$ & $4273$ & $4346$ & $1$ & $6$ \\
\hline
$X(4500)$ & $4506$ & $4346$ & $0$ & $7$ \\
\hline
$X(4630)$ & $4630$ & $4589$ & $1$ & $8$ \\
\hline
$X(4685)$ & $4684$ & $4705$ & $1$ & $9$ \\
\hline
$X(4700)$ & $4704$ & $4705$ & $0$ & $10$ \\
\hline
 &  & $4817$ &  &  \\
\hline
 &  & $4926$ &  &  \\
\hline
 &  & $5032$ &  &  \\
\hline
  \hline
 \end{tabular}
\end{table*}

==> tetraquarks/X_3350_/by_n/fit-_X_X_3350__fixed_slope_n.tex <==
\begin{table}[!ht]
 \centering
 {\small
 \begin{tabular}{cccccc}
  \hline
  \hline
  \thead{$State$} & \thead{$M [MeV]$} & \thead{Thry \\ $M [MeV]$} & \thead{$J$} & \thead{Thry \\ $n$} & \thead{Thry \\ $J + n$} \\
  \hline
  \hline
 &  & $3000$ &  &  & $-4$ \\
\hline
 &  & $3000$ &  &  & $-3$ \\
\hline
 &  & $3000$ &  &  & $-2$ \\
\hline
 &  & $3000$ &  &  & $-1$ \\
\hline
 &  & $3000$ &  &  & $0$ \\
\hline
$X(3350)$ & $3350$ & $3395$ &  &  & $1$ \\
\hline
$X(3800)$ & $3840$ & $3768$ &  &  & $2$ \\
\hline
 &  & $4048$ &  &  & $3$ \\
\hline
 &  & $4284$ &  &  & $4$ \\
\hline
 &  & $4493$ &  &  & $5$ \\
\hline
  \hline
 \end{tabular}}
 \caption{$X(3350)$ Regge trajectory.}
\end{table}

==> tetraquarks/X_3350_/by_n/fit-_X_X_3350__fixed_slope_n_fit_output_all.tex <==
\begin{table}[!ht]
 \centering
 {\small
 \begin{tabular}{ccccccc}
  \hline
  \hline
  \thead{$\chi^{2}_{r}$} & \thead{$\chi^{2}_{hish}$} & \thead{$\alpha^{'}$} & \thead{$a$} & \thead{$m_{1}$} & \thead{$m_{2}$} & \thead{Fit Type} \\
  \hline
  \hline
0.00 & 0.00 & 0.36 & -0.73 & 1.53 & 0.18 & free fit \\
\hline
0.00 & 0.00 & 0.88 & -3.55 & 1.50 & 0.06 & fixed $m_{1}$, $m_{2}$ and $\alpha^{'}$ \\
\hline
2.82 & 0.01 & 0.88 & 0.47 & 2.50 & 0.50 & fixed $\alpha^{'}$ \\
\hline
0.00 & 0.00 & 0.36 & -0.83 & 1.50 & 0.06 & fixed $m_{1}$ and $m_{2}$ \\
\hline
  \hline
 \end{tabular}}
 \caption{}
\end{table}

==> tetraquarks/X_3350_/by_n/fit-_X_X_3350__fixed_slope_n_fit_output_all.tex.tex <==
\begin{table}[!ht]
 \centering
 {\small
 \begin{tabular}{ccccc}
  \hline
  \hline
  \thead{$\chi^{2}_{r}$} & \thead{$\chi^{2}_{hish}$} & \thead{$\alpha^{'}$} & \thead{$a$} & \thead{$m_{1}$} & \thead{$m_{2}$} & \thead{Fit Type} \\
  \hline
  \hline
0.00 & 0.00 & 0.36 & -0.73 & 1.53 & 0.18 & free fit \\
\hline
0.00 & 0.00 & 0.88 & -3.55 & 1.50 & 0.06 & fixed $m_{1}$, $m_{2}$ and $\alpha^{'}$ \\
\hline
2.82 & 0.01 & 0.88 & 0.47 & 2.50 & 0.50 & fixed $\alpha^{'}$ \\
\hline
0.00 & 0.00 & 0.36 & -0.83 & 1.50 & 0.06 & fixed $m_{1}$ and $m_{2}$ \\
\hline
  \hline
 \end{tabular}}
 \caption{}
\end{table}

==> tetraquarks/X_3350_/by_n/fit-_X_X_3350__new_n.tex <==
\begin{table*}[t]
 \centering
  \caption{}
 {\small
 \begin{tabular}{cP{0.1\textwidth}cP{.06\textwidth}cP{.1\textwidth}cP{.05\textwidth}cP{.03\textwidth}cP{.03\textwidth}cP{.03\textwidth}cP{.03\textwidth}|}
  \hline
  \hline
  \thead{$State$} & \thead{$M [MeV]$} & \thead{Thry \\ $M [MeV]$} & \thead{$J$} & \thead{Thry \\ $n$} \\
  \hline
  \hline
 &  & $3643$ &  &  \\
\hline
 &  & $3798$ &  &  \\
\hline
$X(3960)$ & $3955$ & $3945$ & $0$ & $4$ \\
\hline
$X(4140)$ & $4148$ & $4219$ & $1$ & $5$ \\
\hline
$X(4274)$ & $4273$ & $4347$ & $1$ & $6$ \\
\hline
$X(4500)$ & $4506$ & $4347$ & $0$ & $7$ \\
\hline
$X(4630)$ & $4630$ & $4589$ & $1$ & $8$ \\
\hline
$X(4685)$ & $4684$ & $4705$ & $1$ & $9$ \\
\hline
$X(4700)$ & $4704$ & $4705$ & $0$ & $10$ \\
\hline
 &  & $4816$ &  &  \\
\hline
 &  & $4925$ &  &  \\
\hline
 &  & $5031$ &  &  \\
\hline
  \hline
 \end{tabular}
\end{table*}

==> tetraquarks/X_4350_/fit-_X_1j_X_4350_fixed_m_n.tex <==
\begin{longtable}[c]{|c|c|c|c|c|c|}
  \hline
  \thead{$State$} & \thead{$M$ \\ $[MeV]$} & \thead{Thry \\ $M$ \\ $[MeV]$} & \thead{$J$} & \thead{Thry \\ $n$} & \thead{Thry \\ $J + n$} \\
  \hline
  \hline
$X(4350)$ & $4351$ & $4351$ & $1$ & $-1$ & $0$ \\
\hline
$X(4630)$ & $4626$ & $4626$ & $1$ & $0$ & $1$ \\
\hline
 &  & $4875$ &  &  & $2$ \\
\hline
 &  & $5106$ &  &  & $3$ \\
\hline
 &  & $5321$ &  &  & $4$ \\
\hline
 &  & $5523$ &  &  & $5$ \\
\hline
  \caption{$X(4350)$, $X(4630)$ $(n, M^{2})$ HMRT.}
 \end{longtable}

==> tetraquarks/X_4350_/fit-_X_1j_X_4350_new_n.tex <==
\begin{longtable}[c]{|c|c|c|c|c|c|}
  \hline
  \thead{$State$} & \thead{$M$ \\ $[MeV]$} & \thead{Thry \\ $M$ \\ $[MeV]$} & \thead{$J$} & \thead{Thry \\ $n$} & \thead{Thry \\ $J + n$} \\
  \hline
  \hline
$X(4350)$ & $4351$ & $4351$ & $1$ & $-1$ & $0$ \\
\hline
$X(4630)$ & $4626$ & $4626$ & $1$ & $0$ & $1$ \\
\hline
 &  & $4884$ &  &  & $2$ \\
\hline
 &  & $5127$ &  &  & $3$ \\
\hline
 &  & $5358$ &  &  & $4$ \\
\hline
 &  & $5578$ &  &  & $5$ \\
\hline
  \caption{$X(4350)$, $X(4630)$ $(n, M^{2})$ HMRT.}
 \end{longtable}

==> tetraquarks/X_4350_/fit-_X_1j_X_4350_prev_n.tex <==
\begin{longtable}[c]{|c|c|c|c|c|c|}
  \hline
  \thead{$State$} & \thead{$M$ \\ $[MeV]$} & \thead{Thry \\ $M$ \\ $[MeV]$} & \thead{$J$} & \thead{Thry \\ $n$} & \thead{Thry \\ $J + n$} \\
  \hline
  \hline
$X(4350)$ & $4351$ & $4315$ & $1$ & $-1$ & $0$ \\
\hline
$X(4630)$ & $4626$ & $4666$ & $1$ & $0$ & $1$ \\
\hline
 &  & $4976$ &  &  & $2$ \\
\hline
 &  & $5258$ &  &  & $3$ \\
\hline
 &  & $5519$ &  &  & $4$ \\
\hline
 &  & $5763$ &  &  & $5$ \\
\hline
  \caption{$X(4350)$, $X(4630)$ $(n, M^{2})$ HMRT.}
 \end{longtable}

==> tetraquarks/X_6900_/by_n/fit-_T_psi_bs__bs_psi_X_6900_by_n_fixed_slope_n.tex <==
\begin{longtable}[c]{|c|c|c|c|c|c|}
  \hline
  \thead{$State$} & \thead{$M$ \\ $[MeV]$} & \thead{Thry \\ $M$ \\ $[MeV]$} & \thead{$J$} & \thead{Thry \\ $n$} & \thead{Thry \\ $J + n$} \\
  \hline
  \hline
 &  & $5569$ &  &  & $1$ \\
\hline
 &  & $6231$ &  &  & $2$ \\
\hline
$T(6600)_{\psi\psi0}$ & $6552$ & $6611$ &  &  & $3$ \\
\hline
$T(6900)_{\psi\psi0}$ & $6905$ & $6926$ &  &  & $4$ \\
\hline
$T(7300)_{\psi\psi0}$ & $7287$ & $7203$ &  &  & $5$ \\
\hline
 &  & $7455$ &  &  & $6$ \\
\hline
 &  & $7689$ &  &  & $7$ \\
\hline
  \caption{$T_{\psi\psi}$ HMRT.}
 \end{longtable}

==> tetraquarks/X_6900_/by_n/fit-_T_psi_bs__bs_psi_X_6900_by_n_new_n.tex <==
\begin{longtable}[c]{|c|c|c|c|c|c|}
  \hline
  \thead{$State$} & \thead{$M$ \\ $[MeV]$} & \thead{Thry \\ $M$ \\ $[MeV]$} & \thead{$J$} & \thead{Thry \\ $n$} & \thead{Thry \\ $J + n$} \\
  \hline
  \hline
 &  & $5708$ &  &  & $1$ \\
\hline
 &  & $6142$ &  &  & $2$ \\
\hline
$T(6600)_{\psi\psi0}$ & $6552$ & $6544$ &  &  & $3$ \\
\hline
$T(6900)_{\psi\psi0}$ & $6905$ & $6921$ &  &  & $4$ \\
\hline
$T(7300)_{\psi\psi0}$ & $7287$ & $7278$ &  &  & $5$ \\
\hline
 &  & $7617$ &  &  & $6$ \\
\hline
 &  & $7941$ &  &  & $7$ \\
\hline
  \caption{$T_{\psi\psi}$ HMRT.}
 \end{longtable}

==> tetraquarks/X_6900_/by_n/fit-_T_psi_bs__bs_psi_X_6900_by_n_prev_n.tex <==
\begin{longtable}[c]{|c|c|c|c|c|c|}
  \hline
  \thead{$State$} & \thead{$M$ \\ $[MeV]$} & \thead{Thry \\ $M$ \\ $[MeV]$} & \thead{$J$} & \thead{Thry \\ $n$} & \thead{Thry \\ $J + n$} \\
  \hline
  \hline
 &  & $6164$ &  &  & $1$ \\
\hline
 &  & $6432$ &  &  & $2$ \\
\hline
$T(6600)_{psi\\psi0}$ & $6552$ & $6679$ &  &  & $3$ \\
\hline
$T(6900)_{psi\\psi0}$ & $6905$ & $6911$ &  &  & $4$ \\
\hline
$T(7300)_{psi\\psi0}$ & $7287$ & $7129$ &  &  & $5$ \\
\hline
 &  & $7337$ &  &  & $6$ \\
\hline
 &  & $7535$ &  &  & $7$ \\
\hline
  \caption{$T_{\psi\psi}$ HMRT.}
 \end{longtable}

==> tetraquarks/X_6900_/by_n/fit-_T_psi_bs__bs_psi_X_6900_fixed_m_n.tex <==
\begin{table}[!ht]
 \centering
 {\small
 \begin{tabular}{cccccc}
  \hline
  \hline
  \thead{$State$} & \thead{$M [MeV]$} & \thead{Thry \\ $M [MeV]$} & \thead{$J$} & \thead{Thry \\ $n$} & \thead{Thry \\ $J + n$} \\
  \hline
  \hline
 &  & $6000$ &  &  & $-5$ \\
\hline
 &  & $6000$ &  &  & $-4$ \\
\hline
 &  & $6000$ &  &  & $-3$ \\
\hline
 &  & $6000$ &  &  & $-2$ \\
\hline
 &  & $6000$ &  &  & $-1$ \\
\hline
$T(6600)_{\psi\psi0}$ & $6552$ & $6538$ &  &  & $0$ \\
\hline
$T(6900)_{\psi\psi0}$ & $6905$ & $6942$ &  &  & $1$ \\
\hline
$T(7300)_{\psi\psi0}$ & $7287$ & $7265$ &  &  & $2$ \\
\hline
 &  & $7548$ &  &  & $3$ \\
\hline
 &  & $7803$ &  &  & $4$ \\
\hline
 &  & $8040$ &  &  & $5$ \\
\hline
  \hline
 \end{tabular}}
 \caption{$T_{\psi\psi}$ Regge trajectory.}
\end{table}

==> tetraquarks/X_6900_/by_n/fit-_T_psi_bs__bs_psi_X_6900_fixed_slope_n.tex <==
\begin{table}[!ht]
 \centering
 {\small
 \begin{tabular}{cccccc}
  \hline
  \hline
  \thead{$State$} & \thead{$M [MeV]$} & \thead{Thry \\ $M [MeV]$} & \thead{$J$} & \thead{Thry \\ $n$} & \thead{Thry \\ $J + n$} \\
  \hline
  \hline
 &  & $5885$ &  &  & $-5$ \\
\hline
 &  & $5885$ &  &  & $-4$ \\
\hline
 &  & $5885$ &  &  & $-3$ \\
\hline
 &  & $5885$ &  &  & $-2$ \\
\hline
 &  & $5885$ &  &  & $-1$ \\
\hline
$T(6600)_{\psi\psi0}$ & $6552$ & $6542$ &  &  & $0$ \\
\hline
$T(6900)_{\psi\psi0}$ & $6905$ & $6938$ &  &  & $1$ \\
\hline
$T(7300)_{\psi\psi0}$ & $7287$ & $7264$ &  &  & $2$ \\
\hline
 &  & $7551$ &  &  & $3$ \\
\hline
 &  & $7812$ &  &  & $4$ \\
\hline
 &  & $8054$ &  &  & $5$ \\
\hline
  \hline
 \end{tabular}}
 \caption{$T_{\psi\psi}$ Regge trajectory.}
\end{table}

==> tetraquarks/X_6900_/by_n/fit-_T_psi_bs__bs_psi_X_6900_fixed_slope_n_fit_output_all.tex <==
\begin{table}[!ht]
 \centering
 {\small
 \begin{tabular}{ccccccc}
  \hline
  \hline
  \thead{$\chi^{2}_{r}$} & \thead{$\chi^{2}_{hish}$} & \thead{$\alpha^{'}$} & \thead{$a$} & \thead{$m_{1}$} & \thead{$m_{2}$} & \thead{Fit Type} \\
  \hline
  \hline
0.18 & 0.00 & 0.22 & -6.07 & 1.27 & 1.27 & free fit \\
\hline
0.56 & 0.00 & 0.42 & -0.67 & 3.00 & 3.00 & fixed $m_{1}$, $m_{2}$ and $\alpha^{'}$ \\
\hline
0.69 & 0.00 & 0.42 & -0.95 & 2.94 & 2.94 & fixed $\alpha^{'}$ \\
\hline
0.80 & 0.00 & 0.44 & -0.75 & 3.00 & 3.00 & fixed $m_{1}$ and $m_{2}$ \\
\hline
  \hline
 \end{tabular}}
 \caption{}
\end{table}

==> tetraquarks/X_6900_/by_n/fit-_T_psi_bs__bs_psi_X_6900_new_n.tex <==
\begin{table}[!ht]
 \centering
 {\small
 \begin{tabular}{cccccc}
  \hline
  \hline
  \thead{$State$} & \thead{$M [MeV]$} & \thead{Thry \\ $M [MeV]$} & \thead{$J$} & \thead{Thry \\ $n$} & \thead{Thry \\ $J + n$} \\
  \hline
  \hline
 &  & $3921$ &  &  & $-5$ \\
\hline
 &  & $4626$ &  &  & $-4$ \\
\hline
 &  & $5196$ &  &  & $-3$ \\
\hline
 &  & $5692$ &  &  & $-2$ \\
\hline
 &  & $6137$ &  &  & $-1$ \\
\hline
$T(6600)_{\psi\psi0}$ & $6552$ & $6544$ &  &  & $0$ \\
\hline
$T(6900)_{\psi\psi0}$ & $6905$ & $6923$ &  &  & $1$ \\
\hline
$T(7300)_{\psi\psi0}$ & $7287$ & $7278$ &  &  & $2$ \\
\hline
 &  & $7614$ &  &  & $3$ \\
\hline
 &  & $7934$ &  &  & $4$ \\
\hline
 &  & $8239$ &  &  & $5$ \\
\hline
  \hline
 \end{tabular}}
 \caption{$T_{\psi\psi}$ Regge trajectory.}
\end{table}

==> tetraquarks/X_6900_/by_n/fit-_T_psi_bs__bs_psi_X_6900_prev_n.tex <==
\begin{table}[!ht]
 \centering
 {\small
 \begin{tabular}{cccccc}
  \hline
  \hline
  \thead{$State$} & \thead{$M [MeV]$} & \thead{Thry \\ $M [MeV]$} & \thead{$J$} & \thead{Thry \\ $n$} & \thead{Thry \\ $J + n$} \\
  \hline
  \hline
 &  & $6000$ &  &  & $-5$ \\
\hline
 &  & $6000$ &  &  & $-4$ \\
\hline
 &  & $6000$ &  &  & $-3$ \\
\hline
 &  & $6000$ &  &  & $-2$ \\
\hline
 &  & $6000$ &  &  & $-1$ \\
\hline
$T(6600)_{\psi\psi0}$ & $6552$ & $6521$ &  &  & $0$ \\
\hline
$T(6900)_{\psi\psi0}$ & $6905$ & $6948$ &  &  & $1$ \\
\hline
$T(7300)_{\psi\psi0}$ & $7287$ & $7287$ &  &  & $2$ \\
\hline
 &  & $7581$ &  &  & $3$ \\
\hline
 &  & $7847$ &  &  & $4$ \\
\hline
 &  & $8093$ &  &  & $5$ \\
\hline
  \hline
 \end{tabular}}
 \caption{$T_{\psi\psi}$ Regge trajectory.}
\end{table}

==> tetraquarks/Zc/fit-_Z_c_Zc_by_n_fixed_m_n.tex <==
\begin{longtable}[c]{|c|c|c|c|c|c|}
  \hline
  \thead{$State$} & \thead{$M$ \\ $[MeV]$} & \thead{Thry \\ $M$ \\ $[MeV]$} & \thead{$J$} & \thead{Thry \\ $n$} & \thead{Thry \\ $J + n$} \\
  \hline
  \hline
$Z(3900)_{c1}$ & $3887$ & $3887$ & $1$ & $0$ & $1$ \\
\hline
$Z(4200)_{c1}$ & $4196$ & $4197$ & $1$ & $1$ & $2$ \\
\hline
$Z(4430)_{c1}$ & $4478$ & $4477$ & $1$ & $2$ & $3$ \\
\hline
 &  & $4735$ &  &  & $4$ \\
\hline
 &  & $4975$ &  &  & $5$ \\
\hline
 &  & $5201$ &  &  & $6$ \\
\hline
 &  & $5415$ &  &  & $7$ \\
\hline
  \caption{$$Z_{c}$ $(n, M^{2})$$ HMRT.}
 \end{longtable}

==> tetraquarks/Zc/fit-_Z_c_Zc_by_n_new_n.tex <==
\begin{longtable}[c]{|c|c|c|c|c|c|}
  \hline
  \thead{$State$} & \thead{$M$ \\ $[MeV]$} & \thead{Thry \\ $M$ \\ $[MeV]$} & \thead{$J$} & \thead{Thry \\ $n$} & \thead{Thry \\ $J + n$} \\
  \hline
  \hline
$Z(3900)_{c1}$ & $3887$ & $3887$ & $1$ & $0$ & $1$ \\
\hline
$Z(4200)_{c1}$ & $4196$ & $4197$ & $1$ & $1$ & $2$ \\
\hline
$Z(4430)_{c1}$ & $4478$ & $4477$ & $1$ & $2$ & $3$ \\
\hline
 &  & $4735$ &  &  & $4$ \\
\hline
 &  & $4976$ &  &  & $5$ \\
\hline
 &  & $5202$ &  &  & $6$ \\
\hline
 &  & $5417$ &  &  & $7$ \\
\hline
  \caption{$$Z_{c}$ $(n, M^{2})$$ HMRT.}
 \end{longtable}

==> tetraquarks/Zc/fit-_Z_c_Zc_by_n_prev_n.tex <==
\begin{longtable}[c]{|c|c|c|c|c|c|}
  \hline
  \thead{$State$} & \thead{$M$ \\ $[MeV]$} & \thead{Thry \\ $M$ \\ $[MeV]$} & \thead{$J$} & \thead{Thry \\ $n$} & \thead{Thry \\ $J + n$} \\
  \hline
  \hline
$Z(3900)_{c1}$ & $3887$ & $3850$ & $1$ & $0$ & $1$ \\
\hline
$Z(4200)_{c1}$ & $4196$ & $4203$ & $1$ & $1$ & $2$ \\
\hline
$Z(4430)_{c1}$ & $4478$ & $4517$ & $1$ & $2$ & $3$ \\
\hline
 &  & $4804$ &  &  & $4$ \\
\hline
 &  & $5069$ &  &  & $5$ \\
\hline
 &  & $5318$ &  &  & $6$ \\
\hline
 &  & $5552$ &  &  & $7$ \\
\hline
  \caption{$$Z_{c}$ $(n, M^{2})$$ HMRT.}
 \end{longtable}

==> tetraquarks/Zc_3900_/by_n_one_point/fit-_Z_c_Zc_3900__tetra_one_by_n.tex <==
\begin{longtable}[c]{|c|c|c|c|c|c|}
  \hline
  \thead{$State$} & \thead{$M$ \\ $[MeV]$} & \thead{Thry \\ $M$ \\ $[MeV]$} & \thead{$J$} & \thead{Thry \\ $n$} & \thead{Thry \\ $J + n$} \\
  \hline
  \hline
$Z(3900)_{c1}$ & $3887$ & $3887$ & $1$ & $0$ & $1$ \\
\hline
 &  & $4236$ &  &  & $2$ \\
\hline
 &  & $4547$ &  &  & $3$ \\
\hline
 &  & $4831$ &  &  & $4$ \\
\hline
 &  & $5095$ &  &  & $5$ \\
\hline
  \caption{$Z_{c}(3900)$ $(n, M^{2})$ HMRT.} \label{table:Zc_3900_n_HMRT}
 \end{longtable}

==> tetraquarks/Zc_4200_/by_n_one_point/fit-_Z_c_Zc_4200__tetra_one_by_n.tex <==
\begin{longtable}[c]{|c|c|c|c|c|c|}
  \hline
  \thead{$State$} & \thead{$M$ \\ $[MeV]$} & \thead{Thry \\ $M$ \\ $[MeV]$} & \thead{$J$} & \thead{Thry \\ $n$} & \thead{Thry \\ $J + n$} \\
  \hline
  \hline
 &  & $3427$ &  &  & $0$ \\
\hline
 &  & $3842$ &  &  & $1$ \\
\hline
$Z(4200)_{c1}$ & $4196$ & $4196$ & $1$ & $1$ & $2$ \\
\hline
 &  & $4511$ &  &  & $3$ \\
\hline
 &  & $4798$ &  &  & $4$ \\
\hline
  \caption{$Z_{c}(4200)$ $(n, M^{2})$ HMRT.} \label{table:Zc_4200_n_HMRT}
 \end{longtable}

==> tetraquarks/Zc_4430_/by_n_one_point/fit-_Z_c_Zc_4430__tetra_one_by_n.tex <==
\begin{longtable}[c]{|c|c|c|c|c|c|}
  \hline
  \thead{$State$} & \thead{$M$ \\ $[MeV]$} & \thead{Thry \\ $M$ \\ $[MeV]$} & \thead{$J$} & \thead{Thry \\ $n$} & \thead{Thry \\ $J + n$} \\
  \hline
  \hline
 &  & $3800$ &  &  & $1$ \\
\hline
 &  & $4159$ &  &  & $2$ \\
\hline
$Z(4430)_{c1}$ & $4478$ & $4478$ & $1$ & $2$ & $3$ \\
\hline
 &  & $4768$ &  &  & $4$ \\
\hline
 &  & $5036$ &  &  & $5$ \\
\hline
  \caption{$Z_{c}(4430)$ $(n, M^{2})$ HMRT.} \label{table:Zc_4430_n_HMRT}
 \end{longtable}

==> tetraquarks/Zcs/fit-_Z__cs_Zcs_by_n_fixed_slope_n.tex <==
\begin{longtable}[c]{|c|c|c|c|c|c|}
  \hline
  \thead{$State$} & \thead{$M$ \\ $[MeV]$} & \thead{Thry \\ $M$ \\ $[MeV]$} & \thead{$J$} & \thead{Thry \\ $n$} & \thead{Thry \\ $J + n$} \\
  \hline
  \hline
$Z(4000)^{+}_{cs1}$ & $4003$ & $3942$ & $1$ & $0$ & $1$ \\
\hline
$Z(4220)^{+}_{cs1}$ & $4216$ & $4282$ & $1$ & $1$ & $2$ \\
\hline
 &  & $4587$ &  &  & $3$ \\
\hline
 &  & $4868$ &  &  & $4$ \\
\hline
 &  & $5128$ &  &  & $5$ \\
\hline
 &  & $5372$ &  &  & $6$ \\
\hline
  \caption{$Z_{cs}$ $(n, M^{2})$ HMRT.}
 \end{longtable}

==> tetraquarks/Zcs/fit-_Z__cs_Zcs_by_n_new_n.tex <==
\begin{longtable}[c]{|c|c|c|c|c|c|}
  \hline
  \thead{$State$} & \thead{$M$ \\ $[MeV]$} & \thead{Thry \\ $M$ \\ $[MeV]$} & \thead{$J$} & \thead{Thry \\ $n$} & \thead{Thry \\ $J + n$} \\
  \hline
  \hline
$Z(4000)^{+}_{cs1}$ & $4003$ & $4003$ & $1$ & $0$ & $1$ \\
\hline
$Z(4220)^{+}_{cs1}$ & $4216$ & $4216$ & $1$ & $1$ & $2$ \\
\hline
 &  & $4414$ &  &  & $3$ \\
\hline
 &  & $4600$ &  &  & $4$ \\
\hline
 &  & $4775$ &  &  & $5$ \\
\hline
 &  & $4943$ &  &  & $6$ \\
\hline
  \caption{$Z_{cs}$ $(n, M^{2})$ HMRT.}
 \end{longtable}

==> tetraquarks/Zcs/fit-_Z__cs_Zcs_by_n_prev_n.tex <==
\begin{longtable}[c]{|c|c|c|c|c|c|}
  \hline
  \thead{$State$} & \thead{$M$ \\ $[MeV]$} & \thead{Thry \\ $M$ \\ $[MeV]$} & \thead{$J$} & \thead{Thry \\ $n$} & \thead{Thry \\ $J + n$} \\
  \hline
  \hline
$Z(4000)^{+}_{cs1}$ & $4003$ & $3927$ & $1$ & $0$ & $1$ \\
\hline
$Z(4220)^{+}_{cs1}$ & $4216$ & $4300$ & $1$ & $1$ & $2$ \\
\hline
 &  & $4626$ &  &  & $3$ \\
\hline
 &  & $4921$ &  &  & $4$ \\
\hline
 &  & $5192$ &  &  & $5$ \\
\hline
 &  & $5445$ &  &  & $6$ \\
\hline
  \caption{$Z_{cs}$ $(n, M^{2})$ HMRT.}
 \end{longtable}

==> tetraquarks/predictions/bc-bb/spectrum.tex <==
\setlength\LTleft{-1.2cm}
\setlength\LTpre{0.5cm}
{\small\tabcolsep=1pt\footnotesize{\begin{longtable}[!c]{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
  \hline
  \thead{$\#$} & \thead{Candi-\\dates} & \thead{$J^{PC}$} & \thead{Quarks} & \thead{Thry \\ Width \\ $[MeV]$} & \thead{Mesons \\ Pair} & \thead{Meson \\ Threshold \\ $[MeV]$} & \thead{Baryon \\ Anti-\\baryon} & \thead{Baryonic \\ Threshold \\ $[MeV]$} & \thead{$J$ \\ Spec} & \thead{$n$ \\ Spec} & \thead{$a_{T_{j}}$ \\ $a_{T_{n}}$} & \thead{Thry \\ $J + n$} & \thead{Gen-\\uine} \\
  \hline
  \hline
1 & \makecell{} & \makecell{} & $b\bar{b}c\bar{b}$ &  & \makecell{$\eta_{b}(1S) B^{+}_{c}$} & \makecell{$15673$} & \makecell{$\Xi^{+}_{bc} \bar{\Xi}^{0}_{bb}$ \\ $\Xi^{0}_{bc} \bar{\Xi}^{+}_{bb}$ \\ $\Omega^{0}_{bc} \bar{\Omega}^{+}_{bb}$} & \makecell{ \\  \\ } & \makecell{$15683-15723$\\$15894-15927$\\$16074-16103$\\$16235-16262$\\$16384-16409$\\$16523-16547$\\$16655-16677$\\$16781-16802$\\$16901-16921$\\$17016-17036$\\$17128-17147$\\$17236-17255$} & \makecell{$15683-15723$\\$15977-16008$\\$16218-16245$\\$16432-16456$\\$16626-16649$\\$16808-16829$\\$16978-16998$\\$17140-17159$\\$17295-17313$\\$17444-17461$\\$17587-17604$\\$17726-17742$} & \makecell{\makecell{$-1.4$-$-1.3$} \\ \makecell{$-0.99$-$-0.87$}} & \makecell{} & $*$ \\
\hline
 \caption{Tetraquark predicted configurations and thresholds.} \label{table:charm_tetraquarks_predictions}
\end{longtable}}\normalsize}

==> tetraquarks/predictions/bc-bb/thresholds.tex <==
\begin{longtable}[c]{|c|c|c|c|c|c|}
  \hline
  \thead{Thry \\ Width \\ $[MeV]$} & \thead{Mesons \\ Pair} & \thead{Meson \\ Threshold \\ $[MeV]$} & \thead{Baryon \\ Anti-\\baryon} & \thead{Baryonic \\ Threshold \\ $[MeV]$} & \thead{Genuine} \\
  \hline
  \hline
 & \makecell{$\eta_{b}(1S) B^{+}_{c}$} & \makecell{$15673$} & \makecell{$\Xi^{+}_{bc} \bar{\Xi}^{0}_{bb}$ \\ $\Xi^{0}_{bc} \bar{\Xi}^{+}_{bb}$ \\ $\Omega^{0}_{bc} \bar{\Omega}^{+}_{bb}$} & \makecell{ \\  \\ } & $*$ \\
\hline
  \caption{$T_{b\bar{b}c\bar{b}}$ thresholds.} \label{table:Tbcbb_thresholds}
 \end{longtable}

==> tetraquarks/predictions/bc-bc/spectrum.tex <==
\setlength\LTleft{-1.2cm}
\setlength\LTpre{0.5cm}
{\small\tabcolsep=1pt\footnotesize{\begin{longtable}[!c]{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
  \hline
  \thead{$\#$} & \thead{Candi-\\dates} & \thead{$J^{PC}$} & \thead{Quarks} & \thead{Thry \\ Width \\ $[MeV]$} & \thead{Mesons \\ Pair} & \thead{Meson \\ Threshold \\ $[MeV]$} & \thead{Baryon \\ Anti-\\baryon} & \thead{Baryonic \\ Threshold \\ $[MeV]$} & \thead{$J$ \\ Spec} & \thead{$n$ \\ Spec} & \thead{$a_{T_{j}}$ \\ $a_{T_{n}}$} & \thead{Thry \\ $J + n$} & \thead{Gen-\\uine} \\
  \hline
  \hline
1 & \makecell{} & \makecell{} & $b\bar{b}c\bar{c}$ &  & \makecell{$\eta_{b}(1S) \eta_{c}(1S)$ \\ $\bar{B}^{-}_{c} B^{+}_{c}$} & \makecell{$12383$ \\ $12548$} & \makecell{$\Xi^{+}_{bc} \bar{\Xi}^{-}_{bc}$ \\ $\Xi^{0}_{bc} \bar{\Xi}^{0}_{bc}$ \\ $\Omega^{0}_{bc} \bar{\Omega}^{0}_{bc}$} & \makecell{ \\  \\ } & \makecell{$12393-12433$\\$12580-12616$\\$12749-12782$\\$12905-12936$\\$13052-13081$\\$13191-13218$\\$13323-13349$\\$13450-13475$\\$13572-13597$\\$13691-13714$\\$13805-13828$\\$13916-13939$} & \makecell{$12393-12433$\\$12657-12691$\\$12888-12919$\\$13099-13127$\\$13294-13321$\\$13478-13503$\\$13652-13676$\\$13818-13841$\\$13977-13999$\\$14131-14152$\\$14279-14300$\\$14423-14443$} & \makecell{\makecell{$-2.7$-$-2.5$} \\ \makecell{$-1.9$-$-1.7$}} & \makecell{} & $*$ \\
\hline
 \caption{Tetraquark predicted configurations and thresholds.} \label{table:charm_tetraquarks_predictions}
\end{longtable}}\normalsize}

==> tetraquarks/predictions/bc-bc/thresholds.tex <==
\begin{longtable}[c]{|c|c|c|c|c|c|}
  \hline
  \thead{Thry \\ Width \\ $[MeV]$} & \thead{Mesons \\ Pair} & \thead{Meson \\ Threshold \\ $[MeV]$} & \thead{Baryon \\ Anti-\\baryon} & \thead{Baryonic \\ Threshold \\ $[MeV]$} & \thead{Genuine} \\
  \hline
  \hline
 & \makecell{$\eta_{b}(1S) \eta_{c}(1S)$ \\ $\bar{B}^{-}_{c} B^{+}_{c}$} & \makecell{$12383$ \\ $12548$} & \makecell{$\Xi^{+}_{bc} \bar{\Xi}^{-}_{bc}$ \\ $\Xi^{0}_{bc} \bar{\Xi}^{0}_{bc}$ \\ $\Omega^{0}_{bc} \bar{\Omega}^{0}_{bc}$} & \makecell{ \\  \\ } & $*$ \\
\hline
  \caption{$T_{b\bar{b}c\bar{c}}$ thresholds.} \label{table:Tbcbc_thresholds}
 \end{longtable}

==> tetraquarks/predictions/bc-bd/spectrum.tex <==
\setlength\LTleft{-1.2cm}
\setlength\LTpre{0.5cm}
{\small\tabcolsep=1pt\footnotesize{\begin{longtable}[!c]{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
  \hline
  \thead{$\#$} & \thead{Candi-\\dates} & \thead{$J^{PC}$} & \thead{Quarks} & \thead{Thry \\ Width \\ $[MeV]$} & \thead{Mesons \\ Pair} & \thead{Meson \\ Threshold \\ $[MeV]$} & \thead{Baryon \\ Anti-\\baryon} & \thead{Baryonic \\ Threshold \\ $[MeV]$} & \thead{$J$ \\ Spec} & \thead{$n$ \\ Spec} & \thead{$a_{T_{j}}$ \\ $a_{T_{n}}$} & \thead{Thry \\ $J + n$} & \thead{Gen-\\uine} \\
  \hline
  \hline
1 & \makecell{} & \makecell{} & $b\bar{b}c\bar{d}$ &  & \makecell{$\eta_{b}(1S) D^{+}$ \\ $B^{0} B^{+}_{c}$} & \makecell{$11269$ \\ $11554$} & \makecell{$\Xi^{+}_{bc} \bar{\Sigma}^{0}_{b}$ \\ $\Xi^{0}_{bc} \bar{\Sigma}^{+}_{b}$ \\ $\Omega^{0}_{bc} \bar{\Xi}^{+}_{b}$} & \makecell{ \\  \\ } & \makecell{$11279-11319$\\$11477-11513$\\$11655-11687$\\$11819-11849$\\$11972-12001$\\$12117-12144$\\$12255-12281$\\$12387-12412$\\$12514-12538$\\$12637-12660$\\$12755-12778$\\$12871-12892$} & \makecell{$11279-11319$\\$11558-11592$\\$11801-11832$\\$12021-12049$\\$12225-12251$\\$12416-12440$\\$12596-12619$\\$12768-12791$\\$12933-12955$\\$13092-13113$\\$13245-13265$\\$13394-13413$} & \makecell{\makecell{$-2.5$-$-2.3$} \\ \makecell{$-1.7$-$-1.6$}} & \makecell{} & $*$ \\
\hline
 \caption{Tetraquark predicted configurations and thresholds.} \label{table:charm_tetraquarks_predictions}
\end{longtable}}\normalsize}

==> tetraquarks/predictions/bc-bd/thresholds.tex <==
\begin{longtable}[c]{|c|c|c|c|c|c|}
  \hline
  \thead{Thry \\ Width \\ $[MeV]$} & \thead{Mesons \\ Pair} & \thead{Meson \\ Threshold \\ $[MeV]$} & \thead{Baryon \\ Anti-\\baryon} & \thead{Baryonic \\ Threshold \\ $[MeV]$} & \thead{Genuine} \\
  \hline
  \hline
 & \makecell{$\eta_{b}(1S) D^{+}$ \\ $B^{0} B^{+}_{c}$} & \makecell{$11269$ \\ $11554$} & \makecell{$\Xi^{+}_{bc} \bar{\Sigma}^{0}_{b}$ \\ $\Xi^{0}_{bc} \bar{\Sigma}^{+}_{b}$ \\ $\Omega^{0}_{bc} \bar{\Xi}^{+}_{b}$} & \makecell{ \\  \\ } & $*$ \\
\hline
  \caption{$T_{b\bar{b}c\bar{d}}$ thresholds.} \label{table:Tbcbd_thresholds}
 \end{longtable}

==> tetraquarks/predictions/bc-bs/spectrum.tex <==
\setlength\LTleft{-1.2cm}
\setlength\LTpre{0.5cm}
{\small\tabcolsep=1pt\footnotesize{\begin{longtable}[!c]{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
  \hline
  \thead{$\#$} & \thead{Candi-\\dates} & \thead{$J^{PC}$} & \thead{Quarks} & \thead{Thry \\ Width \\ $[MeV]$} & \thead{Mesons \\ Pair} & \thead{Meson \\ Threshold \\ $[MeV]$} & \thead{Baryon \\ Anti-\\baryon} & \thead{Baryonic \\ Threshold \\ $[MeV]$} & \thead{$J$ \\ Spec} & \thead{$n$ \\ Spec} & \thead{$a_{T_{j}}$ \\ $a_{T_{n}}$} & \thead{Thry \\ $J + n$} & \thead{Gen-\\uine} \\
  \hline
  \hline
1 & \makecell{} & \makecell{} & $b\bar{b}c\bar{s}$ &  & \makecell{$\eta_{b}(1S) D^{+}_{s}$ \\ $B^{0}_{s} B^{+}_{c}$} & \makecell{$11367$ \\ $11641$} & \makecell{$\Xi^{+}_{bc} \bar{\Xi}^{0}_{b}$ \\ $\Xi^{0}_{bc} \bar{\Xi}^{+}_{b}$ \\ $\Omega^{0}_{bc} \bar{\Omega}^{+}_{b}$} & \makecell{ \\  \\ } & \makecell{$11377-11417$\\$11608-11641$\\$11805-11834$\\$11981-12008$\\$12144-12169$\\$12296-12319$\\$12440-12462$\\$12576-12598$\\$12707-12728$\\$12833-12853$\\$12955-12974$\\$13073-13091$} & \makecell{$11377-11417$\\$11699-11730$\\$11963-11990$\\$12196-12220$\\$12408-12431$\\$12606-12627$\\$12792-12812$\\$12968-12987$\\$13136-13155$\\$13298-13315$\\$13454-13470$\\$13604-13620$} & \makecell{\makecell{$-1.4$-$-1.3$} \\ \makecell{$-0.98$-$-0.87$}} & \makecell{} & $*$ \\
\hline
 \caption{Tetraquark predicted configurations and thresholds.} \label{table:charm_tetraquarks_predictions}
\end{longtable}}\normalsize}

==> tetraquarks/predictions/bc-bs/thresholds.tex <==
\begin{longtable}[c]{|c|c|c|c|c|c|}
  \hline
  \thead{Thry \\ Width \\ $[MeV]$} & \thead{Mesons \\ Pair} & \thead{Meson \\ Threshold \\ $[MeV]$} & \thead{Baryon \\ Anti-\\baryon} & \thead{Baryonic \\ Threshold \\ $[MeV]$} & \thead{Genuine} \\
  \hline
  \hline
 & \makecell{$\eta_{b}(1S) D^{+}_{s}$ \\ $B^{0}_{s} B^{+}_{c}$} & \makecell{$11367$ \\ $11641$} & \makecell{$\Xi^{+}_{bc} \bar{\Xi}^{0}_{b}$ \\ $\Xi^{0}_{bc} \bar{\Xi}^{+}_{b}$ \\ $\Omega^{0}_{bc} \bar{\Omega}^{+}_{b}$} & \makecell{ \\  \\ } & $*$ \\
\hline
  \caption{$T_{b\bar{b}c\bar{s}}$ thresholds.} \label{table:Tbcbs_thresholds}
 \end{longtable}

==> tetraquarks/predictions/bc-bu/spectrum.tex <==
\setlength\LTleft{-1.2cm}
\setlength\LTpre{0.5cm}
{\small\tabcolsep=1pt\footnotesize{\begin{longtable}[!c]{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
  \hline
  \thead{$\#$} & \thead{Candi-\\dates} & \thead{$J^{PC}$} & \thead{Quarks} & \thead{Thry \\ Width \\ $[MeV]$} & \thead{Mesons \\ Pair} & \thead{Meson \\ Threshold \\ $[MeV]$} & \thead{Baryon \\ Anti-\\baryon} & \thead{Baryonic \\ Threshold \\ $[MeV]$} & \thead{$J$ \\ Spec} & \thead{$n$ \\ Spec} & \thead{$a_{T_{j}}$ \\ $a_{T_{n}}$} & \thead{Thry \\ $J + n$} & \thead{Gen-\\uine} \\
  \hline
  \hline
1 & \makecell{} & \makecell{} & $b\bar{b}c\bar{u}$ &  & \makecell{$\eta_{b}(1S) D^{0}$ \\ $B^{+} B^{+}_{c}$} & \makecell{$11264$ \\ $11553$} & \makecell{$\Xi^{+}_{bc} \bar{\Sigma}^{-}_{b}$ \\ $\Xi^{0}_{bc} \bar{\Sigma}^{0}_{b}$ \\ $\Omega^{0}_{bc} \bar{\Xi}^{0}_{b}$} & \makecell{ \\  \\ } & \makecell{$11274-11314$\\$11473-11508$\\$11651-11683$\\$11815-11845$\\$11969-11997$\\$12114-12141$\\$12252-12277$\\$12384-12409$\\$12511-12535$\\$12634-12657$\\$12753-12775$\\$12868-12890$} & \makecell{$11274-11314$\\$11554-11588$\\$11798-11828$\\$12018-12046$\\$12222-12248$\\$12413-12437$\\$12593-12617$\\$12766-12788$\\$12931-12952$\\$13089-13110$\\$13243-13263$\\$13391-13411$} & \makecell{\makecell{$-2.5$-$-2.3$} \\ \makecell{$-1.7$-$-1.6$}} & \makecell{} & $*$ \\
\hline
 \caption{Tetraquark predicted configurations and thresholds.} \label{table:charm_tetraquarks_predictions}
\end{longtable}}\normalsize}

==> tetraquarks/predictions/bc-bu/thresholds.tex <==
\begin{longtable}[c]{|c|c|c|c|c|c|}
  \hline
  \thead{Thry \\ Width \\ $[MeV]$} & \thead{Mesons \\ Pair} & \thead{Meson \\ Threshold \\ $[MeV]$} & \thead{Baryon \\ Anti-\\baryon} & \thead{Baryonic \\ Threshold \\ $[MeV]$} & \thead{Genuine} \\
  \hline
  \hline
 & \makecell{$\eta_{b}(1S) D^{0}$ \\ $B^{+} B^{+}_{c}$} & \makecell{$11264$ \\ $11553$} & \makecell{$\Xi^{+}_{bc} \bar{\Sigma}^{-}_{b}$ \\ $\Xi^{0}_{bc} \bar{\Sigma}^{0}_{b}$ \\ $\Omega^{0}_{bc} \bar{\Xi}^{0}_{b}$} & \makecell{ \\  \\ } & $*$ \\
\hline
  \caption{$T_{b\bar{b}c\bar{u}}$ thresholds.} \label{table:Tbcbu_thresholds}
 \end{longtable}

==> tetraquarks/predictions/bc-cd/spectrum.tex <==
\setlength\LTleft{-1.2cm}
\setlength\LTpre{0.5cm}
{\small\tabcolsep=1pt\footnotesize{\begin{longtable}[!c]{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
  \hline
  \thead{$\#$} & \thead{Candi-\\dates} & \thead{$J^{PC}$} & \thead{Quarks} & \thead{Thry \\ Width \\ $[MeV]$} & \thead{Mesons \\ Pair} & \thead{Meson \\ Threshold \\ $[MeV]$} & \thead{Baryon \\ Anti-\\baryon} & \thead{Baryonic \\ Threshold \\ $[MeV]$} & \thead{$J$ \\ Spec} & \thead{$n$ \\ Spec} & \thead{$a_{T_{j}}$ \\ $a_{T_{n}}$} & \thead{Thry \\ $J + n$} & \thead{Gen-\\uine} \\
  \hline
  \hline
1 & \makecell{} & \makecell{} & $b\bar{c}c\bar{d}$ &  & \makecell{$\bar{B}^{-}_{c} D^{+}$ \\ $B^{0} \eta_{c}(1S)$} & \makecell{$8144$ \\ $8264$} & \makecell{$\Xi^{+}_{bc} \bar{\Lambda}^{-}_{c}$ \\ $\Xi^{0}_{bc} \bar{\Sigma}^{0}_{c}$ \\ $\Omega^{0}_{bc} \bar{\Xi}^{0}_{c}$} & \makecell{ \\  \\ } & \makecell{$8154-8194$\\$8377-8413$\\$8579-8612$\\$8767-8798$\\$8942-8971$\\$9108-9136$\\$9266-9292$\\$9417-9442$\\$9561-9586$\\$9701-9724$\\$9836-9859$\\$9967-9989$} & \makecell{$8154-8194$\\$8469-8504$\\$8746-8778$\\$8998-9027$\\$9231-9258$\\$9449-9474$\\$9655-9679$\\$9851-9873$\\$10038-10059$\\$10217-10238$\\$10390-10410$\\$10557-10576$} & \makecell{\makecell{$-3.4$-$-3.2$} \\ \makecell{$-2.4$-$-2.2$}} & \makecell{} & $*$ \\
\hline
 \caption{Tetraquark predicted configurations and thresholds.} \label{table:charm_tetraquarks_predictions}
\end{longtable}}\normalsize}

==> tetraquarks/predictions/bc-cd/thresholds.tex <==
\begin{longtable}[c]{|c|c|c|c|c|c|}
  \hline
  \thead{Thry \\ Width \\ $[MeV]$} & \thead{Mesons \\ Pair} & \thead{Meson \\ Threshold \\ $[MeV]$} & \thead{Baryon \\ Anti-\\baryon} & \thead{Baryonic \\ Threshold \\ $[MeV]$} & \thead{Genuine} \\
  \hline
  \hline
 & \makecell{$\bar{B}^{-}_{c} D^{+}$ \\ $B^{0} \eta_{c}(1S)$} & \makecell{$8144$ \\ $8264$} & \makecell{$\Xi^{+}_{bc} \bar{\Lambda}^{-}_{c}$ \\ $\Xi^{0}_{bc} \bar{\Sigma}^{0}_{c}$ \\ $\Omega^{0}_{bc} \bar{\Xi}^{0}_{c}$} & \makecell{ \\  \\ } & $*$ \\
\hline
  \caption{$T_{b\bar{c}c\bar{d}}$ thresholds.} \label{table:Tbccd_thresholds}
 \end{longtable}

==> tetraquarks/predictions/bc-cs/spectrum.tex <==
\setlength\LTleft{-1.2cm}
\setlength\LTpre{0.5cm}
{\small\tabcolsep=1pt\footnotesize{\begin{longtable}[!c]{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
  \hline
  \thead{$\#$} & \thead{Candi-\\dates} & \thead{$J^{PC}$} & \thead{Quarks} & \thead{Thry \\ Width \\ $[MeV]$} & \thead{Mesons \\ Pair} & \thead{Meson \\ Threshold \\ $[MeV]$} & \thead{Baryon \\ Anti-\\baryon} & \thead{Baryonic \\ Threshold \\ $[MeV]$} & \thead{$J$ \\ Spec} & \thead{$n$ \\ Spec} & \thead{$a_{T_{j}}$ \\ $a_{T_{n}}$} & \thead{Thry \\ $J + n$} & \thead{Gen-\\uine} \\
  \hline
  \hline
1 & \makecell{} & \makecell{} & $b\bar{c}c\bar{s}$ &  & \makecell{$\bar{B}^{-}_{c} D^{+}_{s}$ \\ $B^{0}_{s} \eta_{c}(1S)$} & \makecell{$8242$ \\ $8351$} & \makecell{$\Xi^{+}_{bc} \bar{\Xi}^{-}_{c}$ \\ $\Xi^{0}_{bc} \bar{\Xi}^{0}_{c}$ \\ $\Omega^{0}_{bc} \bar{\Omega}^{0}_{c}$} & \makecell{ \\  \\ } & \makecell{$8252-8292$\\$8488-8523$\\$8699-8731$\\$8892-8922$\\$9072-9099$\\$9240-9266$\\$9400-9425$\\$9553-9577$\\$9699-9722$\\$9840-9862$\\$9976-9997$\\$10107-10128$} & \makecell{$8252-8292$\\$8584-8618$\\$8871-8901$\\$9129-9156$\\$9365-9391$\\$9586-9609$\\$9793-9816$\\$9990-10012$\\$10178-10199$\\$10358-10378$\\$10532-10550$\\$10699-10717$} & \makecell{\makecell{$-2.6$-$-2.4$} \\ \makecell{$-1.8$-$-1.7$}} & \makecell{} & $*$ \\
\hline
 \caption{Tetraquark predicted configurations and thresholds.} \label{table:charm_tetraquarks_predictions}
\end{longtable}}\normalsize}

==> tetraquarks/predictions/bc-cs/thresholds.tex <==
\begin{longtable}[c]{|c|c|c|c|c|c|}
  \hline
  \thead{Thry \\ Width \\ $[MeV]$} & \thead{Mesons \\ Pair} & \thead{Meson \\ Threshold \\ $[MeV]$} & \thead{Baryon \\ Anti-\\baryon} & \thead{Baryonic \\ Threshold \\ $[MeV]$} & \thead{Genuine} \\
  \hline
  \hline
 & \makecell{$\bar{B}^{-}_{c} D^{+}_{s}$ \\ $B^{0}_{s} \eta_{c}(1S)$} & \makecell{$8242$ \\ $8351$} & \makecell{$\Xi^{+}_{bc} \bar{\Xi}^{-}_{c}$ \\ $\Xi^{0}_{bc} \bar{\Xi}^{0}_{c}$ \\ $\Omega^{0}_{bc} \bar{\Omega}^{0}_{c}$} & \makecell{ \\  \\ } & $*$ \\
\hline
  \caption{$T_{b\bar{c}c\bar{s}}$ thresholds.} \label{table:Tbccs_thresholds}
 \end{longtable}

==> tetraquarks/predictions/bc-cu/spectrum.tex <==
\setlength\LTleft{-1.2cm}
\setlength\LTpre{0.5cm}
{\small\tabcolsep=1pt\footnotesize{\begin{longtable}[!c]{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
  \hline
  \thead{$\#$} & \thead{Candi-\\dates} & \thead{$J^{PC}$} & \thead{Quarks} & \thead{Thry \\ Width \\ $[MeV]$} & \thead{Mesons \\ Pair} & \thead{Meson \\ Threshold \\ $[MeV]$} & \thead{Baryon \\ Anti-\\baryon} & \thead{Baryonic \\ Threshold \\ $[MeV]$} & \thead{$J$ \\ Spec} & \thead{$n$ \\ Spec} & \thead{$a_{T_{j}}$ \\ $a_{T_{n}}$} & \thead{Thry \\ $J + n$} & \thead{Gen-\\uine} \\
  \hline
  \hline
1 & \makecell{} & \makecell{} & $b\bar{c}c\bar{u}$ &  & \makecell{$\bar{B}^{-}_{c} D^{0}$ \\ $B^{+} \eta_{c}(1S)$} & \makecell{$8139$ \\ $8263$} & \makecell{$\Xi^{+}_{bc} \bar{\Sigma}^{--}_{c}$ \\ $\Xi^{0}_{bc} \bar{\Lambda}^{-}_{c}$ \\ $\Omega^{0}_{bc} \bar{\Xi}^{-}_{c}$} & \makecell{ \\  \\ } & \makecell{$8149-8189$\\$8372-8408$\\$8575-8608$\\$8763-8794$\\$8939-8968$\\$9105-9132$\\$9262-9289$\\$9413-9439$\\$9558-9583$\\$9698-9722$\\$9833-9856$\\$9964-9986$} & \makecell{$8149-8189$\\$8465-8499$\\$8743-8774$\\$8995-9023$\\$9228-9255$\\$9446-9471$\\$9652-9676$\\$9848-9870$\\$10035-10057$\\$10215-10235$\\$10387-10408$\\$10555-10574$} & \makecell{\makecell{$-3.4$-$-3.2$} \\ \makecell{$-2.3$-$-2.2$}} & \makecell{} & $*$ \\
\hline
 \caption{Tetraquark predicted configurations and thresholds.} \label{table:charm_tetraquarks_predictions}
\end{longtable}}\normalsize}

==> tetraquarks/predictions/bc-cu/thresholds.tex <==
\begin{longtable}[c]{|c|c|c|c|c|c|}
  \hline
  \thead{Thry \\ Width \\ $[MeV]$} & \thead{Mesons \\ Pair} & \thead{Meson \\ Threshold \\ $[MeV]$} & \thead{Baryon \\ Anti-\\baryon} & \thead{Baryonic \\ Threshold \\ $[MeV]$} & \thead{Genuine} \\
  \hline
  \hline
 & \makecell{$\bar{B}^{-}_{c} D^{0}$ \\ $B^{+} \eta_{c}(1S)$} & \makecell{$8139$ \\ $8263$} & \makecell{$\Xi^{+}_{bc} \bar{\Sigma}^{--}_{c}$ \\ $\Xi^{0}_{bc} \bar{\Lambda}^{-}_{c}$ \\ $\Omega^{0}_{bc} \bar{\Xi}^{-}_{c}$} & \makecell{ \\  \\ } & $*$ \\
\hline
  \caption{$T_{b\bar{c}c\bar{u}}$ thresholds.} \label{table:Tbccu_thresholds}
 \end{longtable}

==> tetraquarks/predictions/bc-dd/spectrum.tex <==
\setlength\LTleft{-1.2cm}
\setlength\LTpre{0.5cm}
{\small\tabcolsep=1pt\footnotesize{\begin{longtable}[!c]{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
  \hline
  \thead{$\#$} & \thead{Candi-\\dates} & \thead{$J^{PC}$} & \thead{Quarks} & \thead{Thry \\ Width \\ $[MeV]$} & \thead{Mesons \\ Pair} & \thead{Meson \\ Threshold \\ $[MeV]$} & \thead{Baryon \\ Anti-\\baryon} & \thead{Baryonic \\ Threshold \\ $[MeV]$} & \thead{$J$ \\ Spec} & \thead{$n$ \\ Spec} & \thead{$a_{T_{j}}$ \\ $a_{T_{n}}$} & \thead{Thry \\ $J + n$} & \thead{Gen-\\uine} \\
  \hline
  \hline
1 & \makecell{} & \makecell{} & $b\bar{d}c\bar{d}$ &  & \makecell{$B^{0} D^{+}$} & \makecell{$7150$} & \makecell{$\Xi^{+}_{bc} \bar{n}$ \\ $\Xi^{0}_{bc} \bar{\Delta}^{+}$ \\ $\Omega^{0}_{bc} \bar{\Sigma}^{+}$} & \makecell{ \\  \\ } & \makecell{$7160-7200$\\$7454-7487$\\$7706-7736$\\$7932-7959$\\$8138-8163$\\$8330-8353$\\$8509-8531$\\$8679-8700$\\$8841-8860$\\$8995-9014$\\$9143-9162$\\$9286-9304$} & \makecell{$7160-7200$\\$7570-7602$\\$7908-7935$\\$8204-8228$\\$8470-8493$\\$8716-8736$\\$8944-8964$\\$9160-9178$\\$9364-9381$\\$9558-9575$\\$9744-9760$\\$9924-9939$} & \makecell{\makecell{$-2.3$-$-2.1$} \\ \makecell{$-1.6$-$-1.5$}} & \makecell{} & $**$ \\
\hline
 \caption{Tetraquark predicted configurations and thresholds.} \label{table:charm_tetraquarks_predictions}
\end{longtable}}\normalsize}

==> tetraquarks/predictions/bc-dd/thresholds.tex <==
\begin{longtable}[c]{|c|c|c|c|c|c|}
  \hline
  \thead{Thry \\ Width \\ $[MeV]$} & \thead{Mesons \\ Pair} & \thead{Meson \\ Threshold \\ $[MeV]$} & \thead{Baryon \\ Anti-\\baryon} & \thead{Baryonic \\ Threshold \\ $[MeV]$} & \thead{Genuine} \\
  \hline
  \hline
 & \makecell{$B^{0} D^{+}$} & \makecell{$7150$} & \makecell{$\Xi^{+}_{bc} \bar{n}$ \\ $\Xi^{0}_{bc} \bar{\Delta}^{+}$ \\ $\Omega^{0}_{bc} \bar{\Sigma}^{+}$} & \makecell{ \\  \\ } & $**$ \\
\hline
  \caption{$T_{b\bar{d}c\bar{d}}$ thresholds.} \label{table:Tbcdd_thresholds}
 \end{longtable}

==> tetraquarks/predictions/bc-ds/spectrum.tex <==
\setlength\LTleft{-1.2cm}
\setlength\LTpre{0.5cm}
{\small\tabcolsep=1pt\footnotesize{\begin{longtable}[!c]{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
  \hline
  \thead{$\#$} & \thead{Candi-\\dates} & \thead{$J^{PC}$} & \thead{Quarks} & \thead{Thry \\ Width \\ $[MeV]$} & \thead{Mesons \\ Pair} & \thead{Meson \\ Threshold \\ $[MeV]$} & \thead{Baryon \\ Anti-\\baryon} & \thead{Baryonic \\ Threshold \\ $[MeV]$} & \thead{$J$ \\ Spec} & \thead{$n$ \\ Spec} & \thead{$a_{T_{j}}$ \\ $a_{T_{n}}$} & \thead{Thry \\ $J + n$} & \thead{Gen-\\uine} \\
  \hline
  \hline
1 & \makecell{} & \makecell{} & $b\bar{d}c\bar{s}$ &  & \makecell{$B^{0}_{s} D^{+}$ \\ $B^{0} D^{+}_{s}$} & \makecell{$7237$ \\ $7248$} & \makecell{$\Xi^{+}_{bc} \bar{\Lambda}^{0}$ \\ $\Xi^{0}_{bc} \bar{\Sigma}^{+}$ \\ $\Omega^{0}_{bc} \bar{\Xi}^{+}$} & \makecell{ \\  \\ } & \makecell{$7247-7287$\\$7541-7574$\\$7792-7822$\\$8017-8044$\\$8222-8247$\\$8413-8436$\\$8591-8613$\\$8760-8781$\\$8921-8940$\\$9075-9093$\\$9222-9240$\\$9364-9382$} & \makecell{$7247-7287$\\$7657-7688$\\$7993-8020$\\$8287-8311$\\$8553-8574$\\$8797-8817$\\$9024-9043$\\$9238-9256$\\$9441-9458$\\$9635-9651$\\$9820-9836$\\$9999-10014$} & \makecell{\makecell{$-2.0$-$-1.9$} \\ \makecell{$-1.4$-$-1.3$}} & \makecell{} & $**$ \\
\hline
 \caption{Tetraquark predicted configurations and thresholds.} \label{table:charm_tetraquarks_predictions}
\end{longtable}}\normalsize}

==> tetraquarks/predictions/bc-ds/thresholds.tex <==
\begin{longtable}[c]{|c|c|c|c|c|c|}
  \hline
  \thead{Thry \\ Width \\ $[MeV]$} & \thead{Mesons \\ Pair} & \thead{Meson \\ Threshold \\ $[MeV]$} & \thead{Baryon \\ Anti-\\baryon} & \thead{Baryonic \\ Threshold \\ $[MeV]$} & \thead{Genuine} \\
  \hline
  \hline
 & \makecell{$B^{0}_{s} D^{+}$ \\ $B^{0} D^{+}_{s}$} & \makecell{$7237$ \\ $7248$} & \makecell{$\Xi^{+}_{bc} \bar{\Lambda}^{0}$ \\ $\Xi^{0}_{bc} \bar{\Sigma}^{+}$ \\ $\Omega^{0}_{bc} \bar{\Xi}^{+}$} & \makecell{ \\  \\ } & $**$ \\
\hline
  \caption{$T_{b\bar{d}c\bar{s}}$ thresholds.} \label{table:Tbcds_thresholds}
 \end{longtable}

==> tetraquarks/predictions/bc-du/spectrum.tex <==
\setlength\LTleft{-1.2cm}
\setlength\LTpre{0.5cm}
{\small\tabcolsep=1pt\footnotesize{\begin{longtable}[!c]{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
  \hline
  \thead{$\#$} & \thead{Candi-\\dates} & \thead{$J^{PC}$} & \thead{Quarks} & \thead{Thry \\ Width \\ $[MeV]$} & \thead{Mesons \\ Pair} & \thead{Meson \\ Threshold \\ $[MeV]$} & \thead{Baryon \\ Anti-\\baryon} & \thead{Baryonic \\ Threshold \\ $[MeV]$} & \thead{$J$ \\ Spec} & \thead{$n$ \\ Spec} & \thead{$a_{T_{j}}$ \\ $a_{T_{n}}$} & \thead{Thry \\ $J + n$} & \thead{Gen-\\uine} \\
  \hline
  \hline
1 & \makecell{} & \makecell{} & $b\bar{d}c\bar{u}$ &  & \makecell{$B^{0} D^{0}$ \\ $B^{+} D^{+}$} & \makecell{$7145$ \\ $7149$} & \makecell{$\Xi^{+}_{bc} \bar{p}$ \\ $\Xi^{0}_{bc} \bar{n}$ \\ $\Omega^{0}_{bc} \bar{\Lambda}^{0}$} & \makecell{ \\  \\ } & \makecell{$7155-7195$\\$7450-7483$\\$7703-7732$\\$7929-7956$\\$8135-8160$\\$8327-8350$\\$8507-8528$\\$8677-8697$\\$8838-8858$\\$8993-9012$\\$9141-9159$\\$9284-9302$} & \makecell{$7155-7195$\\$7566-7598$\\$7905-7932$\\$8201-8225$\\$8468-8490$\\$8713-8734$\\$8942-8961$\\$9157-9175$\\$9361-9379$\\$9556-9573$\\$9743-9758$\\$9922-9937$} & \makecell{\makecell{$-2.3$-$-2.1$} \\ \makecell{$-1.6$-$-1.5$}} & \makecell{} & $**$ \\
\hline
 \caption{Tetraquark predicted configurations and thresholds.} \label{table:charm_tetraquarks_predictions}
\end{longtable}}\normalsize}

==> tetraquarks/predictions/bc-du/thresholds.tex <==
\begin{longtable}[c]{|c|c|c|c|c|c|}
  \hline
  \thead{Thry \\ Width \\ $[MeV]$} & \thead{Mesons \\ Pair} & \thead{Meson \\ Threshold \\ $[MeV]$} & \thead{Baryon \\ Anti-\\baryon} & \thead{Baryonic \\ Threshold \\ $[MeV]$} & \thead{Genuine} \\
  \hline
  \hline
 & \makecell{$B^{0} D^{0}$ \\ $B^{+} D^{+}$} & \makecell{$7145$ \\ $7149$} & \makecell{$\Xi^{+}_{bc} \bar{p}$ \\ $\Xi^{0}_{bc} \bar{n}$ \\ $\Omega^{0}_{bc} \bar{\Lambda}^{0}$} & \makecell{ \\  \\ } & $**$ \\
\hline
  \caption{$T_{b\bar{d}c\bar{u}}$ thresholds.} \label{table:Tbcdu_thresholds}
 \end{longtable}

==> tetraquarks/predictions/bc-ss/spectrum.tex <==
\setlength\LTleft{-1.2cm}
\setlength\LTpre{0.5cm}
{\small\tabcolsep=1pt\footnotesize{\begin{longtable}[!c]{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
  \hline
  \thead{$\#$} & \thead{Candi-\\dates} & \thead{$J^{PC}$} & \thead{Quarks} & \thead{Thry \\ Width \\ $[MeV]$} & \thead{Mesons \\ Pair} & \thead{Meson \\ Threshold \\ $[MeV]$} & \thead{Baryon \\ Anti-\\baryon} & \thead{Baryonic \\ Threshold \\ $[MeV]$} & \thead{$J$ \\ Spec} & \thead{$n$ \\ Spec} & \thead{$a_{T_{j}}$ \\ $a_{T_{n}}$} & \thead{Thry \\ $J + n$} & \thead{Gen-\\uine} \\
  \hline
  \hline
1 & \makecell{} & \makecell{} & $b\bar{s}c\bar{s}$ &  & \makecell{$B^{0}_{s} D^{+}_{s}$} & \makecell{$7335$} & \makecell{$\Xi^{+}_{bc} \bar{\Xi}^{0}$ \\ $\Xi^{0}_{bc} \bar{\Xi}^{+}$ \\ $\Omega^{0}_{bc} \bar{\Omega}^{+}$} & \makecell{ \\  \\ } & \makecell{$7345-7385$\\$7649-7682$\\$7906-7934$\\$8132-8158$\\$8339-8362$\\$8529-8551$\\$8708-8729$\\$8877-8896$\\$9037-9056$\\$9191-9209$\\$9338-9355$\\$9480-9496$} & \makecell{$7345-7385$\\$7768-7798$\\$8108-8134$\\$8404-8427$\\$8669-8690$\\$8913-8933$\\$9140-9158$\\$9354-9371$\\$9556-9573$\\$9749-9765$\\$9934-9949$\\$10112-10126$} & \makecell{\makecell{$-1.6$-$-1.5$} \\ \makecell{$-1.1$-$-1.0$}} & \makecell{} & $**$ \\
\hline
 \caption{Tetraquark predicted configurations and thresholds.} \label{table:charm_tetraquarks_predictions}
\end{longtable}}\normalsize}

==> tetraquarks/predictions/bc-ss/thresholds.tex <==
\begin{longtable}[c]{|c|c|c|c|c|c|}
  \hline
  \thead{Thry \\ Width \\ $[MeV]$} & \thead{Mesons \\ Pair} & \thead{Meson \\ Threshold \\ $[MeV]$} & \thead{Baryon \\ Anti-\\baryon} & \thead{Baryonic \\ Threshold \\ $[MeV]$} & \thead{Genuine} \\
  \hline
  \hline
 & \makecell{$B^{0}_{s} D^{+}_{s}$} & \makecell{$7335$} & \makecell{$\Xi^{+}_{bc} \bar{\Xi}^{0}$ \\ $\Xi^{0}_{bc} \bar{\Xi}^{+}$ \\ $\Omega^{0}_{bc} \bar{\Omega}^{+}$} & \makecell{ \\  \\ } & $**$ \\
\hline
  \caption{$T_{b\bar{s}c\bar{s}}$ thresholds.} \label{table:Tbcss_thresholds}
 \end{longtable}

==> tetraquarks/predictions/bc-su/spectrum.tex <==
\setlength\LTleft{-1.2cm}
\setlength\LTpre{0.5cm}
{\small\tabcolsep=1pt\footnotesize{\begin{longtable}[!c]{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
  \hline
  \thead{$\#$} & \thead{Candi-\\dates} & \thead{$J^{PC}$} & \thead{Quarks} & \thead{Thry \\ Width \\ $[MeV]$} & \thead{Mesons \\ Pair} & \thead{Meson \\ Threshold \\ $[MeV]$} & \thead{Baryon \\ Anti-\\baryon} & \thead{Baryonic \\ Threshold \\ $[MeV]$} & \thead{$J$ \\ Spec} & \thead{$n$ \\ Spec} & \thead{$a_{T_{j}}$ \\ $a_{T_{n}}$} & \thead{Thry \\ $J + n$} & \thead{Gen-\\uine} \\
  \hline
  \hline
1 & \makecell{} & \makecell{} & $b\bar{s}c\bar{u}$ &  & \makecell{$B^{0}_{s} D^{0}$ \\ $B^{+} D^{+}_{s}$} & \makecell{$7232$ \\ $7247$} & \makecell{$\Xi^{+}_{bc} \bar{\Sigma}^{-}$ \\ $\Xi^{0}_{bc} \bar{\Lambda}^{0}$ \\ $\Omega^{0}_{bc} \bar{\Xi}^{0}$} & \makecell{ \\  \\ } & \makecell{$7242-7282$\\$7537-7570$\\$7789-7818$\\$8014-8040$\\$8219-8244$\\$8410-8433$\\$8589-8610$\\$8758-8778$\\$8918-8938$\\$9072-9091$\\$9220-9238$\\$9362-9380$} & \makecell{$7242-7282$\\$7653-7684$\\$7990-8017$\\$8284-8308$\\$8550-8572$\\$8794-8814$\\$9022-9041$\\$9236-9254$\\$9439-9456$\\$9633-9649$\\$9818-9834$\\$9997-10012$} & \makecell{\makecell{$-2.0$-$-1.9$} \\ \makecell{$-1.4$-$-1.3$}} & \makecell{} & $**$ \\
\hline
 \caption{Tetraquark predicted configurations and thresholds.} \label{table:charm_tetraquarks_predictions}
\end{longtable}}\normalsize}

==> tetraquarks/predictions/bc-su/thresholds.tex <==
\begin{longtable}[c]{|c|c|c|c|c|c|}
  \hline
  \thead{Thry \\ Width \\ $[MeV]$} & \thead{Mesons \\ Pair} & \thead{Meson \\ Threshold \\ $[MeV]$} & \thead{Baryon \\ Anti-\\baryon} & \thead{Baryonic \\ Threshold \\ $[MeV]$} & \thead{Genuine} \\
  \hline
  \hline
 & \makecell{$B^{0}_{s} D^{0}$ \\ $B^{+} D^{+}_{s}$} & \makecell{$7232$ \\ $7247$} & \makecell{$\Xi^{+}_{bc} \bar{\Sigma}^{-}$ \\ $\Xi^{0}_{bc} \bar{\Lambda}^{0}$ \\ $\Omega^{0}_{bc} \bar{\Xi}^{0}$} & \makecell{ \\  \\ } & $**$ \\
\hline
  \caption{$T_{b\bar{s}c\bar{u}}$ thresholds.} \label{table:Tbcsu_thresholds}
 \end{longtable}

==> tetraquarks/predictions/bc-uu/spectrum.tex <==
\setlength\LTleft{-1.2cm}
\setlength\LTpre{0.5cm}
{\small\tabcolsep=1pt\footnotesize{\begin{longtable}[!c]{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
  \hline
  \thead{$\#$} & \thead{Candi-\\dates} & \thead{$J^{PC}$} & \thead{Quarks} & \thead{Thry \\ Width \\ $[MeV]$} & \thead{Mesons \\ Pair} & \thead{Meson \\ Threshold \\ $[MeV]$} & \thead{Baryon \\ Anti-\\baryon} & \thead{Baryonic \\ Threshold \\ $[MeV]$} & \thead{$J$ \\ Spec} & \thead{$n$ \\ Spec} & \thead{$a_{T_{j}}$ \\ $a_{T_{n}}$} & \thead{Thry \\ $J + n$} & \thead{Gen-\\uine} \\
  \hline
  \hline
1 & \makecell{} & \makecell{} & $b\bar{u}c\bar{u}$ &  & \makecell{$B^{+} D^{0}$} & \makecell{$7144$} & \makecell{$\Xi^{+}_{bc} \bar{\Delta}^{--}$ \\ $\Xi^{0}_{bc} \bar{p}$ \\ $\Omega^{0}_{bc} \bar{\Sigma}^{-}$} & \makecell{ \\  \\ } & \makecell{$7154-7194$\\$7449-7482$\\$7702-7732$\\$7928-7955$\\$8135-8159$\\$8326-8349$\\$8506-8528$\\$8676-8697$\\$8838-8857$\\$8992-9011$\\$9141-9159$\\$9284-9301$} & \makecell{$7154-7194$\\$7565-7597$\\$7904-7931$\\$8200-8224$\\$8467-8489$\\$8713-8733$\\$8942-8961$\\$9157-9175$\\$9361-9378$\\$9556-9572$\\$9742-9758$\\$9921-9937$} & \makecell{\makecell{$-2.3$-$-2.1$} \\ \makecell{$-1.6$-$-1.5$}} & \makecell{} & $**$ \\
\hline
 \caption{Tetraquark predicted configurations and thresholds.} \label{table:charm_tetraquarks_predictions}
\end{longtable}}\normalsize}

==> tetraquarks/predictions/bc-uu/thresholds.tex <==
\begin{longtable}[c]{|c|c|c|c|c|c|}
  \hline
  \thead{Thry \\ Width \\ $[MeV]$} & \thead{Mesons \\ Pair} & \thead{Meson \\ Threshold \\ $[MeV]$} & \thead{Baryon \\ Anti-\\baryon} & \thead{Baryonic \\ Threshold \\ $[MeV]$} & \thead{Genuine} \\
  \hline
  \hline
 & \makecell{$B^{+} D^{0}$} & \makecell{$7144$} & \makecell{$\Xi^{+}_{bc} \bar{\Delta}^{--}$ \\ $\Xi^{0}_{bc} \bar{p}$ \\ $\Omega^{0}_{bc} \bar{\Sigma}^{-}$} & \makecell{ \\  \\ } & $**$ \\
\hline
  \caption{$T_{b\bar{u}c\bar{u}}$ thresholds.} \label{table:Tbcuu_thresholds}
 \end{longtable}

==> tetraquarks/predictions/cc-bb/thresholds.tex <==
\begin{longtable}[c]{|c|c|c|c|c|c|}
  \hline
  \thead{Thry \\ Width \\ $[MeV]$} & \thead{Mesons \\ Pair} & \thead{Meson \\ Threshold \\ $[MeV]$} & \thead{Baryon \\ Anti-\\baryon} & \thead{Baryonic \\ Threshold \\ $[MeV]$} & \thead{Genuine} \\
  \hline
  \hline
 & \makecell{$B^{+}_{c} B^{+}_{c}$} & \makecell{$12548$} & \makecell{$\Xi^{++}_{cc} \bar{\Xi}^{0}_{bb}$ \\ $\Xi^{+}_{cc} \bar{\Xi}^{+}_{bb}$ \\ $\Omega^{+}_{cc} \bar{\Omega}^{+}_{bb}$} & \makecell{ \\  \\ } & $**$ \\
\hline
  \caption{$T_{c\bar{b}c\bar{b}}$ thresholds.} \label{table:Tccbb_thresholds}
 \end{longtable}

==> tetraquarks/predictions/cc-bc/thresholds.tex <==
\begin{longtable}[c]{|c|c|c|c|c|c|}
  \hline
  \thead{Thry \\ Width \\ $[MeV]$} & \thead{Mesons \\ Pair} & \thead{Meson \\ Threshold \\ $[MeV]$} & \thead{Baryon \\ Anti-\\baryon} & \thead{Baryonic \\ Threshold \\ $[MeV]$} & \thead{Genuine} \\
  \hline
  \hline
 & \makecell{$B^{+}_{c} \eta_{c}(1S)$ \\ $\eta_{c}(1S) B^{+}_{c}$} & \makecell{$9258$ \\ $9258$} & \makecell{$\Xi^{++}_{cc} \bar{\Xi}^{-}_{bc}$ \\ $\Xi^{+}_{cc} \bar{\Xi}^{0}_{bc}$ \\ $\Omega^{+}_{cc} \bar{\Omega}^{0}_{bc}$} & \makecell{ \\  \\ } & $*$ \\
\hline
  \caption{$T_{c\bar{b}c\bar{c}}$ thresholds.} \label{table:Tccbc_thresholds}
 \end{longtable}

==> tetraquarks/predictions/cc-bd/thresholds.tex <==
\begin{longtable}[c]{|c|c|c|c|c|c|}
  \hline
  \thead{Thry \\ Width \\ $[MeV]$} & \thead{Mesons \\ Pair} & \thead{Meson \\ Threshold \\ $[MeV]$} & \thead{Baryon \\ Anti-\\baryon} & \thead{Baryonic \\ Threshold \\ $[MeV]$} & \thead{Genuine} \\
  \hline
  \hline
 & \makecell{$B^{+}_{c} D^{+}$ \\ $D^{+} B^{+}_{c}$} & \makecell{$8144$ \\ $8144$} & \makecell{$\Xi^{+}_{cc} \bar{\Sigma}^{+}_{b}$ \\ $\Xi^{++}_{cc} \bar{\Sigma}^{0}_{b}$ \\ $\Omega^{+}_{cc} \bar{\Xi}^{+}_{b}$} & \makecell{$9335$ \\  \\ } & $**$ \\
\hline
  \caption{$T_{c\bar{b}c\bar{d}}$ thresholds.} \label{table:Tccbd_thresholds}
 \end{longtable}

==> tetraquarks/predictions/cc-bs/thresholds.tex <==
\begin{longtable}[c]{|c|c|c|c|c|c|}
  \hline
  \thead{Thry \\ Width \\ $[MeV]$} & \thead{Mesons \\ Pair} & \thead{Meson \\ Threshold \\ $[MeV]$} & \thead{Baryon \\ Anti-\\baryon} & \thead{Baryonic \\ Threshold \\ $[MeV]$} & \thead{Genuine} \\
  \hline
  \hline
 & \makecell{$B^{+}_{c} D^{+}_{s}$ \\ $D^{+}_{s} B^{+}_{c}$} & \makecell{$8242$ \\ $8242$} & \makecell{$\Xi^{+}_{cc} \bar{\Xi}^{+}_{b}$ \\ $\Xi^{++}_{cc} \bar{\Xi}^{0}_{b}$ \\ $\Omega^{+}_{cc} \bar{\Omega}^{+}_{b}$} & \makecell{$9316$ \\ $9414$ \\ } & $**$ \\
\hline
  \caption{$T_{c\bar{b}c\bar{s}}$ thresholds.} \label{table:Tccbs_thresholds}
 \end{longtable}

==> tetraquarks/predictions/cc-bu/thresholds.tex <==
\begin{longtable}[c]{|c|c|c|c|c|c|}
  \hline
  \thead{Thry \\ Width \\ $[MeV]$} & \thead{Mesons \\ Pair} & \thead{Meson \\ Threshold \\ $[MeV]$} & \thead{Baryon \\ Anti-\\baryon} & \thead{Baryonic \\ Threshold \\ $[MeV]$} & \thead{Genuine} \\
  \hline
  \hline
 & \makecell{$B^{+}_{c} D^{0}$ \\ $D^{0} B^{+}_{c}$} & \makecell{$8139$ \\ $8139$} & \makecell{$\Xi^{++}_{cc} \bar{\Sigma}^{-}_{b}$ \\ $\Xi^{+}_{cc} \bar{\Sigma}^{0}_{b}$ \\ $\Omega^{+}_{cc} \bar{\Xi}^{0}_{b}$} & \makecell{$9433$ \\  \\ } & $**$ \\
\hline
  \caption{$T_{c\bar{b}c\bar{u}}$ thresholds.} \label{table:Tccbu_thresholds}
 \end{longtable}

==> tetraquarks/predictions/cc-cc/spectrum.tex <==
\setlength\LTleft{-1.2cm}
\setlength\LTpre{0.5cm}
{\small\tabcolsep=1pt\footnotesize{\begin{longtable}[!c]{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
  \hline
  \thead{$\#$} & \thead{Candi-\\dates} & \thead{$J^{PC}$} & \thead{Quarks} & \thead{Thry \\ Width \\ $[MeV]$} & \thead{Mesons \\ Pair} & \thead{Meson \\ Threshold \\ $[MeV]$} & \thead{Baryon \\ Anti-\\baryon} & \thead{Baryonic \\ Threshold \\ $[MeV]$} & \thead{$J$ \\ Spec} & \thead{$n$ \\ Spec} & \thead{$a_{T_{j}}$ \\ $a_{T_{n}}$} & \thead{Thry \\ $J + n$} & \thead{Gen-\\uine} \\
  \hline
  \hline
1 & \makecell{$T_{\psi\psi}(6600)$\\$T_{\psi\psi}(6600)$\\$T_{\psi\psi}(6900)$\\$T_{\psi\psi}(6900)$\\$T_{\psi\psi}(7300)$} & \makecell{$?^{??}$\\$?^{??}$\\$?^{??}$\\$?^{??}$\\$?^{??}$} & $c\bar{c}c\bar{c}$ & \makecell{$6-21$\\$29-58$} & \makecell{$\eta_{c}(1S) \eta_{c}(1S)$} & \makecell{$5968$} & \makecell{$\Xi^{+}_{cc} \bar{\Xi}^{-}_{cc}$ \\ $\Xi^{++}_{cc} \bar{\Xi}^{--}_{cc}$ \\ $\Omega^{+}_{cc} \bar{\Omega}^{-}_{cc}$} & \makecell{$7038$ \\ $7244$ \\ } & \makecell{$6768-6887$\\$6926-7040$\\$7078-7188$\\$7225-7331$\\$7366-7469$} & \makecell{$6622-6745$\\$6857-6973$\\$7078-7188$\\$7288-7393$\\$7489-7589$} & \makecell{\makecell{$-5.9$-$-5.1$} \\ \makecell{$-4.2$-$-3.7$}} & \makecell{$6$ \\ $4$} & $*$ \\
\hline
 \caption{Tetraquark predicted configurations and thresholds.} \label{table:charm_tetraquarks_predictions}
\end{longtable}}\normalsize}

==> tetraquarks/predictions/cc-cd/thresholds.tex <==
\begin{longtable}[c]{|c|c|c|c|c|c|}
  \hline
  \thead{Thry \\ Width \\ $[MeV]$} & \thead{Mesons \\ Pair} & \thead{Meson \\ Threshold \\ $[MeV]$} & \thead{Baryon \\ Anti-\\baryon} & \thead{Baryonic \\ Threshold \\ $[MeV]$} & \thead{Genuine} \\
  \hline
  \hline
\makecell{$8-24$\\$30-61$} & \makecell{$\eta_{c}(1S) D^{+}$ \\ $D^{+} \eta_{c}(1S)$} & \makecell{$4854$ \\ $4854$} & \makecell{$\Xi^{++}_{cc} \bar{\Lambda}^{-}_{c}$ \\ $\Xi^{+}_{cc} \bar{\Sigma}^{0}_{c}$ \\ $\Omega^{+}_{cc} \bar{\Xi}^{0}_{c}$} & \makecell{$5908$ \\ $5973$ \\ } & $*$ \\
\hline
  \caption{$T_{c\bar{c}c\bar{d}}$ thresholds.} \label{table:Tcccd_thresholds}
 \end{longtable}

==> tetraquarks/predictions/cc-cs/thresholds.tex <==
\begin{longtable}[c]{|c|c|c|c|c|c|}
  \hline
  \thead{Thry \\ Width \\ $[MeV]$} & \thead{Mesons \\ Pair} & \thead{Meson \\ Threshold \\ $[MeV]$} & \thead{Baryon \\ Anti-\\baryon} & \thead{Baryonic \\ Threshold \\ $[MeV]$} & \thead{Genuine} \\
  \hline
  \hline
\makecell{$26-53$\\$27-55$} & \makecell{$\eta_{c}(1S) D^{+}_{s}$ \\ $D^{+}_{s} \eta_{c}(1S)$} & \makecell{$4952$ \\ $4952$} & \makecell{$\Xi^{+}_{cc} \bar{\Xi}^{0}_{c}$ \\ $\Xi^{++}_{cc} \bar{\Xi}^{-}_{c}$ \\ $\Omega^{+}_{cc} \bar{\Omega}^{0}_{c}$} & \makecell{$5989$ \\ $6090$ \\ } & $*$ \\
\hline
  \caption{$T_{c\bar{c}c\bar{s}}$ thresholds.} \label{table:Tcccs_thresholds}
 \end{longtable}

==> tetraquarks/predictions/cc-cu/thresholds.tex <==
\begin{longtable}[c]{|c|c|c|c|c|c|}
  \hline
  \thead{Thry \\ Width \\ $[MeV]$} & \thead{Mesons \\ Pair} & \thead{Meson \\ Threshold \\ $[MeV]$} & \thead{Baryon \\ Anti-\\baryon} & \thead{Baryonic \\ Threshold \\ $[MeV]$} & \thead{Genuine} \\
  \hline
  \hline
\makecell{$13-33$\\$29-59$} & \makecell{$\eta_{c}(1S) D^{0}$ \\ $D^{0} \eta_{c}(1S)$} & \makecell{$4849$ \\ $4849$} & \makecell{$\Xi^{+}_{cc} \bar{\Lambda}^{-}_{c}$ \\ $\Xi^{++}_{cc} \bar{\Sigma}^{--}_{c}$ \\ $\Omega^{+}_{cc} \bar{\Xi}^{-}_{c}$} & \makecell{$5805$ \\ $6076$ \\ } & $*$ \\
\hline
  \caption{$T_{c\bar{c}c\bar{u}}$ thresholds.} \label{table:Tcccu_thresholds}
 \end{longtable}

==> tetraquarks/predictions/cc-dd/thresholds.tex <==
\begin{longtable}[c]{|c|c|c|c|c|c|}
  \hline
  \thead{Thry \\ Width \\ $[MeV]$} & \thead{Mesons \\ Pair} & \thead{Meson \\ Threshold \\ $[MeV]$} & \thead{Baryon \\ Anti-\\baryon} & \thead{Baryonic \\ Threshold \\ $[MeV]$} & \thead{Genuine} \\
  \hline
  \hline
 & \makecell{$D^{+} D^{+}$} & \makecell{$3740$} & \makecell{$\Xi^{++}_{cc} \bar{n}$ \\ $\Xi^{+}_{cc} \bar{\Delta}^{+}$ \\ $\Omega^{+}_{cc} \bar{\Sigma}^{+}$} & \makecell{$4562$ \\ $4751$ \\ } & $**$ \\
\hline
  \caption{$T_{c\bar{d}c\bar{d}}$ thresholds.} \label{table:Tccdd_thresholds}
 \end{longtable}

==> tetraquarks/predictions/cc-ds/thresholds.tex <==
\begin{longtable}[c]{|c|c|c|c|c|c|}
  \hline
  \thead{Thry \\ Width \\ $[MeV]$} & \thead{Mesons \\ Pair} & \thead{Meson \\ Threshold \\ $[MeV]$} & \thead{Baryon \\ Anti-\\baryon} & \thead{Baryonic \\ Threshold \\ $[MeV]$} & \thead{Genuine} \\
  \hline
  \hline
 & \makecell{$D^{+} D^{+}_{s}$ \\ $D^{+}_{s} D^{+}$} & \makecell{$3838$ \\ $3838$} & \makecell{$\Xi^{+}_{cc} \bar{\Sigma}^{+}$ \\ $\Xi^{++}_{cc} \bar{\Lambda}^{0}$ \\ $\Omega^{+}_{cc} \bar{\Xi}^{+}$} & \makecell{$4716$ \\ $4738$ \\ } & $**$ \\
\hline
  \caption{$T_{c\bar{d}c\bar{s}}$ thresholds.} \label{table:Tccds_thresholds}
 \end{longtable}

==> tetraquarks/predictions/cc-du/spectrum.tex <==
\setlength\LTleft{-1.2cm}
\setlength\LTpre{0.5cm}
{\small\tabcolsep=1pt\footnotesize{\begin{longtable}[!c]{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
  \hline
  \thead{$\#$} & \thead{Candi-\\dates} & \thead{$J^{PC}$} & \thead{Quarks} & \thead{Thry \\ Width \\ $[MeV]$} & \thead{Mesons \\ Pair} & \thead{Meson \\ Threshold \\ $[MeV]$} & \thead{Baryon \\ Anti-\\baryon} & \thead{Baryonic \\ Threshold \\ $[MeV]$} & \thead{$J$ \\ Spec} & \thead{$n$ \\ Spec} & \thead{$a_{T_{j}}$ \\ $a_{T_{n}}$} & \thead{Thry \\ $J + n$} & \thead{Gen-\\uine} \\
  \hline
  \hline
1 & \makecell{$T_{cc}(3875)$} & \makecell{$?^{?}$} & $c\bar{d}c\bar{u}$ &  & \makecell{$D^{+} D^{0}$ \\ $D^{0} D^{+}$} & \makecell{$3735$ \\ $3735$} & \makecell{$\Xi^{+}_{cc} \bar{n}$ \\ $\Xi^{++}_{cc} \bar{p}$ \\ $\Omega^{+}_{cc} \bar{\Lambda}^{0}$} & \makecell{$4459$ \\ $4560$ \\ } & \makecell{$3983-4118$\\$4255-4375$\\$4499-4609$\\$4723-4825$\\$4932-5027$} & \makecell{$4499-4609$\\$4818-4917$\\$5107-5198$\\$5373-5458$\\$5622-5702$} & \makecell{\makecell{$-3.7$-$-3.3$} \\ \makecell{$-3.0$-$-2.6$}} & \makecell{$2$ \\ $1$} & $**$ \\
\hline
 \caption{Tetraquark predicted configurations and thresholds.} \label{table:charm_tetraquarks_predictions}
\end{longtable}}\normalsize}

==> tetraquarks/predictions/cc-ss/thresholds.tex <==
\begin{longtable}[c]{|c|c|c|c|c|c|}
  \hline
  \thead{Thry \\ Width \\ $[MeV]$} & \thead{Mesons \\ Pair} & \thead{Meson \\ Threshold \\ $[MeV]$} & \thead{Baryon \\ Anti-\\baryon} & \thead{Baryonic \\ Threshold \\ $[MeV]$} & \thead{Genuine} \\
  \hline
  \hline
 & \makecell{$D^{+}_{s} D^{+}_{s}$} & \makecell{$3936$} & \makecell{$\Xi^{+}_{cc} \bar{\Xi}^{+}$ \\ $\Xi^{++}_{cc} \bar{\Xi}^{0}$ \\ $\Omega^{+}_{cc} \bar{\Omega}^{+}$} & \makecell{$4841$ \\ $4937$ \\ } & $**$ \\
\hline
  \caption{$T_{c\bar{s}c\bar{s}}$ thresholds.} \label{table:Tccss_thresholds}
 \end{longtable}

==> tetraquarks/predictions/cc-su/thresholds.tex <==
\begin{longtable}[c]{|c|c|c|c|c|c|}
  \hline
  \thead{Thry \\ Width \\ $[MeV]$} & \thead{Mesons \\ Pair} & \thead{Meson \\ Threshold \\ $[MeV]$} & \thead{Baryon \\ Anti-\\baryon} & \thead{Baryonic \\ Threshold \\ $[MeV]$} & \thead{Genuine} \\
  \hline
  \hline
 & \makecell{$D^{+}_{s} D^{0}$ \\ $D^{0} D^{+}_{s}$} & \makecell{$3833$ \\ $3833$} & \makecell{$\Xi^{+}_{cc} \bar{\Lambda}^{0}$ \\ $\Xi^{++}_{cc} \bar{\Sigma}^{-}$ \\ $\Omega^{+}_{cc} \bar{\Xi}^{0}$} & \makecell{$4635$ \\ $4811$ \\ } & $**$ \\
\hline
  \caption{$T_{c\bar{s}c\bar{u}}$ thresholds.} \label{table:Tccsu_thresholds}
 \end{longtable}

==> tetraquarks/predictions/cc-uu/thresholds.tex <==
\begin{longtable}[c]{|c|c|c|c|c|c|}
  \hline
  \thead{Thry \\ Width \\ $[MeV]$} & \thead{Mesons \\ Pair} & \thead{Meson \\ Threshold \\ $[MeV]$} & \thead{Baryon \\ Anti-\\baryon} & \thead{Baryonic \\ Threshold \\ $[MeV]$} & \thead{Genuine} \\
  \hline
  \hline
 & \makecell{$D^{0} D^{0}$} & \makecell{$3730$} & \makecell{$\Xi^{+}_{cc} \bar{p}$ \\ $\Xi^{++}_{cc} \bar{\Delta}^{--}$ \\ $\Omega^{+}_{cc} \bar{\Sigma}^{-}$} & \makecell{$4457$ \\ $4854$ \\ } & $**$ \\
\hline
  \caption{$T_{c\bar{u}c\bar{u}}$ thresholds.} \label{table:Tccuu_thresholds}
 \end{longtable}

==> tetraquarks/predictions/cd-bb/thresholds.tex <==
\begin{longtable}[c]{|c|c|c|c|c|c|}
  \hline
  \thead{Thry \\ Width \\ $[MeV]$} & \thead{Mesons \\ Pair} & \thead{Meson \\ Threshold \\ $[MeV]$} & \thead{Baryon \\ Anti-\\baryon} & \thead{Baryonic \\ Threshold \\ $[MeV]$} & \thead{Genuine} \\
  \hline
  \hline
 & \makecell{$B^{+}_{c} \bar{B}^{0}$} & \makecell{$11554$} & \makecell{$\Lambda^{+}_{c} \bar{\Xi}^{0}_{bb}$ \\ $\Sigma^{0}_{c} \bar{\Xi}^{+}_{bb}$ \\ $\Xi^{0}_{c} \bar{\Omega}^{+}_{bb}$} & \makecell{ \\  \\ } & $**$ \\
\hline
  \caption{$T_{c\bar{b}d\bar{b}}$ thresholds.} \label{table:Tcdbb_thresholds}
 \end{longtable}

==> tetraquarks/predictions/cd-bc/thresholds.tex <==
\begin{longtable}[c]{|c|c|c|c|c|c|}
  \hline
  \thead{Thry \\ Width \\ $[MeV]$} & \thead{Mesons \\ Pair} & \thead{Meson \\ Threshold \\ $[MeV]$} & \thead{Baryon \\ Anti-\\baryon} & \thead{Baryonic \\ Threshold \\ $[MeV]$} & \thead{Genuine} \\
  \hline
  \hline
 & \makecell{$B^{+}_{c} D^{-}$ \\ $\eta_{c}(1S) \bar{B}^{0}$} & \makecell{$8144$ \\ $8264$} & \makecell{$\Lambda^{+}_{c} \bar{\Xi}^{-}_{bc}$ \\ $\Sigma^{0}_{c} \bar{\Xi}^{0}_{bc}$ \\ $\Xi^{0}_{c} \bar{\Omega}^{0}_{bc}$} & \makecell{ \\  \\ } & $*$ \\
\hline
  \caption{$T_{c\bar{b}d\bar{c}}$ thresholds.} \label{table:Tcdbc_thresholds}
 \end{longtable}

==> tetraquarks/predictions/cd-bd/j_predictions.tex <==
\begin{longtable}[c]{|c|c|}
  \hline
  \thead{$J$ \\ Spec} & \thead{$a_{T_{j}}$} \\
  \hline
  \hline
\makecell{$7986-8106$\\$8150-8265$\\$8307-8417$\\$8457-8563$\\$8602-8704$\\$8742-8840$\\$8877-8973$\\$9008-9101$\\$9136-9226$\\$9260-9348$\\$9381-9467$\\$9499-9584$} & \makecell{$-2.6$-$-1.8$} \\
\hline
  \caption{$T_{c\bar{b}d\bar{d}}$ $(J, M^2)$ predictions.} \label{table:Tcdbd_j_predictions}
 \end{longtable}

==> tetraquarks/predictions/cd-bd/n_predictions.tex <==
\begin{longtable}[c]{|c|c|}
  \hline
  \thead{$n$ \\ Spec} & \thead{$a_{T_{n}}$} \\
  \hline
  \hline
\makecell{$7833-7959$\\$8078-8195$\\$8307-8417$\\$8522-8626$\\$8726-8826$\\$8921-9016$\\$9107-9199$\\$9287-9375$\\$9460-9545$\\$9628-9710$\\$9790-9870$\\$9948-10026$} & \makecell{$-2.3$-$-1.8$} \\
\hline
  \caption{$T_{c\bar{b}d\bar{d}}$ $(n, M^2)$ predictions.} \label{table:Tcdbd_n_predictions}
 \end{longtable}

==> tetraquarks/predictions/cd-bd/thresholds.tex <==
\begin{longtable}[c]{|c|c|c|c|c|c|}
  \hline
  \thead{Thry \\ Width \\ $[MeV]$} & \thead{Mesons \\ Pair} & \thead{Meson \\ Threshold \\ $[MeV]$} & \thead{Baryon \\ Anti-\\baryon} & \thead{Baryonic \\ Threshold \\ $[MeV]$} & \thead{Genuine} \\
  \hline
  \hline
 & \makecell{$B^{+}_{c} \pi^{0}_{d}$ \\ $D^{+} \bar{B}^{0}$} & \makecell{$6409$ \\ $7150$} & \makecell{$\Xi^{0}_{c} \bar{\Xi}^{+}_{b}$ \\ $\Sigma^{0}_{c} \bar{\Sigma}^{+}_{b}$ \\ $\Lambda^{+}_{c} \bar{\Sigma}^{0}_{b}$} & \makecell{$8267$ \\ $8270$ \\ } &  \\
\hline
  \caption{$T_{c\bar{b}d\bar{d}}$ thresholds.} \label{table:Tcdbd_thresholds}
 \end{longtable}

==> tetraquarks/predictions/cd-bs/thresholds.tex <==
\begin{longtable}[c]{|c|c|c|c|c|c|}
  \hline
  \thead{Thry \\ Width \\ $[MeV]$} & \thead{Mesons \\ Pair} & \thead{Meson \\ Threshold \\ $[MeV]$} & \thead{Baryon \\ Anti-\\baryon} & \thead{Baryonic \\ Threshold \\ $[MeV]$} & \thead{Genuine} \\
  \hline
  \hline
 & \makecell{$B^{+}_{c} K^{0}$ \\ $D^{+}_{s} \bar{B}^{0}$} & \makecell{$6772$ \\ $7248$} & \makecell{$\Lambda^{+}_{c} \bar{\Xi}^{0}_{b}$ \\ $\Sigma^{0}_{c} \bar{\Xi}^{+}_{b}$ \\ $\Xi^{0}_{c} \bar{\Omega}^{+}_{b}$} & \makecell{$8078$ \\ $8251$ \\ $8516$} & $**$ \\
\hline
  \caption{$T_{c\bar{b}d\bar{s}}$ thresholds.} \label{table:Tcdbs_thresholds}
 \end{longtable}

==> tetraquarks/predictions/cd-bu/thresholds.tex <==
\begin{longtable}[c]{|c|c|c|c|c|c|}
  \hline
  \thead{Thry \\ Width \\ $[MeV]$} & \thead{Mesons \\ Pair} & \thead{Meson \\ Threshold \\ $[MeV]$} & \thead{Baryon \\ Anti-\\baryon} & \thead{Baryonic \\ Threshold \\ $[MeV]$} & \thead{Genuine} \\
  \hline
  \hline
 & \makecell{$B^{+}_{c} \pi^{-}$ \\ $D^{0} \bar{B}^{0}$} & \makecell{$6414$ \\ $7145$} & \makecell{$\Lambda^{+}_{c} \bar{\Sigma}^{-}_{b}$ \\ $\Xi^{0}_{c} \bar{\Xi}^{0}_{b}$ \\ $\Sigma^{0}_{c} \bar{\Sigma}^{0}_{b}$} & \makecell{$8097$ \\ $8262$ \\ } & $**$ \\
\hline
  \caption{$T_{c\bar{b}d\bar{u}}$ thresholds.} \label{table:Tcdbu_thresholds}
 \end{longtable}

==> tetraquarks/predictions/cd-cd/j_predictions.tex <==
\begin{longtable}[c]{|c|c|}
  \hline
  \thead{$J$ \\ Spec} & \thead{$a_{T_{j}}$} \\
  \hline
  \hline
\makecell{$4182-4308$\\$4404-4521$\\$4612-4722$\\$4808-4912$\\$4993-5092$\\$5170-5265$\\$5340-5431$\\$5503-5591$\\$5660-5745$\\$5812-5894$\\$5959-6039$\\$6102-6180$} & \makecell{$-2.7$-$-2.2$} \\
\hline
  \caption{$T_{c\bar{c}d\bar{d}}$ $(J, M^2)$ predictions.} \label{table:Tcdcd_j_predictions}
 \end{longtable}

==> tetraquarks/predictions/cd-cd/n_predictions.tex <==
\begin{longtable}[c]{|c|c|}
  \hline
  \thead{$n$ \\ Spec} & \thead{$a_{T_{n}}$} \\
  \hline
  \hline
\makecell{$3969-4104$\\$4308-4428$\\$4612-4722$\\$4891-4993$\\$5151-5246$\\$5395-5485$\\$5626-5711$\\$5845-5927$\\$6055-6134$\\$6257-6332$\\$6451-6524$\\$6639-6709$} & \makecell{$-2.3$-$-2.0$} \\
\hline
  \caption{$T_{c\bar{c}d\bar{d}}$ $(n, M^2)$ predictions.} \label{table:Tcdcd_n_predictions}
 \end{longtable}

==> tetraquarks/predictions/cd-cd/thresholds.tex <==
\begin{longtable}[c]{|c|c|c|c|c|c|}
  \hline
  \thead{Thry \\ Width \\ $[MeV]$} & \thead{Mesons \\ Pair} & \thead{Meson \\ Threshold \\ $[MeV]$} & \thead{Baryon \\ Anti-\\baryon} & \thead{Baryonic \\ Threshold \\ $[MeV]$} & \thead{Genuine} \\
  \hline
  \hline
\makecell{$24-51$\\$32-64$} & \makecell{$\eta_{c}(1S) \pi^{0}_{d}$ \\ $D^{+} D^{-}$} & \makecell{$3119$ \\ $3740$} & \makecell{$\Lambda^{+}_{c} \bar{\Lambda}^{-}_{c}$ \\ $\Sigma^{0}_{c} \bar{\Sigma}^{0}_{c}$ \\ $\Xi^{0}_{c} \bar{\Xi}^{0}_{c}$} & \makecell{$4572$ \\ $4908$ \\ $4940$} &  \\
\hline
  \caption{$T_{c\bar{c}d\bar{d}}$ thresholds.} \label{table:Tcdcd_thresholds}
 \end{longtable}

==> tetraquarks/predictions/cd-cs/thresholds.tex <==
\begin{longtable}[c]{|c|c|c|c|c|c|}
  \hline
  \thead{Thry \\ Width \\ $[MeV]$} & \thead{Mesons \\ Pair} & \thead{Meson \\ Threshold \\ $[MeV]$} & \thead{Baryon \\ Anti-\\baryon} & \thead{Baryonic \\ Threshold \\ $[MeV]$} & \thead{Genuine} \\
  \hline
  \hline
\makecell{$47-80$\\$29-59$} & \makecell{$\eta_{c}(1S) K^{0}$ \\ $D^{+}_{s} D^{-}$} & \makecell{$3482$ \\ $3838$} & \makecell{$\Lambda^{+}_{c} \bar{\Xi}^{-}_{c}$ \\ $\Sigma^{0}_{c} \bar{\Xi}^{0}_{c}$ \\ $\Xi^{0}_{c} \bar{\Omega}^{0}_{c}$} & \makecell{$4754$ \\ $4924$ \\ $5165$} & $*$ \\
\hline
  \caption{$T_{c\bar{c}d\bar{s}}$ thresholds.} \label{table:Tcdcs_thresholds}
 \end{longtable}

==> tetraquarks/predictions/cd-cu/thresholds.tex <==
\begin{longtable}[c]{|c|c|c|c|c|c|}
  \hline
  \thead{Thry \\ Width \\ $[MeV]$} & \thead{Mesons \\ Pair} & \thead{Meson \\ Threshold \\ $[MeV]$} & \thead{Baryon \\ Anti-\\baryon} & \thead{Baryonic \\ Threshold \\ $[MeV]$} & \thead{Genuine} \\
  \hline
  \hline
\makecell{$11-31$\\$34-67$} & \makecell{$\eta_{c}(1S) \pi^{-}$ \\ $D^{0} D^{-}$} & \makecell{$3124$ \\ $3735$} & \makecell{$\Lambda^{+}_{c} \bar{\Sigma}^{--}_{c}$ \\ $\Sigma^{0}_{c} \bar{\Lambda}^{-}_{c}$ \\ $\Xi^{0}_{c} \bar{\Xi}^{-}_{c}$} & \makecell{$4740$ \\ $4740$ \\ $4938$} & $*$ \\
\hline
  \caption{$T_{c\bar{c}d\bar{u}}$ thresholds.} \label{table:Tcdcu_thresholds}
 \end{longtable}

==> tetraquarks/predictions/cd-dd/j_predictions.tex <==
\begin{longtable}[c]{|c|c|}
  \hline
  \thead{$J$ \\ Spec} & \thead{$a_{T_{j}}$} \\
  \hline
  \hline
\makecell{$2637-2782$\\$2974-3098$\\$3266-3376$\\$3528-3628$\\$3767-3860$\\$3990-4076$\\$4198-4280$\\$4395-4473$\\$4582-4656$\\$4761-4832$\\$4933-5001$\\$5098-5163$} & \makecell{$-1.6$-$-1.2$} \\
\hline
  \caption{$T_{c\bar{d}d\bar{d}}$ $(J, M^2)$ predictions.} \label{table:Tcddd_j_predictions}
 \end{longtable}

==> tetraquarks/predictions/cd-dd/n_predictions.tex <==
\begin{longtable}[c]{|c|c|}
  \hline
  \thead{$n$ \\ Spec} & \thead{$a_{T_{n}}$} \\
  \hline
  \hline
\makecell{$2273-2451$\\$2831-2963$\\$3266-3376$\\$3637-3733$\\$3966-4053$\\$4265-4345$\\$4541-4616$\\$4800-4870$\\$5043-5110$\\$5274-5338$\\$5495-5555$\\$5706-5764$} & \makecell{$-1.2$-$-0.93$} \\
\hline
  \caption{$T_{c\bar{d}d\bar{d}}$ $(n, M^2)$ predictions.} \label{table:Tcddd_n_predictions}
 \end{longtable}

==> tetraquarks/predictions/cd-dd/thresholds.tex <==
\begin{longtable}[c]{|c|c|c|c|c|c|}
  \hline
  \thead{Thry \\ Width \\ $[MeV]$} & \thead{Mesons \\ Pair} & \thead{Meson \\ Threshold \\ $[MeV]$} & \thead{Baryon \\ Anti-\\baryon} & \thead{Baryonic \\ Threshold \\ $[MeV]$} & \thead{Genuine} \\
  \hline
  \hline
\makecell{$78-117$\\$31-61$} & \makecell{$D^{+} \pi^{0}_{d}$} & \makecell{$2005$} & \makecell{$\Lambda^{+}_{c} \bar{n}$ \\ $\Xi^{0}_{c} \bar{\Sigma}^{+}$ \\ $\Sigma^{0}_{c} \bar{\Delta}^{+}$} & \makecell{$3226$ \\ $3667$ \\ $3686$} &  \\
\hline
  \caption{$T_{c\bar{d}d\bar{d}}$ thresholds.} \label{table:Tcddd_thresholds}
 \end{longtable}

==> tetraquarks/predictions/cd-ds/j_predictions.tex <==
\begin{longtable}[c]{|c|c|}
  \hline
  \thead{$J$ \\ Spec} & \thead{$a_{T_{j}}$} \\
  \hline
  \hline
\makecell{$2841-2983$\\$3162-3284$\\$3442-3552$\\$3695-3796$\\$3928-4021$\\$4144-4232$\\$4348-4431$\\$4541-4620$\\$4725-4800$\\$4900-4972$\\$5069-5138$\\$5231-5298$} & \makecell{$-1.8$-$-1.3$} \\
\hline
  \caption{$T_{c\bar{d}d\bar{s}}$ $(J, M^2)$ predictions.} \label{table:Tcdds_j_predictions}
 \end{longtable}

==> tetraquarks/predictions/cd-ds/n_predictions.tex <==
\begin{longtable}[c]{|c|c|}
  \hline
  \thead{$n$ \\ Spec} & \thead{$a_{T_{n}}$} \\
  \hline
  \hline
\makecell{$2502-2672$\\$3025-3155$\\$3442-3552$\\$3801-3898$\\$4121-4209$\\$4413-4495$\\$4685-4761$\\$4938-5010$\\$5178-5246$\\$5405-5470$\\$5623-5684$\\$5831-5890$} & \makecell{$-1.3$-$-1.0$} \\
\hline
  \caption{$T_{c\bar{d}d\bar{s}}$ $(n, M^2)$ predictions.} \label{table:Tcdds_n_predictions}
 \end{longtable}

==> tetraquarks/predictions/cd-ds/thresholds.tex <==
\begin{longtable}[c]{|c|c|c|c|c|c|}
  \hline
  \thead{Thry \\ Width \\ $[MeV]$} & \thead{Mesons \\ Pair} & \thead{Meson \\ Threshold \\ $[MeV]$} & \thead{Baryon \\ Anti-\\baryon} & \thead{Baryonic \\ Threshold \\ $[MeV]$} & \thead{Genuine} \\
  \hline
  \hline
\makecell{$121-195$\\$29-57$} & \makecell{$D^{+}_{s} \pi^{0}_{d}$ \\ $D^{+} K^{0}$} & \makecell{$2103$ \\ $2368$} & \makecell{$\Lambda^{+}_{c} \bar{\Lambda}^{0}$ \\ $\Sigma^{0}_{c} \bar{\Sigma}^{+}$ \\ $\Xi^{0}_{c} \bar{\Xi}^{+}$} & \makecell{$3402$ \\ $3651$ \\ $3792$} &  \\
\hline
  \caption{$T_{c\bar{d}d\bar{s}}$ thresholds.} \label{table:Tcdds_thresholds}
 \end{longtable}

==> tetraquarks/predictions/cd-du/spectrum.tex <==
\setlength\LTleft{-1.2cm}
\setlength\LTpre{0.5cm}
{\small\tabcolsep=1pt\footnotesize{\begin{longtable}[!c]{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
  \hline
  \thead{$\#$} & \thead{Candi-\\dates} & \thead{$J^{PC}$} & \thead{Quarks} & \thead{Thry \\ Width \\ $[MeV]$} & \thead{Mesons \\ Pair} & \thead{Meson \\ Threshold \\ $[MeV]$} & \thead{Baryon \\ Anti-\\baryon} & \thead{Baryonic \\ Threshold \\ $[MeV]$} & \thead{$J$ \\ Spec} & \thead{$n$ \\ Spec} & \thead{$a_{T_{j}}$ \\ $a_{T_{n}}$} & \thead{Thry \\ $J + n$} & \thead{Gen-\\uine} \\
  \hline
  \hline
1 & \makecell{$X(3500)$\\$X(3800)$} & \makecell{(${0}$ or ${1}$)$^{??}$\\$?^{??}$} & $c\bar{d}d\bar{u}$ & \makecell{$79-118$\\$30-61$} & \makecell{$D^{0} \pi^{0}_{d}$ \\ $D^{+} \pi^{-}$} & \makecell{$2000$ \\ $2010$} & \makecell{$\Lambda^{+}_{c} \bar{p}$ \\ $\Sigma^{0}_{c} \bar{n}$ \\ $\Xi^{0}_{c} \bar{\Lambda}^{0}$} & \makecell{$3224$ \\ $3394$ \\ $3586$} & \makecell{$2634-2779$\\$2972-3095$\\$3264-3374$\\$3526-3626$\\$3766-3858$} & \makecell{$2270-2448$\\$2829-2961$\\$3264-3374$\\$3635-3731$\\$3964-4051$} & \makecell{\makecell{$-1.6$-$-1.2$} \\ \makecell{$-1.2$-$-0.92$}} & \makecell{$3$ \\ $2$} &  \\
\hline
 \caption{Tetraquark predicted configurations and thresholds.} \label{table:charm_tetraquarks_predictions}
\end{longtable}}\normalsize}

==> tetraquarks/predictions/cd-ss/thresholds.tex <==
\begin{longtable}[c]{|c|c|c|c|c|c|}
  \hline
  \thead{Thry \\ Width \\ $[MeV]$} & \thead{Mesons \\ Pair} & \thead{Meson \\ Threshold \\ $[MeV]$} & \thead{Baryon \\ Anti-\\baryon} & \thead{Baryonic \\ Threshold \\ $[MeV]$} & \thead{Genuine} \\
  \hline
  \hline
\makecell{$168-307$\\$26-53$} & \makecell{$D^{+}_{s} K^{0}$} & \makecell{$2466$} & \makecell{$\Lambda^{+}_{c} \bar{\Xi}^{0}$ \\ $\Sigma^{0}_{c} \bar{\Xi}^{+}$ \\ $\Xi^{0}_{c} \bar{\Omega}^{+}$} & \makecell{$3601$ \\ $3776$ \\ $4142$} & $**$ \\
\hline
  \caption{$T_{c\bar{s}d\bar{s}}$ thresholds.} \label{table:Tcdss_thresholds}
 \end{longtable}

==> tetraquarks/predictions/cd-su/spectrum.tex <==
\setlength\LTleft{-1.2cm}
\setlength\LTpre{0.5cm}
{\small\tabcolsep=1pt\footnotesize{\begin{longtable}[!c]{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
  \hline
  \thead{$\#$} & \thead{Candi-\\dates} & \thead{$J^{PC}$} & \thead{Quarks} & \thead{Thry \\ Width \\ $[MeV]$} & \thead{Mesons \\ Pair} & \thead{Meson \\ Threshold \\ $[MeV]$} & \thead{Baryon \\ Anti-\\baryon} & \thead{Baryonic \\ Threshold \\ $[MeV]$} & \thead{$J$ \\ Spec} & \thead{$n$ \\ Spec} & \thead{$a_{T_{j}}$ \\ $a_{T_{n}}$} & \thead{Thry \\ $J + n$} & \thead{Gen-\\uine} \\
  \hline
  \hline
1 & \makecell{$T^{a}_{c\bar{s}0}(2900)^{0}$} & \makecell{$0^{?}$} & $c\bar{s}d\bar{u}$ & \makecell{$100-152$\\$29-59$} & \makecell{$D^{+}_{s} \pi^{-}$ \\ $D^{0} K^{0}$} & \makecell{$2108$ \\ $2363$} & \makecell{$\Lambda^{+}_{c} \bar{\Sigma}^{-}$ \\ $\Sigma^{0}_{c} \bar{\Lambda}^{0}$ \\ $\Xi^{0}_{c} \bar{\Xi}^{0}$} & \makecell{$3475$ \\ $3570$ \\ $3785$} & \makecell{$2936-3075$\\$3243-3365$\\$3515-3625$\\$3762-3863$\\$3990-4084$} & \makecell{$2616-2780$\\$3112-3240$\\$3515-3625$\\$3865-3963$\\$4179-4269$} & \makecell{\makecell{$-2.0$-$-1.6$} \\ \makecell{$-1.5$-$-1.2$}} & \makecell{$3$ \\ $2$} & $**$ \\
\hline
 \caption{Tetraquark predicted configurations and thresholds.} \label{table:charm_tetraquarks_predictions}
\end{longtable}}\normalsize}

==> tetraquarks/predictions/cd-su/thresholds.tex <==
\begin{longtable}[c]{|c|c|c|c|c|c|}
  \hline
  \thead{Thry \\ Width \\ $[MeV]$} & \thead{Mesons \\ Pair} & \thead{Meson \\ Threshold \\ $[MeV]$} & \thead{Baryon \\ Anti-\\baryon} & \thead{Baryonic \\ Threshold \\ $[MeV]$} & \thead{Genuine} \\
  \hline
  \hline
\makecell{$100-152$\\$29-59$} & \makecell{$D^{+}_{s} \pi^{-}$ \\ $D^{0} K^{0}$} & \makecell{$2108$ \\ $2363$} & \makecell{$\Lambda^{+}_{c} \bar{\Sigma}^{-}$ \\ $\Sigma^{0}_{c} \bar{\Lambda}^{0}$ \\ $\Xi^{0}_{c} \bar{\Xi}^{0}$} & \makecell{$3475$ \\ $3570$ \\ $3785$} & $**$ \\
\hline
  \caption{$T_{c\bar{s}d\bar{u}}$ thresholds.} \label{table:Tcdsu_thresholds}
 \end{longtable}

==> tetraquarks/predictions/cd-uu/thresholds.tex <==
\begin{longtable}[c]{|c|c|c|c|c|c|}
  \hline
  \thead{Thry \\ Width \\ $[MeV]$} & \thead{Mesons \\ Pair} & \thead{Meson \\ Threshold \\ $[MeV]$} & \thead{Baryon \\ Anti-\\baryon} & \thead{Baryonic \\ Threshold \\ $[MeV]$} & \thead{Genuine} \\
  \hline
  \hline
\makecell{$41-72$\\$32-63$} & \makecell{$D^{0} \pi^{-}$} & \makecell{$2005$} & \makecell{$\Sigma^{0}_{c} \bar{p}$ \\ $\Lambda^{+}_{c} \bar{\Delta}^{--}$ \\ $\Xi^{0}_{c} \bar{\Sigma}^{-}$} & \makecell{$3392$ \\ $3518$ \\ $3659$} & $**$ \\
\hline
  \caption{$T_{c\bar{u}d\bar{u}}$ thresholds.} \label{table:Tcduu_thresholds}
 \end{longtable}

==> tetraquarks/predictions/cs-bb/thresholds.tex <==
\begin{longtable}[c]{|c|c|c|c|c|c|}
  \hline
  \thead{Thry \\ Width \\ $[MeV]$} & \thead{Mesons \\ Pair} & \thead{Meson \\ Threshold \\ $[MeV]$} & \thead{Baryon \\ Anti-\\baryon} & \thead{Baryonic \\ Threshold \\ $[MeV]$} & \thead{Genuine} \\
  \hline
  \hline
 & \makecell{$B^{+}_{c} \bar{B}^{0}_{s}$} & \makecell{$11641$} & \makecell{$\Xi^{+}_{c} \bar{\Xi}^{0}_{bb}$ \\ $\Xi^{0}_{c} \bar{\Xi}^{+}_{bb}$ \\ $\Omega^{0}_{c} \bar{\Omega}^{+}_{bb}$} & \makecell{ \\  \\ } & $**$ \\
\hline
  \caption{$T_{c\bar{b}s\bar{b}}$ thresholds.} \label{table:Tcsbb_thresholds}
 \end{longtable}

==> tetraquarks/predictions/cs-bc/thresholds.tex <==
\begin{longtable}[c]{|c|c|c|c|c|c|}
  \hline
  \thead{Thry \\ Width \\ $[MeV]$} & \thead{Mesons \\ Pair} & \thead{Meson \\ Threshold \\ $[MeV]$} & \thead{Baryon \\ Anti-\\baryon} & \thead{Baryonic \\ Threshold \\ $[MeV]$} & \thead{Genuine} \\
  \hline
  \hline
 & \makecell{$B^{+}_{c} D^{-}_{s}$ \\ $\eta_{c}(1S) \bar{B}^{0}_{s}$} & \makecell{$8242$ \\ $8351$} & \makecell{$\Xi^{+}_{c} \bar{\Xi}^{-}_{bc}$ \\ $\Xi^{0}_{c} \bar{\Xi}^{0}_{bc}$ \\ $\Omega^{0}_{c} \bar{\Omega}^{0}_{bc}$} & \makecell{ \\  \\ } & $*$ \\
\hline
  \caption{$T_{c\bar{b}s\bar{c}}$ thresholds.} \label{table:Tcsbc_thresholds}
 \end{longtable}

==> tetraquarks/predictions/cs-bd/thresholds.tex <==
\begin{longtable}[c]{|c|c|c|c|c|c|}
  \hline
  \thead{Thry \\ Width \\ $[MeV]$} & \thead{Mesons \\ Pair} & \thead{Meson \\ Threshold \\ $[MeV]$} & \thead{Baryon \\ Anti-\\baryon} & \thead{Baryonic \\ Threshold \\ $[MeV]$} & \thead{Genuine} \\
  \hline
  \hline
 & \makecell{$B^{+}_{c} \bar{K}^{0}$ \\ $D^{+} \bar{B}^{0}_{s}$} & \makecell{$6772$ \\ $7237$} & \makecell{$\Xi^{0}_{c} \bar{\Sigma}^{+}_{b}$ \\ $\Omega^{0}_{c} \bar{\Xi}^{+}_{b}$ \\ $\Xi^{+}_{c} \bar{\Sigma}^{0}_{b}$} & \makecell{$8286$ \\ $8492$ \\ } & $**$ \\
\hline
  \caption{$T_{c\bar{b}s\bar{d}}$ thresholds.} \label{table:Tcsbd_thresholds}
 \end{longtable}

==> tetraquarks/predictions/cs-bs/j_predictions.tex <==
\begin{longtable}[c]{|c|c|}
  \hline
  \thead{$J$ \\ Spec} & \thead{$a_{T_{j}}$} \\
  \hline
  \hline
\makecell{$7915-8042$\\$8115-8232$\\$8300-8410$\\$8474-8578$\\$8638-8737$\\$8795-8889$\\$8944-9035$\\$9088-9176$\\$9227-9312$\\$9362-9444$\\$9492-9572$\\$9619-9696$} & \makecell{$-2.8$-$-2.2$} \\
\hline
  \caption{$T_{c\bar{b}s\bar{s}}$ $(J, M^2)$ predictions.} \label{table:Tcsbs_j_predictions}
 \end{longtable}

==> tetraquarks/predictions/cs-bs/n_predictions.tex <==
\begin{longtable}[c]{|c|c|}
  \hline
  \thead{$n$ \\ Spec} & \thead{$a_{T_{n}}$} \\
  \hline
  \hline
\makecell{$7722-7860$\\$8028-8150$\\$8300-8410$\\$8548-8649$\\$8778-8873$\\$8993-9083$\\$9197-9282$\\$9391-9473$\\$9577-9655$\\$9755-9831$\\$9928-10001$\\$10094-10165$} & \makecell{$-2.7$-$-2.3$} \\
\hline
  \caption{$T_{c\bar{b}s\bar{s}}$ $(n, M^2)$ predictions.} \label{table:Tcsbs_n_predictions}
 \end{longtable}

==> tetraquarks/predictions/cs-bs/thresholds.tex <==
\begin{longtable}[c]{|c|c|c|c|c|c|}
  \hline
  \thead{Thry \\ Width \\ $[MeV]$} & \thead{Mesons \\ Pair} & \thead{Meson \\ Threshold \\ $[MeV]$} & \thead{Baryon \\ Anti-\\baryon} & \thead{Baryonic \\ Threshold \\ $[MeV]$} & \thead{Genuine} \\
  \hline
  \hline
 & \makecell{$B^{+}_{c} \phi(1020)$ \\ $D^{+}_{s} \bar{B}^{0}_{s}$} & \makecell{$7293$ \\ $7335$} & \makecell{$\Xi^{+}_{c} \bar{\Xi}^{0}_{b}$ \\ $\Xi^{0}_{c} \bar{\Xi}^{+}_{b}$ \\ $\Omega^{0}_{c} \bar{\Omega}^{+}_{b}$} & \makecell{$8260$ \\ $8267$ \\ $8741$} &  \\
\hline
  \caption{$T_{c\bar{b}s\bar{s}}$ thresholds.} \label{table:Tcsbs_thresholds}
 \end{longtable}

==> tetraquarks/predictions/cs-bu/thresholds.tex <==
\begin{longtable}[c]{|c|c|c|c|c|c|}
  \hline
  \thead{Thry \\ Width \\ $[MeV]$} & \thead{Mesons \\ Pair} & \thead{Meson \\ Threshold \\ $[MeV]$} & \thead{Baryon \\ Anti-\\baryon} & \thead{Baryonic \\ Threshold \\ $[MeV]$} & \thead{Genuine} \\
  \hline
  \hline
 & \makecell{$B^{+}_{c} K^{-}$ \\ $D^{0} \bar{B}^{0}_{s}$} & \makecell{$6768$ \\ $7232$} & \makecell{$\Xi^{+}_{c} \bar{\Sigma}^{-}_{b}$ \\ $\Omega^{0}_{c} \bar{\Xi}^{0}_{b}$ \\ $\Xi^{0}_{c} \bar{\Sigma}^{0}_{b}$} & \makecell{$8279$ \\ $8487$ \\ } & $**$ \\
\hline
  \caption{$T_{c\bar{b}s\bar{u}}$ thresholds.} \label{table:Tcsbu_thresholds}
 \end{longtable}

==> tetraquarks/predictions/cs-cd/thresholds.tex <==
\begin{longtable}[c]{|c|c|c|c|c|c|}
  \hline
  \thead{Thry \\ Width \\ $[MeV]$} & \thead{Mesons \\ Pair} & \thead{Meson \\ Threshold \\ $[MeV]$} & \thead{Baryon \\ Anti-\\baryon} & \thead{Baryonic \\ Threshold \\ $[MeV]$} & \thead{Genuine} \\
  \hline
  \hline
\makecell{$47-80$\\$29-59$} & \makecell{$\eta_{c}(1S) \bar{K}^{0}$ \\ $D^{+} D^{-}_{s}$} & \makecell{$3482$ \\ $3838$} & \makecell{$\Xi^{+}_{c} \bar{\Lambda}^{-}_{c}$ \\ $\Xi^{0}_{c} \bar{\Sigma}^{0}_{c}$ \\ $\Omega^{0}_{c} \bar{\Xi}^{0}_{c}$} & \makecell{$4754$ \\ $4924$ \\ $5165$} & $*$ \\
\hline
  \caption{$T_{c\bar{c}s\bar{d}}$ thresholds.} \label{table:Tcscd_thresholds}
 \end{longtable}

==> tetraquarks/predictions/cs-cs/spectrum.tex <==
\setlength\LTleft{-1.2cm}
\setlength\LTpre{0.5cm}
{\small\tabcolsep=1pt\footnotesize{\begin{longtable}[!c]{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
  \hline
  \thead{$\#$} & \thead{Candi-\\dates} & \thead{$J^{PC}$} & \thead{Quarks} & \thead{Thry \\ Width \\ $[MeV]$} & \thead{Mesons \\ Pair} & \thead{Meson \\ Threshold \\ $[MeV]$} & \thead{Baryon \\ Anti-\\baryon} & \thead{Baryonic \\ Threshold \\ $[MeV]$} & \thead{$J$ \\ Spec} & \thead{$n$ \\ Spec} & \thead{$a_{T_{j}}$ \\ $a_{T_{n}}$} & \thead{Thry \\ $J + n$} & \thead{Gen-\\uine} \\
  \hline
  \hline
1 & \makecell{$X(3960)$\\$X(4140)$\\$X(4274)$\\$\chi_{c0}(4500)$\\$\chi_{c1}(4685)$\\$\chi_{c0}(4700)$\\$X(4350)$\\$X(4630)$\\$\psi(4360)$\\$\psi(4660)$} & \makecell{$0^{++}$\\$1^{++}$\\$1^{++}$\\$0^{++}$\\$1^{++}$\\$0^{++}$\\$?^{?+}$\\$1^{-+}$\\$1^{--}$\\$1^{--}$} & $c\bar{c}s\bar{s}$ & \makecell{$89-134$\\$27-54$} & \makecell{$D^{+}_{s} D^{-}_{s}$ \\ $\eta_{c}(1S) \phi(1020)$} & \makecell{$3936$ \\ $4003$} & \makecell{$\Xi^{+}_{c} \bar{\Xi}^{-}_{c}$ \\ $\Xi^{0}_{c} \bar{\Xi}^{0}_{c}$ \\ $\Omega^{0}_{c} \bar{\Omega}^{0}_{c}$} & \makecell{$4936$ \\ $4940$ \\ $5390$} & \makecell{$4536-4664$\\$4765-4882$\\$4976-5086$\\$5174-5278$\\$5361-5459$} & \makecell{$4315-4454$\\$4666-4787$\\$4976-5086$\\$5258-5359$\\$5519-5613$} & \makecell{\makecell{$-3.8$-$-3.2$} \\ \makecell{$-2.7$-$-2.3$}} & \makecell{$3$ \\ $2$} &  \\
\hline
 \caption{Tetraquark predicted configurations and thresholds.} \label{table:charm_tetraquarks_predictions}
\end{longtable}}\normalsize}

==> tetraquarks/predictions/cs-cu/thresholds.tex <==
\begin{longtable}[c]{|c|c|c|c|c|c|}
  \hline
  \thead{Thry \\ Width \\ $[MeV]$} & \thead{Mesons \\ Pair} & \thead{Meson \\ Threshold \\ $[MeV]$} & \thead{Baryon \\ Anti-\\baryon} & \thead{Baryonic \\ Threshold \\ $[MeV]$} & \thead{Genuine} \\
  \hline
  \hline
\makecell{$47-79$\\$29-59$} & \makecell{$\eta_{c}(1S) K^{-}$ \\ $D^{0} D^{-}_{s}$} & \makecell{$3478$ \\ $3833$} & \makecell{$\Xi^{0}_{c} \bar{\Lambda}^{-}_{c}$ \\ $\Xi^{+}_{c} \bar{\Sigma}^{--}_{c}$ \\ $\Omega^{0}_{c} \bar{\Xi}^{-}_{c}$} & \makecell{$4756$ \\ $4922$ \\ $5163$} & $*$ \\
\hline
  \caption{$T_{c\bar{c}s\bar{u}}$ thresholds.} \label{table:Tcscu_thresholds}
 \end{longtable}

==> tetraquarks/predictions/cs-dd/thresholds.tex <==
\begin{longtable}[c]{|c|c|c|c|c|c|}
  \hline
  \thead{Thry \\ Width \\ $[MeV]$} & \thead{Mesons \\ Pair} & \thead{Meson \\ Threshold \\ $[MeV]$} & \thead{Baryon \\ Anti-\\baryon} & \thead{Baryonic \\ Threshold \\ $[MeV]$} & \thead{Genuine} \\
  \hline
  \hline
\makecell{$127-208$\\$27-54$} & \makecell{$D^{+} \bar{K}^{0}$} & \makecell{$2368$} & \makecell{$\Xi^{+}_{c} \bar{n}$ \\ $\Xi^{0}_{c} \bar{\Delta}^{+}$ \\ $\Omega^{0}_{c} \bar{\Sigma}^{+}$} & \makecell{$3408$ \\ $3702$ \\ $3892$} & $**$ \\
\hline
  \caption{$T_{c\bar{d}s\bar{d}}$ thresholds.} \label{table:Tcsdd_thresholds}
 \end{longtable}

==> tetraquarks/predictions/cs-ds/j_predictions.tex <==
\begin{longtable}[c]{|c|c|}
  \hline
  \thead{$J$ \\ Spec} & \thead{$a_{T_{j}}$} \\
  \hline
  \hline
\makecell{$3001-3148$\\$3336-3460$\\$3624-3734$\\$3881-3981$\\$4117-4209$\\$4335-4421$\\$4539-4621$\\$4733-4810$\\$4916-4990$\\$5092-5163$\\$5260-5328$\\$5422-5488$} & \makecell{$-1.3$-$-0.9$} \\
\hline
  \caption{$T_{c\bar{d}s\bar{s}}$ $(J, M^2)$ predictions.} \label{table:Tcsds_j_predictions}
 \end{longtable}

==> tetraquarks/predictions/cs-ds/n_predictions.tex <==
\begin{longtable}[c]{|c|c|}
  \hline
  \thead{$n$ \\ Spec} & \thead{$a_{T_{n}}$} \\
  \hline
  \hline
\makecell{$2632-2817$\\$3194-3327$\\$3624-3734$\\$3988-4085$\\$4311-4398$\\$4605-4685$\\$4876-4951$\\$5130-5200$\\$5369-5435$\\$5596-5659$\\$5812-5873$\\$6020-6078$} & \makecell{$-0.99$-$-0.7$} \\
\hline
  \caption{$T_{c\bar{d}s\bar{s}}$ $(n, M^2)$ predictions.} \label{table:Tcsds_n_predictions}
 \end{longtable}

==> tetraquarks/predictions/cs-ds/thresholds.tex <==
\begin{longtable}[c]{|c|c|c|c|c|c|}
  \hline
  \thead{Thry \\ Width \\ $[MeV]$} & \thead{Mesons \\ Pair} & \thead{Meson \\ Threshold \\ $[MeV]$} & \thead{Baryon \\ Anti-\\baryon} & \thead{Baryonic \\ Threshold \\ $[MeV]$} & \thead{Genuine} \\
  \hline
  \hline
\makecell{$178-332$\\$25-51$} & \makecell{$D^{+}_{s} \bar{K}^{0}$ \\ $D^{+} \phi(1020)$} & \makecell{$2466$ \\ $2889$} & \makecell{$\Xi^{+}_{c} \bar{\Lambda}^{0}$ \\ $\Xi^{0}_{c} \bar{\Sigma}^{+}$ \\ $\Omega^{0}_{c} \bar{\Xi}^{+}$} & \makecell{$3584$ \\ $3667$ \\ $4017$} &  \\
\hline
  \caption{$T_{c\bar{d}s\bar{s}}$ thresholds.} \label{table:Tcsds_thresholds}
 \end{longtable}

==> tetraquarks/predictions/cs-du/spectrum.tex <==
\setlength\LTleft{-1.2cm}
\setlength\LTpre{0.5cm}
{\small\tabcolsep=1pt\footnotesize{\begin{longtable}[!c]{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
  \hline
  \thead{$\#$} & \thead{Candi-\\dates} & \thead{$J^{PC}$} & \thead{Quarks} & \thead{Thry \\ Width \\ $[MeV]$} & \thead{Mesons \\ Pair} & \thead{Meson \\ Threshold \\ $[MeV]$} & \thead{Baryon \\ Anti-\\baryon} & \thead{Baryonic \\ Threshold \\ $[MeV]$} & \thead{$J$ \\ Spec} & \thead{$n$ \\ Spec} & \thead{$a_{T_{j}}$ \\ $a_{T_{n}}$} & \thead{Thry \\ $J + n$} & \thead{Gen-\\uine} \\
  \hline
  \hline
1 & \makecell{$T_{cs0}(2900)^{0}$} & \makecell{$0^{+}$} & $c\bar{d}s\bar{u}$ & \makecell{$127-210$\\$27-54$} & \makecell{$D^{0} \bar{K}^{0}$ \\ $D^{+} K^{-}$} & \makecell{$2363$ \\ $2364$} & \makecell{$\Xi^{+}_{c} \bar{p}$ \\ $\Xi^{0}_{c} \bar{n}$ \\ $\Omega^{0}_{c} \bar{\Lambda}^{0}$} & \makecell{$3406$ \\ $3410$ \\ $3811$} & \makecell{$2790-2941$\\$3145-3270$\\$3446-3556$\\$3713-3812$\\$3955-4047$} & \makecell{$3446-3556$\\$3823-3919$\\$4155-4241$\\$4456-4535$\\$4733-4806$} & \makecell{\makecell{$-2.2$-$-1.8$} \\ \makecell{$-1.9$-$-1.6$}} & \makecell{$2$ \\ $1$} & $**$ \\
\hline
 \caption{Tetraquark predicted configurations and thresholds.} \label{table:charm_tetraquarks_predictions}
\end{longtable}}\normalsize}

==> tetraquarks/predictions/cs-du/thresholds.tex <==
\begin{longtable}[c]{|c|c|c|c|c|c|}
  \hline
  \thead{Thry \\ Width \\ $[MeV]$} & \thead{Mesons \\ Pair} & \thead{Meson \\ Threshold \\ $[MeV]$} & \thead{Baryon \\ Anti-\\baryon} & \thead{Baryonic \\ Threshold \\ $[MeV]$} & \thead{Genuine} \\
  \hline
  \hline
\makecell{$127-210$\\$27-54$} & \makecell{$D^{0} \bar{K}^{0}$ \\ $D^{+} K^{-}$} & \makecell{$2363$ \\ $2364$} & \makecell{$\Xi^{+}_{c} \bar{p}$ \\ $\Xi^{0}_{c} \bar{n}$ \\ $\Omega^{0}_{c} \bar{\Lambda}^{0}$} & \makecell{$3406$ \\ $3410$ \\ $3811$} & $**$ \\
\hline
  \caption{$T_{c\bar{d}s\bar{u}}$ thresholds.} \label{table:Tcsdu_thresholds}
 \end{longtable}

==> tetraquarks/predictions/cs-ss/j_predictions.tex <==
\begin{longtable}[c]{|c|c|}
  \hline
  \thead{$J$ \\ Spec} & \thead{$a_{T_{j}}$} \\
  \hline
  \hline
\makecell{$3214-3360$\\$3541-3665$\\$3823-3933$\\$4075-4175$\\$4306-4399$\\$4520-4607$\\$4721-4803$\\$4912-4990$\\$5093-5167$\\$5266-5337$\\$5432-5500$\\$5592-5658$} & \makecell{$-2.2$-$-1.8$} \\
\hline
  \caption{$T_{c\bar{s}s\bar{s}}$ $(J, M^2)$ predictions.} \label{table:Tcsss_j_predictions}
 \end{longtable}

==> tetraquarks/predictions/cs-ss/n_predictions.tex <==
\begin{longtable}[c]{|c|c|}
  \hline
  \thead{$n$ \\ Spec} & \thead{$a_{T_{n}}$} \\
  \hline
  \hline
\makecell{$3823-3933$\\$4180-4277$\\$4497-4585$\\$4786-4866$\\$5053-5128$\\$5303-5374$\\$5539-5606$\\$5763-5827$\\$5977-6038$\\$6182-6241$\\$6379-6436$\\$6569-6624$} & \makecell{$-1.9$-$-1.6$} \\
\hline
  \caption{$T_{c\bar{s}s\bar{s}}$ $(n, M^2)$ predictions.} \label{table:Tcsss_n_predictions}
 \end{longtable}

==> tetraquarks/predictions/cs-ss/thresholds.tex <==
\begin{longtable}[c]{|c|c|c|c|c|c|}
  \hline
  \thead{Thry \\ Width \\ $[MeV]$} & \thead{Mesons \\ Pair} & \thead{Meson \\ Threshold \\ $[MeV]$} & \thead{Baryon \\ Anti-\\baryon} & \thead{Baryonic \\ Threshold \\ $[MeV]$} & \thead{Genuine} \\
  \hline
  \hline
\makecell{$242-504$\\$23-47$} & \makecell{$D^{+}_{s} \phi(1020)$} & \makecell{$2987$} & \makecell{$\Xi^{+}_{c} \bar{\Xi}^{0}$ \\ $\Xi^{0}_{c} \bar{\Xi}^{+}$ \\ $\Omega^{0}_{c} \bar{\Omega}^{+}$} & \makecell{$3783$ \\ $3792$ \\ $4367$} &  \\
\hline
  \caption{$T_{c\bar{s}s\bar{s}}$ thresholds.} \label{table:Tcsss_thresholds}
 \end{longtable}

==> tetraquarks/predictions/cs-su/j_predictions.tex <==
\begin{longtable}[c]{|c|c|}
  \hline
  \thead{$J$ \\ Spec} & \thead{$a_{T_{j}}$} \\
  \hline
  \hline
\makecell{$3004-3150$\\$3338-3462$\\$3626-3736$\\$3883-3983$\\$4118-4211$\\$4336-4423$\\$4541-4622$\\$4734-4811$\\$4918-4992$\\$5093-5164$\\$5262-5330$\\$5424-5489$} & \makecell{$-1.3$-$-0.91$} \\
\hline
  \caption{$T_{c\bar{s}s\bar{u}}$ $(J, M^2)$ predictions.} \label{table:Tcssu_j_predictions}
 \end{longtable}

==> tetraquarks/predictions/cs-su/n_predictions.tex <==
\begin{longtable}[c]{|c|c|}
  \hline
  \thead{$n$ \\ Spec} & \thead{$a_{T_{n}}$} \\
  \hline
  \hline
\makecell{$2636-2820$\\$3197-3329$\\$3626-3736$\\$3990-4086$\\$4313-4400$\\$4606-4686$\\$4878-4952$\\$5131-5201$\\$5370-5437$\\$5597-5660$\\$5813-5874$\\$6021-6079$} & \makecell{$-1.0$-$-0.71$} \\
\hline
  \caption{$T_{c\bar{s}s\bar{u}}$ $(n, M^2)$ predictions.} \label{table:Tcssu_n_predictions}
 \end{longtable}

==> tetraquarks/predictions/cs-su/thresholds.tex <==
\begin{longtable}[c]{|c|c|c|c|c|c|}
  \hline
  \thead{Thry \\ Width \\ $[MeV]$} & \thead{Mesons \\ Pair} & \thead{Meson \\ Threshold \\ $[MeV]$} & \thead{Baryon \\ Anti-\\baryon} & \thead{Baryonic \\ Threshold \\ $[MeV]$} & \thead{Genuine} \\
  \hline
  \hline
\makecell{$178-330$\\$25-51$} & \makecell{$D^{+}_{s} K^{-}$ \\ $D^{0} \phi(1020)$} & \makecell{$2462$ \\ $2884$} & \makecell{$\Xi^{0}_{c} \bar{\Lambda}^{0}$ \\ $\Xi^{+}_{c} \bar{\Sigma}^{-}$ \\ $\Omega^{0}_{c} \bar{\Xi}^{0}$} & \makecell{$3586$ \\ $3657$ \\ $4010$} &  \\
\hline
  \caption{$T_{c\bar{s}s\bar{u}}$ thresholds.} \label{table:Tcssu_thresholds}
 \end{longtable}

==> tetraquarks/predictions/cs-uu/thresholds.tex <==
\begin{longtable}[c]{|c|c|c|c|c|c|}
  \hline
  \thead{Thry \\ Width \\ $[MeV]$} & \thead{Mesons \\ Pair} & \thead{Meson \\ Threshold \\ $[MeV]$} & \thead{Baryon \\ Anti-\\baryon} & \thead{Baryonic \\ Threshold \\ $[MeV]$} & \thead{Genuine} \\
  \hline
  \hline
\makecell{$127-208$\\$27-54$} & \makecell{$D^{0} K^{-}$} & \makecell{$2359$} & \makecell{$\Xi^{0}_{c} \bar{p}$ \\ $\Xi^{+}_{c} \bar{\Delta}^{--}$ \\ $\Omega^{0}_{c} \bar{\Sigma}^{-}$} & \makecell{$3408$ \\ $3700$ \\ $3884$} & $**$ \\
\hline
  \caption{$T_{c\bar{u}s\bar{u}}$ thresholds.} \label{table:Tcsuu_thresholds}
 \end{longtable}

==> tetraquarks/predictions/cu-bb/thresholds.tex <==
\begin{longtable}[c]{|c|c|c|c|c|c|}
  \hline
  \thead{Thry \\ Width \\ $[MeV]$} & \thead{Mesons \\ Pair} & \thead{Meson \\ Threshold \\ $[MeV]$} & \thead{Baryon \\ Anti-\\baryon} & \thead{Baryonic \\ Threshold \\ $[MeV]$} & \thead{Genuine} \\
  \hline
  \hline
 & \makecell{$B^{+}_{c} B^{-}$} & \makecell{$11553$} & \makecell{$\Sigma^{++}_{c} \bar{\Xi}^{0}_{bb}$ \\ $\Lambda^{+}_{c} \bar{\Xi}^{+}_{bb}$ \\ $\Xi^{+}_{c} \bar{\Omega}^{+}_{bb}$} & \makecell{ \\  \\ } & $**$ \\
\hline
  \caption{$T_{c\bar{b}u\bar{b}}$ thresholds.} \label{table:Tcubb_thresholds}
 \end{longtable}

==> tetraquarks/predictions/cu-bc/thresholds.tex <==
\begin{longtable}[c]{|c|c|c|c|c|c|}
  \hline
  \thead{Thry \\ Width \\ $[MeV]$} & \thead{Mesons \\ Pair} & \thead{Meson \\ Threshold \\ $[MeV]$} & \thead{Baryon \\ Anti-\\baryon} & \thead{Baryonic \\ Threshold \\ $[MeV]$} & \thead{Genuine} \\
  \hline
  \hline
 & \makecell{$B^{+}_{c} \bar{D}^{0}$ \\ $\eta_{c}(1S) B^{-}$} & \makecell{$8139$ \\ $8263$} & \makecell{$\Sigma^{++}_{c} \bar{\Xi}^{-}_{bc}$ \\ $\Lambda^{+}_{c} \bar{\Xi}^{0}_{bc}$ \\ $\Xi^{+}_{c} \bar{\Omega}^{0}_{bc}$} & \makecell{ \\  \\ } & $*$ \\
\hline
  \caption{$T_{c\bar{b}u\bar{c}}$ thresholds.} \label{table:Tcubc_thresholds}
 \end{longtable}

==> tetraquarks/predictions/cu-bd/thresholds.tex <==
\begin{longtable}[c]{|c|c|c|c|c|c|}
  \hline
  \thead{Thry \\ Width \\ $[MeV]$} & \thead{Mesons \\ Pair} & \thead{Meson \\ Threshold \\ $[MeV]$} & \thead{Baryon \\ Anti-\\baryon} & \thead{Baryonic \\ Threshold \\ $[MeV]$} & \thead{Genuine} \\
  \hline
  \hline
 & \makecell{$B^{+}_{c} \pi^{+}$ \\ $D^{+} B^{-}$} & \makecell{$6414$ \\ $7149$} & \makecell{$\Lambda^{+}_{c} \bar{\Sigma}^{+}_{b}$ \\ $\Xi^{+}_{c} \bar{\Xi}^{+}_{b}$ \\ $\Sigma^{++}_{c} \bar{\Sigma}^{0}_{b}$} & \makecell{$8102$ \\ $8265$ \\ } & $**$ \\
\hline
  \caption{$T_{c\bar{b}u\bar{d}}$ thresholds.} \label{table:Tcubd_thresholds}
 \end{longtable}

==> tetraquarks/predictions/cu-bs/thresholds.tex <==
\begin{longtable}[c]{|c|c|c|c|c|c|}
  \hline
  \thead{Thry \\ Width \\ $[MeV]$} & \thead{Mesons \\ Pair} & \thead{Meson \\ Threshold \\ $[MeV]$} & \thead{Baryon \\ Anti-\\baryon} & \thead{Baryonic \\ Threshold \\ $[MeV]$} & \thead{Genuine} \\
  \hline
  \hline
 & \makecell{$B^{+}_{c} K^{+}$ \\ $D^{+}_{s} B^{-}$} & \makecell{$6768$ \\ $7247$} & \makecell{$\Lambda^{+}_{c} \bar{\Xi}^{+}_{b}$ \\ $\Sigma^{++}_{c} \bar{\Xi}^{0}_{b}$ \\ $\Xi^{+}_{c} \bar{\Omega}^{+}_{b}$} & \makecell{$8083$ \\ $8246$ \\ $8514$} & $**$ \\
\hline
  \caption{$T_{c\bar{b}u\bar{s}}$ thresholds.} \label{table:Tcubs_thresholds}
 \end{longtable}

==> tetraquarks/predictions/cu-bu/j_predictions.tex <==
\begin{longtable}[c]{|c|c|}
  \hline
  \thead{$J$ \\ Spec} & \thead{$a_{T_{j}}$} \\
  \hline
  \hline
\makecell{$7978-8099$\\$8143-8258$\\$8300-8410$\\$8451-8556$\\$8595-8698$\\$8735-8834$\\$8871-8967$\\$9002-9095$\\$9130-9220$\\$9254-9343$\\$9375-9462$\\$9494-9578$} & \makecell{$-2.5$-$-1.8$} \\
\hline
  \caption{$T_{c\bar{b}u\bar{u}}$ $(J, M^2)$ predictions.} \label{table:Tcubu_j_predictions}
 \end{longtable}

==> tetraquarks/predictions/cu-bu/n_predictions.tex <==
\begin{longtable}[c]{|c|c|}
  \hline
  \thead{$n$ \\ Spec} & \thead{$a_{T_{n}}$} \\
  \hline
  \hline
\makecell{$7825-7951$\\$8071-8188$\\$8300-8410$\\$8516-8620$\\$8720-8819$\\$8915-9010$\\$9102-9193$\\$9281-9369$\\$9455-9540$\\$9622-9705$\\$9785-9865$\\$9943-10021$} & \makecell{$-2.3$-$-1.8$} \\
\hline
  \caption{$T_{c\bar{b}u\bar{u}}$ $(n, M^2)$ predictions.} \label{table:Tcubu_n_predictions}
 \end{longtable}

==> tetraquarks/predictions/cu-bu/thresholds.tex <==
\begin{longtable}[c]{|c|c|c|c|c|c|}
  \hline
  \thead{Thry \\ Width \\ $[MeV]$} & \thead{Mesons \\ Pair} & \thead{Meson \\ Threshold \\ $[MeV]$} & \thead{Baryon \\ Anti-\\baryon} & \thead{Baryonic \\ Threshold \\ $[MeV]$} & \thead{Genuine} \\
  \hline
  \hline
 & \makecell{$B^{+}_{c} \pi^{0}_{u}$ \\ $D^{0} B^{-}$} & \makecell{$6409$ \\ $7144$} & \makecell{$\Xi^{+}_{c} \bar{\Xi}^{0}_{b}$ \\ $\Sigma^{++}_{c} \bar{\Sigma}^{-}_{b}$ \\ $\Lambda^{+}_{c} \bar{\Sigma}^{0}_{b}$} & \makecell{$8260$ \\ $8265$ \\ } &  \\
\hline
  \caption{$T_{c\bar{b}u\bar{u}}$ thresholds.} \label{table:Tcubu_thresholds}
 \end{longtable}

==> tetraquarks/predictions/cu-cd/spectrum.tex <==
\setlength\LTleft{-1.2cm}
\setlength\LTpre{0.5cm}
{\small\tabcolsep=1pt\footnotesize{\begin{longtable}[!c]{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
  \hline
  \thead{$\#$} & \thead{Candi-\\dates} & \thead{$J^{PC}$} & \thead{Quarks} & \thead{Thry \\ Width \\ $[MeV]$} & \thead{Mesons \\ Pair} & \thead{Meson \\ Threshold \\ $[MeV]$} & \thead{Baryon \\ Anti-\\baryon} & \thead{Baryonic \\ Threshold \\ $[MeV]$} & \thead{$J$ \\ Spec} & \thead{$n$ \\ Spec} & \thead{$a_{T_{j}}$ \\ $a_{T_{n}}$} & \thead{Thry \\ $J + n$} & \thead{Gen-\\uine} \\
  \hline
  \hline
1 & \makecell{} & \makecell{} & $c\bar{c}u\bar{d}$ & \makecell{$11-31$\\$34-67$} & \makecell{$\eta_{c}(1S) \pi^{+}$ \\ $D^{+} \bar{D}^{0}$} & \makecell{$3124$ \\ $3735$} & \makecell{$\Sigma^{++}_{c} \bar{\Lambda}^{-}_{c}$ \\ $\Lambda^{+}_{c} \bar{\Sigma}^{0}_{c}$ \\ $\Xi^{+}_{c} \bar{\Xi}^{0}_{c}$} & \makecell{$4740$ \\ $4740$ \\ $4938$} & \makecell{$4373-4497$\\$4583-4699$\\$4780-4890$\\$4967-5072$\\$5145-5245$} & \makecell{$4174-4306$\\$4491-4611$\\$4780-4890$\\$5047-5150$\\$5297-5394$} & \makecell{\makecell{$-2.6$-$-2.0$} \\ \makecell{$-2.0$-$-1.6$}} & \makecell{$6$ \\ $4$} & $*$ \\
\hline
 \caption{Tetraquark predicted configurations and thresholds.} \label{table:charm_tetraquarks_predictions}
\end{longtable}}\normalsize}

==> tetraquarks/predictions/cu-cs/spectrum.tex <==
\setlength\LTleft{-1.2cm}
\setlength\LTpre{0.5cm}
{\small\tabcolsep=1pt\footnotesize{\begin{longtable}[!c]{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
  \hline
  \thead{$\#$} & \thead{Candi-\\dates} & \thead{$J^{PC}$} & \thead{Quarks} & \thead{Thry \\ Width \\ $[MeV]$} & \thead{Mesons \\ Pair} & \thead{Meson \\ Threshold \\ $[MeV]$} & \thead{Baryon \\ Anti-\\baryon} & \thead{Baryonic \\ Threshold \\ $[MeV]$} & \thead{$J$ \\ Spec} & \thead{$n$ \\ Spec} & \thead{$a_{T_{j}}$ \\ $a_{T_{n}}$} & \thead{Thry \\ $J + n$} & \thead{Gen-\\uine} \\
  \hline
  \hline
1 & \makecell{$T_{\psi s1}^{\theta}(4000)^{+}$\\$T_{\psi s1}(4220)^{+}$\\$T_{\psi s1}^{\theta}(4000)^{0}$} & \makecell{$1^{+}$\\$1^{+}$\\$1^{+}$} & $c\bar{c}u\bar{s}$ & \makecell{$47-79$\\$29-59$} & \makecell{$\eta_{c}(1S) K^{+}$ \\ $D^{+}_{s} \bar{D}^{0}$} & \makecell{$3478$ \\ $3833$} & \makecell{$\Lambda^{+}_{c} \bar{\Xi}^{0}_{c}$ \\ $\Sigma^{++}_{c} \bar{\Xi}^{-}_{c}$ \\ $\Xi^{+}_{c} \bar{\Omega}^{0}_{c}$} & \makecell{$4756$ \\ $4922$ \\ $5163$} & \makecell{$4362-4488$\\$4587-4704$\\$4796-4906$\\$4993-5097$\\$5179-5278$} & \makecell{$4145-4282$\\$4489-4610$\\$4796-4906$\\$5076-5178$\\$5337-5432$} & \makecell{\makecell{$-3.3$-$-2.7$} \\ \makecell{$-2.0$-$-1.6$}} & \makecell{$4$ \\ $3$} & $*$ \\
\hline
 \caption{Tetraquark predicted configurations and thresholds.} \label{table:charm_tetraquarks_predictions}
\end{longtable}}\normalsize}

==> tetraquarks/predictions/cu-cu/j_predictions.tex <==
\begin{longtable}[c]{|c|c|}
  \hline
  \thead{$J$ \\ Spec} & \thead{$a_{T_{j}}$} \\
  \hline
  \hline
\makecell{$4182-4308$\\$4404-4521$\\$4612-4722$\\$4808-4912$\\$4993-5092$\\$5170-5265$\\$5340-5431$\\$5503-5591$\\$5660-5745$\\$5812-5894$\\$5959-6039$\\$6102-6180$} & \makecell{$-2.7$-$-2.2$} \\
\hline
  \caption{$T_{c\bar{c}u\bar{u}}$ $(J, M^2)$ predictions.} \label{table:Tcucu_j_predictions}
 \end{longtable}

==> tetraquarks/predictions/cu-cu/n_predictions.tex <==
\begin{longtable}[c]{|c|c|}
  \hline
  \thead{$n$ \\ Spec} & \thead{$a_{T_{n}}$} \\
  \hline
  \hline
\makecell{$3969-4104$\\$4308-4428$\\$4612-4722$\\$4891-4993$\\$5151-5246$\\$5395-5485$\\$5626-5711$\\$5845-5927$\\$6055-6134$\\$6257-6332$\\$6451-6524$\\$6639-6709$} & \makecell{$-2.3$-$-2.0$} \\
\hline
  \caption{$T_{c\bar{c}u\bar{u}}$ $(n, M^2)$ predictions.} \label{table:Tcucu_n_predictions}
 \end{longtable}

==> tetraquarks/predictions/cu-cu/thresholds.tex <==
\begin{longtable}[c]{|c|c|c|c|c|c|}
  \hline
  \thead{Thry \\ Width \\ $[MeV]$} & \thead{Mesons \\ Pair} & \thead{Meson \\ Threshold \\ $[MeV]$} & \thead{Baryon \\ Anti-\\baryon} & \thead{Baryonic \\ Threshold \\ $[MeV]$} & \thead{Genuine} \\
  \hline
  \hline
\makecell{$24-51$\\$32-64$} & \makecell{$\eta_{c}(1S) \pi^{0}_{u}$ \\ $D^{0} \bar{D}^{0}$} & \makecell{$3119$ \\ $3730$} & \makecell{$\Lambda^{+}_{c} \bar{\Lambda}^{-}_{c}$ \\ $\Sigma^{++}_{c} \bar{\Sigma}^{--}_{c}$ \\ $\Xi^{+}_{c} \bar{\Xi}^{-}_{c}$} & \makecell{$4572$ \\ $4908$ \\ $4936$} &  \\
\hline
  \caption{$T_{c\bar{c}u\bar{u}}$ thresholds.} \label{table:Tcucu_thresholds}
 \end{longtable}

==> tetraquarks/predictions/cu-dd/thresholds.tex <==
\begin{longtable}[c]{|c|c|c|c|c|c|}
  \hline
  \thead{Thry \\ Width \\ $[MeV]$} & \thead{Mesons \\ Pair} & \thead{Meson \\ Threshold \\ $[MeV]$} & \thead{Baryon \\ Anti-\\baryon} & \thead{Baryonic \\ Threshold \\ $[MeV]$} & \thead{Genuine} \\
  \hline
  \hline
\makecell{$40-71$\\$32-63$} & \makecell{$D^{+} \pi^{+}$} & \makecell{$2010$} & \makecell{$\Sigma^{++}_{c} \bar{n}$ \\ $\Lambda^{+}_{c} \bar{\Delta}^{+}$ \\ $\Xi^{+}_{c} \bar{\Sigma}^{+}$} & \makecell{$3394$ \\ $3518$ \\ $3665$} & $**$ \\
\hline
  \caption{$T_{c\bar{d}u\bar{d}}$ thresholds.} \label{table:Tcudd_thresholds}
 \end{longtable}

==> tetraquarks/predictions/cu-ds/spectrum.tex <==
\setlength\LTleft{-1.2cm}
\setlength\LTpre{0.5cm}
{\small\tabcolsep=1pt\footnotesize{\begin{longtable}[!c]{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
  \hline
  \thead{$\#$} & \thead{Candi-\\dates} & \thead{$J^{PC}$} & \thead{Quarks} & \thead{Thry \\ Width \\ $[MeV]$} & \thead{Mesons \\ Pair} & \thead{Meson \\ Threshold \\ $[MeV]$} & \thead{Baryon \\ Anti-\\baryon} & \thead{Baryonic \\ Threshold \\ $[MeV]$} & \thead{$J$ \\ Spec} & \thead{$n$ \\ Spec} & \thead{$a_{T_{j}}$ \\ $a_{T_{n}}$} & \thead{Thry \\ $J + n$} & \thead{Gen-\\uine} \\
  \hline
  \hline
1 & \makecell{$T_{cs1}(2900)^{0}$\\$T^{a}_{c\bar{s}0}(2900)^{++}$} & \makecell{$1^{-}$\\$0^{?}$} & $c\bar{d}u\bar{s}$ & \makecell{$98-147$\\$29-59$} & \makecell{$D^{+}_{s} \pi^{+}$ \\ $D^{+} K^{+}$} & \makecell{$2108$ \\ $2364$} & \makecell{$\Lambda^{+}_{c} \bar{\Sigma}^{+}$ \\ $\Sigma^{++}_{c} \bar{\Lambda}^{0}$ \\ $\Xi^{+}_{c} \bar{\Xi}^{+}$} & \makecell{$3483$ \\ $3570$ \\ $3790$} & \makecell{$2946-3085$\\$3252-3374$\\$3523-3633$\\$3769-3870$\\$3996-4091$} & \makecell{$2628-2791$\\$3121-3250$\\$3523-3633$\\$3872-3970$\\$4186-4275$} & \makecell{\makecell{$-2.1$-$-1.6$} \\ \makecell{$-1.5$-$-1.2$}} & \makecell{$3$ \\ $2$} & $**$ \\
\hline
 \caption{Tetraquark predicted configurations and thresholds.} \label{table:charm_tetraquarks_predictions}
\end{longtable}}\normalsize}

==> tetraquarks/predictions/cu-ds/thresholds.tex <==
\begin{longtable}[c]{|c|c|c|c|c|c|}
  \hline
  \thead{Thry \\ Width \\ $[MeV]$} & \thead{Mesons \\ Pair} & \thead{Meson \\ Threshold \\ $[MeV]$} & \thead{Baryon \\ Anti-\\baryon} & \thead{Baryonic \\ Threshold \\ $[MeV]$} & \thead{Genuine} \\
  \hline
  \hline
\makecell{$98-147$\\$29-59$} & \makecell{$D^{+}_{s} \pi^{+}$ \\ $D^{+} K^{+}$} & \makecell{$2108$ \\ $2364$} & \makecell{$\Lambda^{+}_{c} \bar{\Sigma}^{+}$ \\ $\Sigma^{++}_{c} \bar{\Lambda}^{0}$ \\ $\Xi^{+}_{c} \bar{\Xi}^{+}$} & \makecell{$3483$ \\ $3570$ \\ $3790$} & $**$ \\
\hline
  \caption{$T_{c\bar{d}u\bar{s}}$ thresholds.} \label{table:Tcuds_thresholds}
 \end{longtable}

==> tetraquarks/predictions/cu-du/j_predictions.tex <==
\begin{longtable}[c]{|c|c|}
  \hline
  \thead{$J$ \\ Spec} & \thead{$a_{T_{j}}$} \\
  \hline
  \hline
\makecell{$2637-2782$\\$2974-3098$\\$3266-3376$\\$3528-3628$\\$3767-3860$\\$3990-4076$\\$4198-4280$\\$4395-4473$\\$4582-4656$\\$4761-4832$\\$4933-5001$\\$5098-5163$} & \makecell{$-1.6$-$-1.2$} \\
\hline
  \caption{$T_{c\bar{d}u\bar{u}}$ $(J, M^2)$ predictions.} \label{table:Tcudu_j_predictions}
 \end{longtable}

==> tetraquarks/predictions/cu-du/n_predictions.tex <==
\begin{longtable}[c]{|c|c|}
  \hline
  \thead{$n$ \\ Spec} & \thead{$a_{T_{n}}$} \\
  \hline
  \hline
\makecell{$2273-2451$\\$2831-2963$\\$3266-3376$\\$3637-3733$\\$3966-4053$\\$4265-4345$\\$4541-4616$\\$4800-4870$\\$5043-5110$\\$5274-5338$\\$5495-5555$\\$5706-5764$} & \makecell{$-1.2$-$-0.93$} \\
\hline
  \caption{$T_{c\bar{d}u\bar{u}}$ $(n, M^2)$ predictions.} \label{table:Tcudu_n_predictions}
 \end{longtable}

==> tetraquarks/predictions/cu-du/thresholds.tex <==
\begin{longtable}[c]{|c|c|c|c|c|c|}
  \hline
  \thead{Thry \\ Width \\ $[MeV]$} & \thead{Mesons \\ Pair} & \thead{Meson \\ Threshold \\ $[MeV]$} & \thead{Baryon \\ Anti-\\baryon} & \thead{Baryonic \\ Threshold \\ $[MeV]$} & \thead{Genuine} \\
  \hline
  \hline
\makecell{$78-117$\\$31-61$} & \makecell{$D^{+} \pi^{0}_{u}$ \\ $D^{0} \pi^{+}$} & \makecell{$2005$ \\ $2005$} & \makecell{$\Lambda^{+}_{c} \bar{n}$ \\ $\Sigma^{++}_{c} \bar{p}$ \\ $\Xi^{+}_{c} \bar{\Lambda}^{0}$} & \makecell{$3226$ \\ $3392$ \\ $3584$} &  \\
\hline
  \caption{$T_{c\bar{d}u\bar{u}}$ thresholds.} \label{table:Tcudu_thresholds}
 \end{longtable}

==> tetraquarks/predictions/cu-ss/thresholds.tex <==
\begin{longtable}[c]{|c|c|c|c|c|c|}
  \hline
  \thead{Thry \\ Width \\ $[MeV]$} & \thead{Mesons \\ Pair} & \thead{Meson \\ Threshold \\ $[MeV]$} & \thead{Baryon \\ Anti-\\baryon} & \thead{Baryonic \\ Threshold \\ $[MeV]$} & \thead{Genuine} \\
  \hline
  \hline
\makecell{$166-300$\\$27-53$} & \makecell{$D^{+}_{s} K^{+}$} & \makecell{$2462$} & \makecell{$\Lambda^{+}_{c} \bar{\Xi}^{+}$ \\ $\Sigma^{++}_{c} \bar{\Xi}^{0}$ \\ $\Xi^{+}_{c} \bar{\Omega}^{+}$} & \makecell{$3608$ \\ $3769$ \\ $4140$} & $**$ \\
\hline
  \caption{$T_{c\bar{s}u\bar{s}}$ thresholds.} \label{table:Tcuss_thresholds}
 \end{longtable}

==> tetraquarks/predictions/cu-su/j_predictions.tex <==
\begin{longtable}[c]{|c|c|}
  \hline
  \thead{$J$ \\ Spec} & \thead{$a_{T_{j}}$} \\
  \hline
  \hline
\makecell{$2841-2983$\\$3162-3284$\\$3442-3552$\\$3695-3796$\\$3928-4021$\\$4144-4232$\\$4348-4431$\\$4541-4620$\\$4725-4800$\\$4900-4972$\\$5069-5138$\\$5231-5298$} & \makecell{$-1.8$-$-1.3$} \\
\hline
  \caption{$T_{c\bar{s}u\bar{u}}$ $(J, M^2)$ predictions.} \label{table:Tcusu_j_predictions}
 \end{longtable}

==> tetraquarks/predictions/cu-su/n_predictions.tex <==
\begin{longtable}[c]{|c|c|}
  \hline
  \thead{$n$ \\ Spec} & \thead{$a_{T_{n}}$} \\
  \hline
  \hline
\makecell{$2502-2672$\\$3025-3155$\\$3442-3552$\\$3801-3898$\\$4121-4209$\\$4413-4495$\\$4685-4761$\\$4938-5010$\\$5178-5246$\\$5405-5470$\\$5623-5684$\\$5831-5890$} & \makecell{$-1.3$-$-1.0$} \\
\hline
  \caption{$T_{c\bar{s}u\bar{u}}$ $(n, M^2)$ predictions.} \label{table:Tcusu_n_predictions}
 \end{longtable}

==> tetraquarks/predictions/cu-su/spectrum.tex <==
\setlength\LTleft{-1.2cm}
\setlength\LTpre{0.5cm}
{\small\tabcolsep=1pt\footnotesize{\begin{longtable}[!c]{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
  \hline
  \thead{$\#$} & \thead{Candi-\\dates} & \thead{$J^{PC}$} & \thead{Quarks} & \thead{Thry \\ Width \\ $[MeV]$} & \thead{Mesons \\ Pair} & \thead{Meson \\ Threshold \\ $[MeV]$} & \thead{Baryon \\ Anti-\\baryon} & \thead{Baryonic \\ Threshold \\ $[MeV]$} & \thead{$J$ \\ Spec} & \thead{$n$ \\ Spec} & \thead{$a_{T_{j}}$ \\ $a_{T_{n}}$} & \thead{Thry \\ $J + n$} & \thead{Gen-\\uine} \\
  \hline
  \hline
1 & \makecell{$X(2632)$} & \makecell{$?^{??}$} & $c\bar{s}u\bar{u}$ & \makecell{$121-195$\\$29-57$} & \makecell{$D^{+}_{s} \pi^{0}_{u}$ \\ $D^{0} K^{+}$} & \makecell{$2103$ \\ $2359$} & \makecell{$\Lambda^{+}_{c} \bar{\Lambda}^{0}$ \\ $\Sigma^{++}_{c} \bar{\Sigma}^{-}$ \\ $\Xi^{+}_{c} \bar{\Xi}^{0}$} & \makecell{$3402$ \\ $3643$ \\ $3783$} & \makecell{$2841-2983$\\$3162-3284$\\$3442-3552$\\$3695-3796$\\$3928-4021$} & \makecell{$2502-2672$\\$3025-3155$\\$3442-3552$\\$3801-3898$\\$4121-4209$} & \makecell{\makecell{$-1.8$-$-1.3$} \\ \makecell{$-1.3$-$-1.0$}} & \makecell{$3$ \\ $2$} &  \\
\hline
 \caption{Tetraquark predicted configurations and thresholds.} \label{table:charm_tetraquarks_predictions}
\end{longtable}}\normalsize}

==> tetraquarks/predictions/cu-su/thresholds.tex <==
\begin{longtable}[c]{|c|c|c|c|c|c|}
  \hline
  \thead{Thry \\ Width \\ $[MeV]$} & \thead{Mesons \\ Pair} & \thead{Meson \\ Threshold \\ $[MeV]$} & \thead{Baryon \\ Anti-\\baryon} & \thead{Baryonic \\ Threshold \\ $[MeV]$} & \thead{Genuine} \\
  \hline
  \hline
\makecell{$121-195$\\$29-57$} & \makecell{$D^{+}_{s} \pi^{0}_{u}$ \\ $D^{0} K^{+}$} & \makecell{$2103$ \\ $2359$} & \makecell{$\Lambda^{+}_{c} \bar{\Lambda}^{0}$ \\ $\Sigma^{++}_{c} \bar{\Sigma}^{-}$ \\ $\Xi^{+}_{c} \bar{\Xi}^{0}$} & \makecell{$3402$ \\ $3643$ \\ $3783$} &  \\
\hline
  \caption{$T_{c\bar{s}u\bar{u}}$ thresholds.} \label{table:Tcusu_thresholds}
 \end{longtable}

==> tetraquarks/predictions/cu-uu/j_predictions.tex <==
\begin{longtable}[c]{|c|c|}
  \hline
  \thead{$J$ \\ Spec} & \thead{$a_{T_{j}}$} \\
  \hline
  \hline
\makecell{$2634-2779$\\$2972-3095$\\$3264-3374$\\$3526-3626$\\$3766-3858$\\$3988-4075$\\$4197-4278$\\$4394-4471$\\$4581-4655$\\$4760-4831$\\$4931-5000$\\$5097-5162$} & \makecell{$-1.6$-$-1.2$} \\
\hline
  \caption{$T_{c\bar{u}u\bar{u}}$ $(J, M^2)$ predictions.} \label{table:Tcuuu_j_predictions}
 \end{longtable}

==> tetraquarks/predictions/cu-uu/n_predictions.tex <==
\begin{longtable}[c]{|c|c|}
  \hline
  \thead{$n$ \\ Spec} & \thead{$a_{T_{n}}$} \\
  \hline
  \hline
\makecell{$2270-2448$\\$2829-2961$\\$3264-3374$\\$3635-3731$\\$3964-4051$\\$4263-4344$\\$4540-4615$\\$4799-4869$\\$5042-5109$\\$5273-5337$\\$5494-5554$\\$5705-5763$} & \makecell{$-1.2$-$-0.92$} \\
\hline
  \caption{$T_{c\bar{u}u\bar{u}}$ $(n, M^2)$ predictions.} \label{table:Tcuuu_n_predictions}
 \end{longtable}

==> tetraquarks/predictions/cu-uu/thresholds.tex <==
\begin{longtable}[c]{|c|c|c|c|c|c|}
  \hline
  \thead{Thry \\ Width \\ $[MeV]$} & \thead{Mesons \\ Pair} & \thead{Meson \\ Threshold \\ $[MeV]$} & \thead{Baryon \\ Anti-\\baryon} & \thead{Baryonic \\ Threshold \\ $[MeV]$} & \thead{Genuine} \\
  \hline
  \hline
\makecell{$79-118$\\$30-61$} & \makecell{$D^{0} \pi^{0}_{u}$} & \makecell{$2000$} & \makecell{$\Lambda^{+}_{c} \bar{p}$ \\ $\Xi^{+}_{c} \bar{\Sigma}^{-}$ \\ $\Sigma^{++}_{c} \bar{\Delta}^{--}$} & \makecell{$3224$ \\ $3657$ \\ $3686$} &  \\
\hline
  \caption{$T_{c\bar{u}u\bar{u}}$ thresholds.} \label{table:Tcuuu_thresholds}
 \end{longtable}

==> tetraquarks/predictions/ds-cu/spectrum.tex <==
\setlength\LTleft{-1.2cm}
\setlength\LTpre{0.5cm}
{\small\tabcolsep=1pt\footnotesize{\begin{longtable}[!c]{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
  \hline
  \thead{$\#$} & \thead{Candi-\\dates} & \thead{$J^{PC}$} & \thead{Quarks} & \thead{Thry \\ Width \\ $[MeV]$} & \thead{Mesons \\ Pair} & \thead{Meson \\ Threshold \\ $[MeV]$} & \thead{Baryon \\ Anti-\\baryon} & \thead{Baryonic \\ Threshold \\ $[MeV]$} & \thead{$J$ \\ Spec} & \thead{$n$ \\ Spec} & \thead{$a_{T_{j}}$ \\ $a_{T_{n}}$} & \thead{Thry \\ $J + n$} & \thead{Gen-\\uine} \\
  \hline
  \hline
1 & \makecell{} & \makecell{} & $d\bar{c}s\bar{u}$ & \makecell{$98-147$\\$29-59$} & \makecell{$\pi^{-} D^{-}_{s}$ \\ $D^{-} K^{-}$} & \makecell{$2108$ \\ $2364$} & \makecell{$\Sigma^{-} \bar{\Lambda}^{-}_{c}$ \\ $\Lambda^{0} \bar{\Sigma}^{--}_{c}$ \\ $\Xi^{-} \bar{\Xi}^{-}_{c}$} & \makecell{$3483$ \\ $3570$ \\ $3790$} & \makecell{$2946-3085$\\$3252-3374$\\$3523-3633$\\$3769-3870$\\$3996-4091$} & \makecell{$2628-2791$\\$3121-3250$\\$3523-3633$\\$3872-3970$\\$4186-4275$} & \makecell{\makecell{$-2.1$-$-1.6$} \\ \makecell{$-1.5$-$-1.2$}} & \makecell{$3$ \\ $2$} & $**$ \\
\hline
 \caption{Tetraquark predicted configurations and thresholds.} \label{table:charm_tetraquarks_predictions}
\end{longtable}}\normalsize}

==> tetraquarks/predictions/du-du/spectrum.tex <==
\setlength\LTleft{-1.2cm}
\setlength\LTpre{0.5cm}
{\small\tabcolsep=1pt\footnotesize{\begin{longtable}[!c]{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
  \hline
  \thead{$\#$} & \thead{Candi-\\dates} & \thead{$J^{PC}$} & \thead{Quarks} & \thead{Thry \\ Width \\ $[MeV]$} & \thead{Mesons \\ Pair} & \thead{Meson \\ Threshold \\ $[MeV]$} & \thead{Baryon \\ Anti-\\baryon} & \thead{Baryonic \\ Threshold \\ $[MeV]$} & \thead{$J$ \\ Spec} & \thead{$n$ \\ Spec} & \thead{$a_{T_{j}}$ \\ $a_{T_{n}}$} & \thead{Thry \\ $J + n$} & \thead{Gen-\\uine} \\
  \hline
  \hline
1 & \makecell{$f_{4}(2300)$} & \makecell{$4^{++}$} & $d\bar{d}u\bar{u}$ & \makecell{$25-115$\\$38-75$} & \makecell{$\pi^{0}_{d} \pi^{0}_{u}$ \\ $\pi^{-} \pi^{+}$} & \makecell{$270$ \\ $280$} & \makecell{$p \bar{p}$ \\ $n \bar{n}$ \\ $\Lambda^{0} \bar{\Lambda}^{0}$} & \makecell{$1876$ \\ $1880$ \\ $2232$} & \makecell{$1157-1332$\\$1583-1715$\\$1916-2026$\\$2199-2295$\\$2450-2536$} & \makecell{$1120-1300$\\$1570-1702$\\$1916-2026$\\$2209-2305$\\$2467-2553$} & \makecell{\makecell{$-1.5$-$-1.1$} \\ \makecell{$-1.4$-$-1.0$}} & \makecell{$2$} &  \\
\hline
 \caption{Tetraquark predicted configurations and thresholds.} \label{table:charm_tetraquarks_predictions}
\end{longtable}}\normalsize}

==> tetraquarks/predictions/du-su/spectrum.tex <==
\setlength\LTleft{-1.2cm}
\setlength\LTpre{0.5cm}
{\small\tabcolsep=1pt\footnotesize{\begin{longtable}[!c]{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
  \hline
  \thead{$\#$} & \thead{Candi-\\dates} & \thead{$J^{PC}$} & \thead{Quarks} & \thead{Thry \\ Width \\ $[MeV]$} & \thead{Mesons \\ Pair} & \thead{Meson \\ Threshold \\ $[MeV]$} & \thead{Baryon \\ Anti-\\baryon} & \thead{Baryonic \\ Threshold \\ $[MeV]$} & \thead{$J$ \\ Spec} & \thead{$n$ \\ Spec} & \thead{$a_{T_{j}}$ \\ $a_{T_{n}}$} & \thead{Thry \\ $J + n$} & \thead{Gen-\\uine} \\
  \hline
  \hline
1 & \makecell{$K(3100)^{0}$} & \makecell{$?^{??}$} & $d\bar{s}u\bar{u}$ & \makecell{$45-209$\\$34-66$} & \makecell{$K^{0} \pi^{0}_{u}$ \\ $\pi^{-} K^{+}$} & \makecell{$633$ \\ $634$} & \makecell{$n \bar{\Lambda}^{0}$ \\ $p \bar{\Sigma}^{-}$ \\ $\Lambda^{0} \bar{\Xi}^{0}$} & \makecell{$2056$ \\ $2127$ \\ $2431$} & \makecell{$1378-1547$\\$1778-1908$\\$2096-2206$\\$2369-2466$\\$2611-2699$} & \makecell{$1344-1517$\\$1765-1896$\\$2096-2206$\\$2378-2475$\\$2628-2715$} & \makecell{\makecell{$-1.5$-$-1.2$} \\ \makecell{$-1.4$-$-1.0$}} & \makecell{$2$} &  \\
\hline
 \caption{Tetraquark predicted configurations and thresholds.} \label{table:charm_tetraquarks_predictions}
\end{longtable}}\normalsize}

==> tetraquarks/predictions/su-su/spectrum.tex <==
\setlength\LTleft{-1.2cm}
\setlength\LTpre{0.5cm}
{\small\tabcolsep=1pt\footnotesize{\begin{longtable}[!c]{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
  \hline
  \thead{$\#$} & \thead{Candi-\\dates} & \thead{$J^{PC}$} & \thead{Quarks} & \thead{Thry \\ Width \\ $[MeV]$} & \thead{Mesons \\ Pair} & \thead{Meson \\ Threshold \\ $[MeV]$} & \thead{Baryon \\ Anti-\\baryon} & \thead{Baryonic \\ Threshold \\ $[MeV]$} & \thead{$J$ \\ Spec} & \thead{$n$ \\ Spec} & \thead{$a_{T_{j}}$ \\ $a_{T_{n}}$} & \thead{Thry \\ $J + n$} & \thead{Gen-\\uine} \\
  \hline
  \hline
1 & \makecell{$f_{2}(2300)$\\$\omega(2300)$\\$f_{3}(2300)$\\$X(3250)$\\$X(3250)$} & \makecell{$2^{++}$\\$1^{--}$\\$3^{++}$\\$?^{??}$\\$?^{??}$} & $s\bar{s}u\bar{u}$ & \makecell{$79-364$\\$30-59$} & \makecell{$K^{-} K^{+}$ \\ $\phi(1020) \pi^{0}_{u}$} & \makecell{$988$ \\ $1154$} & \makecell{$\Lambda^{0} \bar{\Lambda}^{0}$ \\ $\Sigma^{+} \bar{\Sigma}^{-}$ \\ $\Xi^{0} \bar{\Xi}^{0}$} & \makecell{$2232$ \\ $2378$ \\ $2630$} & \makecell{$1591-1755$\\$1968-2097$\\$2272-2382$\\$2535-2633$\\$2770-2859$} & \makecell{$1559-1727$\\$1956-2085$\\$2272-2382$\\$2544-2641$\\$2786-2875$} & \makecell{\makecell{$-1.6$-$-1.2$} \\ \makecell{$-1.5$-$-1.1$}} & \makecell{$2$} &  \\
\hline
 \caption{Tetraquark predicted configurations and thresholds.} \label{table:charm_tetraquarks_predictions}
\end{longtable}}\normalsize}

==> tetraquarks/predictions/su-uu/j_predictions.tex <==
\begin{longtable}[c]{|c|c|}
  \hline
  \thead{$J$ \\ Spec} & \thead{$a_{T_{j}}$} \\
  \hline
  \hline
\makecell{$1375-1544$\\$1776-1906$\\$2094-2204$\\$2367-2464$\\$2610-2698$\\$2831-2912$\\$3035-3110$\\$3226-3296$\\$3405-3472$\\$3576-3639$\\$3738-3799$\\$3893-3952$} & \makecell{$-1.5$-$-1.2$} \\
\hline
  \caption{$T_{s\bar{u}u\bar{u}}$ $(J, M^2)$ predictions.} \label{table:Tsuuu_j_predictions}
 \end{longtable}

==> tetraquarks/predictions/su-uu/n_predictions.tex <==
\begin{longtable}[c]{|c|c|}
  \hline
  \thead{$n$ \\ Spec} & \thead{$a_{T_{n}}$} \\
  \hline
  \hline
\makecell{$1340-1514$\\$1763-1894$\\$2094-2204$\\$2376-2473$\\$2626-2714$\\$2854-2934$\\$3063-3138$\\$3259-3329$\\$3443-3509$\\$3618-3681$\\$3784-3844$\\$3943-4000$} & \makecell{$-1.4$-$-1.0$} \\
\hline
  \caption{$T_{s\bar{u}u\bar{u}}$ $(n, M^2)$ predictions.} \label{table:Tsuuu_n_predictions}
 \end{longtable}

==> tetraquarks/predictions/su-uu/spectrum.tex <==
\setlength\LTleft{-1.2cm}
\setlength\LTpre{0.5cm}
{\small\tabcolsep=1pt\footnotesize{\begin{longtable}[!c]{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
  \hline
  \thead{$\#$} & \thead{Candi-\\dates} & \thead{$J^{PC}$} & \thead{Quarks} & \thead{Thry \\ Width \\ $[MeV]$} & \thead{Mesons \\ Pair} & \thead{Meson \\ Threshold \\ $[MeV]$} & \thead{Baryon \\ Anti-\\baryon} & \thead{Baryonic \\ Threshold \\ $[MeV]$} & \thead{$J$ \\ Spec} & \thead{$n$ \\ Spec} & \thead{$a_{T_{j}}$ \\ $a_{T_{n}}$} & \thead{Thry \\ $J + n$} & \thead{Gen-\\uine} \\
  \hline
  \hline
1 & \makecell{} & \makecell{} & $s\bar{u}u\bar{u}$ & \makecell{$45-211$\\$33-66$} & \makecell{$K^{-} \pi^{0}_{u}$} & \makecell{$629$} & \makecell{$\Lambda^{0} \bar{p}$ \\ $\Sigma^{+} \bar{\Delta}^{--}$ \\ $\Xi^{0} \bar{\Sigma}^{-}$} & \makecell{$2054$ \\ $2421$ \\ $2504$} & \makecell{$1375-1544$\\$1776-1906$\\$2094-2204$\\$2367-2464$\\$2610-2698$} & \makecell{$1340-1514$\\$1763-1894$\\$2094-2204$\\$2376-2473$\\$2626-2714$} & \makecell{\makecell{$-1.5$-$-1.2$} \\ \makecell{$-1.4$-$-1.0$}} & \makecell{$2$} &  \\
\hline
 \caption{Tetraquark predicted configurations and thresholds.} \label{table:charm_tetraquarks_predictions}
\end{longtable}}\normalsize}

==> tetraquarks/predictions/su-uu/thresholds.tex <==
\begin{longtable}[c]{|c|c|c|c|c|c|}
  \hline
  \thead{Thry \\ Width \\ $[MeV]$} & \thead{Mesons \\ Pair} & \thead{Meson \\ Threshold \\ $[MeV]$} & \thead{Baryon \\ Anti-\\baryon} & \thead{Baryonic \\ Threshold \\ $[MeV]$} & \thead{Genuine} \\
  \hline
  \hline
\makecell{$45-211$\\$33-66$} & \makecell{$K^{-} \pi^{0}_{u}$} & \makecell{$629$} & \makecell{$\Lambda^{0} \bar{p}$ \\ $\Sigma^{+} \bar{\Delta}^{--}$ \\ $\Xi^{0} \bar{\Sigma}^{-}$} & \makecell{$2054$ \\ $2421$ \\ $2504$} &  \\
\hline
  \caption{$T_{s\bar{u}u\bar{u}}$ thresholds.} \label{table:Tsuuu_thresholds}
 \end{longtable}

==> tetraquarks/predictions/uu-du/spectrum.tex <==
\setlength\LTleft{-1.2cm}
\setlength\LTpre{0.5cm}
{\small\tabcolsep=1pt\footnotesize{\begin{longtable}[!c]{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
  \hline
  \thead{$\#$} & \thead{Candi-\\dates} & \thead{$J^{PC}$} & \thead{Quarks} & \thead{Thry \\ Width \\ $[MeV]$} & \thead{Mesons \\ Pair} & \thead{Meson \\ Threshold \\ $[MeV]$} & \thead{Baryon \\ Anti-\\baryon} & \thead{Baryonic \\ Threshold \\ $[MeV]$} & \thead{$J$ \\ Spec} & \thead{$n$ \\ Spec} & \thead{$a_{T_{j}}$ \\ $a_{T_{n}}$} & \thead{Thry \\ $J + n$} & \thead{Gen-\\uine} \\
  \hline
  \hline
1 & \makecell{} & \makecell{} & $u\bar{d}u\bar{u}$ & \makecell{$24-115$\\$38-75$} & \makecell{$\pi^{+} \pi^{0}_{u}$ \\ $\pi^{0}_{u} \pi^{+}$} & \makecell{$275$ \\ $275$} & \makecell{$p \bar{n}$ \\ $\Delta^{++} \bar{p}$ \\ $\Sigma^{+} \bar{\Lambda}^{0}$} & \makecell{$1878$ \\ $2170$ \\ $2305$} & \makecell{$1161-1335$\\$1585-1717$\\$1918-2028$\\$2201-2297$\\$2451-2538$} & \makecell{$1124-1303$\\$1572-1705$\\$1918-2028$\\$2210-2306$\\$2468-2555$} & \makecell{\makecell{$-1.5$-$-1.1$} \\ \makecell{$-1.4$-$-1.0$}} & \makecell{$2$} &  \\
\hline
 \caption{Tetraquark predicted configurations and thresholds.} \label{table:charm_tetraquarks_predictions}
\end{longtable}}\normalsize}

==> tetraquarks/predictions/uu-uu/j_predictions.tex <==
\begin{longtable}[c]{|c|c|}
  \hline
  \thead{$J$ \\ Spec} & \thead{$a_{T_{j}}$} \\
  \hline
  \hline
\makecell{$1157-1332$\\$1583-1715$\\$1916-2026$\\$2199-2295$\\$2450-2536$\\$2677-2756$\\$2886-2960$\\$3081-3150$\\$3264-3330$\\$3438-3500$\\$3603-3663$\\$3761-3818$} & \makecell{$-1.5$-$-1.1$} \\
\hline
  \caption{$T_{u\bar{u}u\bar{u}}$ $(J, M^2)$ predictions.} \label{table:Tuuuu_j_predictions}
 \end{longtable}

==> tetraquarks/predictions/uu-uu/n_predictions.tex <==
\begin{longtable}[c]{|c|c|}
  \hline
  \thead{$n$ \\ Spec} & \thead{$a_{T_{n}}$} \\
  \hline
  \hline
\makecell{$1120-1300$\\$1570-1702$\\$1916-2026$\\$2209-2305$\\$2467-2553$\\$2700-2779$\\$2915-2988$\\$3115-3184$\\$3303-3368$\\$3481-3542$\\$3650-3709$\\$3811-3868$} & \makecell{$-1.4$-$-1.0$} \\
\hline
  \caption{$T_{u\bar{u}u\bar{u}}$ $(n, M^2)$ predictions.} \label{table:Tuuuu_n_predictions}
 \end{longtable}

==> tetraquarks/predictions/uu-uu/spectrum.tex <==
\setlength\LTleft{-1.2cm}
\setlength\LTpre{0.5cm}
{\small\tabcolsep=1pt\footnotesize{\begin{longtable}[!c]{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
  \hline
  \thead{$\#$} & \thead{Candi-\\dates} & \thead{$J^{PC}$} & \thead{Quarks} & \thead{Thry \\ Width \\ $[MeV]$} & \thead{Mesons \\ Pair} & \thead{Meson \\ Threshold \\ $[MeV]$} & \thead{Baryon \\ Anti-\\baryon} & \thead{Baryonic \\ Threshold \\ $[MeV]$} & \thead{$J$ \\ Spec} & \thead{$n$ \\ Spec} & \thead{$a_{T_{j}}$ \\ $a_{T_{n}}$} & \thead{Thry \\ $J + n$} & \thead{Gen-\\uine} \\
  \hline
  \hline
1 & \makecell{} & \makecell{} & $u\bar{u}u\bar{u}$ & \makecell{$25-115$\\$38-75$} & \makecell{$\pi^{0}_{u} \pi^{0}_{u}$} & \makecell{$270$} & \makecell{$p \bar{p}$ \\ $\Sigma^{+} \bar{\Sigma}^{-}$ \\ $\Delta^{++} \bar{\Delta}^{--}$} & \makecell{$1876$ \\ $2378$ \\ $2464$} & \makecell{$1157-1332$\\$1583-1715$\\$1916-2026$\\$2199-2295$\\$2450-2536$} & \makecell{$1120-1300$\\$1570-1702$\\$1916-2026$\\$2209-2305$\\$2467-2553$} & \makecell{\makecell{$-1.5$-$-1.1$} \\ \makecell{$-1.4$-$-1.0$}} & \makecell{$2$} &  \\
\hline
 \caption{Tetraquark predicted configurations and thresholds.} \label{table:charm_tetraquarks_predictions}
\end{longtable}}\normalsize}

==> tetraquarks/predictions/uu-uu/thresholds.tex <==
\begin{longtable}[c]{|c|c|c|c|c|c|}
  \hline
  \thead{Thry \\ Width \\ $[MeV]$} & \thead{Mesons \\ Pair} & \thead{Meson \\ Threshold \\ $[MeV]$} & \thead{Baryon \\ Anti-\\baryon} & \thead{Baryonic \\ Threshold \\ $[MeV]$} & \thead{Genuine} \\
  \hline
  \hline
\makecell{$25-115$\\$38-75$} & \makecell{$\pi^{0}_{u} \pi^{0}_{u}$} & \makecell{$270$} & \makecell{$p \bar{p}$ \\ $\Sigma^{+} \bar{\Sigma}^{-}$ \\ $\Delta^{++} \bar{\Delta}^{--}$} & \makecell{$1876$ \\ $2378$ \\ $2464$} &  \\
\hline
  \caption{$T_{u\bar{u}u\bar{u}}$ thresholds.} \label{table:Tuuuu_thresholds}
 \end{longtable}

==> tetraquarks/psi/by_n/fit-_psi_1j_psi_fixed_m_n.tex <==
\begin{longtable}[c]{|c|c|c|c|c|c|}
  \hline
  \thead{$State$} & \thead{$M$ \\ $[MeV]$} & \thead{Thry \\ $M$ \\ $[MeV]$} & \thead{$J$} & \thead{Thry \\ $n$} & \thead{Thry \\ $J + n$} \\
  \hline
  \hline
$\psi(4360)$ & $4372$ & $4364$ & $1$ & $0$ & $1$ \\
\hline
$\psi(4660)$ & $4630$ & $4637$ & $1$ & $1$ & $2$ \\
\hline
 &  & $4885$ &  &  & $3$ \\
\hline
 &  & $5115$ &  &  & $4$ \\
\hline
 &  & $5329$ &  &  & $5$ \\
\hline
 &  & $5531$ &  &  & $6$ \\
\hline
  \caption{$\psi$ $(n, M^{2})$ HMRT.}
 \end{longtable}

==> tetraquarks/psi/by_n/fit-_psi_1j_psi_new_n.tex <==
\begin{longtable}[c]{|c|c|c|c|c|c|}
  \hline
  \thead{$State$} & \thead{$M$ \\ $[MeV]$} & \thead{Thry \\ $M$ \\ $[MeV]$} & \thead{$J$} & \thead{Thry \\ $n$} & \thead{Thry \\ $J + n$} \\
  \hline
  \hline
$\psi(4360)$ & $4372$ & $4372$ & $1$ & $0$ & $1$ \\
\hline
$\psi(4660)$ & $4630$ & $4630$ & $1$ & $1$ & $2$ \\
\hline
 &  & $4869$ &  &  & $3$ \\
\hline
 &  & $5094$ &  &  & $4$ \\
\hline
 &  & $5306$ &  &  & $5$ \\
\hline
 &  & $5508$ &  &  & $6$ \\
\hline
  \caption{$\psi$ $(n, M^{2})$ HMRT.}
 \end{longtable}

==> tetraquarks/psi/by_n/fit-_psi_1j_psi_prev_n.tex <==
\begin{longtable}[c]{|c|c|c|c|c|c|}
  \hline
  \thead{$State$} & \thead{$M$ \\ $[MeV]$} & \thead{Thry \\ $M$ \\ $[MeV]$} & \thead{$J$} & \thead{Thry \\ $n$} & \thead{Thry \\ $J + n$} \\
  \hline
  \hline
$\psi(4360)$ & $4372$ & $4329$ & $1$ & $0$ & $1$ \\
\hline
$\psi(4660)$ & $4630$ & $4678$ & $1$ & $1$ & $2$ \\
\hline
 &  & $4987$ &  &  & $3$ \\
\hline
 &  & $5268$ &  &  & $4$ \\
\hline
 &  & $5528$ &  &  & $5$ \\
\hline
 &  & $5772$ &  &  & $6$ \\
\hline
  \caption{$\psi$ $(n, M^{2})$ HMRT.}
 \end{longtable}

==> tetraquarks/rho_3/by_J_one_point/fit-_rho__rho_tetra_one_by_j.tex <==
\begin{longtable}[c]{|c|c|c|c|c|c|}
  \hline
  \thead{$State$} & \thead{$M$ \\ $[MeV]$} & \thead{Thry \\ $M$ \\ $[MeV]$} & \thead{$J$} & \thead{Thry \\ $n$} & \thead{Thry \\ $J + n$} \\
  \hline
  \hline
 &  & $1653$ &  &  & $2$ \\
\hline
 &  & $1974$ &  &  & $3$ \\
\hline
$\rho(2250)^{+}$ & $2250$ & $2250$ & $3$ & $1$ & $4$ \\
\hline
 &  & $2495$ &  &  & $5$ \\
\hline
 &  & $2719$ &  &  & $6$ \\
\hline
  \caption{$$\rho_{3}$ $(J, M^{2})$$ HMRT.} \label{table:rho_3_2250_J_HMRT}
 \end{longtable}

==> tetraquarks/rho_3/by_n_one_point/fit-_rho__rho_tetra_one_by_n.tex <==
\begin{longtable}[c]{|c|c|c|c|c|c|}
  \hline
  \thead{$State$} & \thead{$M$ \\ $[MeV]$} & \thead{Thry \\ $M$ \\ $[MeV]$} & \thead{$J$} & \thead{Thry \\ $n$} & \thead{Thry \\ $J + n$} \\
  \hline
  \hline
 &  & $1627$ &  &  & $1$ \\
\hline
 &  & $1964$ &  &  & $2$ \\
\hline
$\rho(2250)^{+}$ & $2250$ & $2250$ & $3$ & $0$ & $3$ \\
\hline
 &  & $2504$ &  &  & $4$ \\
\hline
 &  & $2734$ &  &  & $5$ \\
\hline
  \caption{$$\rho_{3}$ $(n, M^{2})$$ HMRT.} \label{table:rho_3_2250_n_HMRT}
 \end{longtable}

==> tetraquarks/thresholds/Tcbdd_one_by_J.tex <==
\begin{table}[!ht]
 \centering
 {\small
 \begin{longtable}[c]{|c|c|c|c|c|c|}
  \hline
  \hline
  \thead{$State$} & \thead{$M [MeV]$} & \thead{Thry \\ $M [MeV]$} & \thead{$J$} & \thead{Thry \\ $n$} & \thead{Thry \\ $J + n$} \\
  \hline
  \hline
 &  & $7613$ &  &  & $-2$ \\
\hline
 &  & $7768$ &  &  & $-1$ \\
\hline
 &  & $7913$ &  &  & $0$ \\
\hline
 &  & $8051$ &  &  & $1$ \\
\hline
 &  & $8182$ &  &  & $2$ \\
\hline
$T_{c\bar{b}d\bar{d}}$ & $8307$ & $8307$ &  &  & $3$ \\
\hline
 &  & $8427$ &  &  & $4$ \\
\hline
 &  & $8544$ &  &  & $5$ \\
\hline
 &  & $8656$ &  &  & $6$ \\
\hline
  \hline
 \end{longtable}}
 \caption{T_{c\bar{b}d\bar{d}} Regge trajectory.}
\end{table}

==> tetraquarks/thresholds/Tcbdd_one_by_n.tex <==
\begin{table}[!ht]
 \centering
 {\small
 \begin{longtable}[c]{|c|c|c|c|c|c|}
  \hline
  \hline
  \thead{$State$} & \thead{$M [MeV]$} & \thead{Thry \\ $M [MeV]$} & \thead{$J$} & \thead{Thry \\ $n$} & \thead{Thry \\ $J + n$} \\
  \hline
  \hline
 &  & $6954$ &  &  & $-2$ \\
\hline
 &  & $7286$ &  &  & $-1$ \\
\hline
 &  & $7577$ &  &  & $0$ \\
\hline
 &  & $7839$ &  &  & $1$ \\
\hline
 &  & $8081$ &  &  & $2$ \\
\hline
$T_{c\bar{b}d\bar{d}}$ & $8307$ & $8307$ &  &  & $3$ \\
\hline
 &  & $8520$ &  &  & $4$ \\
\hline
 &  & $8722$ &  &  & $5$ \\
\hline
 &  & $8915$ &  &  & $6$ \\
\hline
  \hline
 \end{longtable}}
 \caption{T_{c\bar{b}d\bar{d}} Regge trajectory.}
\end{table}

==> tetraquarks/thresholds/Tcbds_one_by_J.tex <==
\begin{table}[!ht]
 \centering
 {\small
 \begin{longtable}[c]{|c|c|c|c|c|c|}
  \hline
  \hline
  \thead{$State$} & \thead{$M [MeV]$} & \thead{Thry \\ $M [MeV]$} & \thead{$J$} & \thead{Thry \\ $n$} & \thead{Thry \\ $J + n$} \\
  \hline
  \hline
 &  & $7290$ &  &  & $-2$ \\
\hline
 &  & $7487$ &  &  & $-1$ \\
\hline
 &  & $7664$ &  &  & $0$ \\
\hline
 &  & $7826$ &  &  & $1$ \\
\hline
 &  & $7976$ &  &  & $2$ \\
\hline
$T_{c\bar{b}d\bar{s}}$ & $8118$ & $8118$ &  &  & $3$ \\
\hline
 &  & $8252$ &  &  & $4$ \\
\hline
 &  & $8381$ &  &  & $5$ \\
\hline
 &  & $8504$ &  &  & $6$ \\
\hline
  \hline
 \end{longtable}}
 \caption{T_{c\bar{b}d\bar{s}} Regge trajectory.}
\end{table}

==> tetraquarks/thresholds/Tcbds_one_by_n.tex <==
\begin{table}[!ht]
 \centering
 {\small
 \begin{longtable}[c]{|c|c|c|c|c|c|}
  \hline
  \hline
  \thead{$State$} & \thead{$M [MeV]$} & \thead{Thry \\ $M [MeV]$} & \thead{$J$} & \thead{Thry \\ $n$} & \thead{Thry \\ $J + n$} \\
  \hline
  \hline
 &  & $6296$ &  &  & $-2$ \\
\hline
 &  & $6582$ &  &  & $-1$ \\
\hline
 &  & $7136$ &  &  & $0$ \\
\hline
 &  & $7518$ &  &  & $1$ \\
\hline
 &  & $7837$ &  &  & $2$ \\
\hline
$T_{c\bar{b}d\bar{s}}$ & $8118$ & $8118$ &  &  & $3$ \\
\hline
 &  & $8373$ &  &  & $4$ \\
\hline
 &  & $8609$ &  &  & $5$ \\
\hline
 &  & $8829$ &  &  & $6$ \\
\hline
  \hline
 \end{longtable}}
 \caption{T_{c\bar{b}d\bar{s}} Regge trajectory.}
\end{table}
